Querying Circumscribed Description Logic Knowledge Bases

Circumscription is one of the main approaches for defining non-monotonic description logics (DLs). While the decidability and complexity of traditional reasoning tasks such as satisfiability of circumscribed DL knowledge bases (KBs) is well understood, for evaluating conjunctive queries (CQs) and unions thereof (UCQs), not even decidability had been established. In this paper, we prove decidability of (U)CQ evaluation on circumscribed DL KBs and obtain a rather complete picture of both the combined complexity and the data complexity, for DLs ranging from ALCHIO via EL to various versions of DL-Lite. We also study the much simpler atomic queries (AQs).

==> bool-neighborhoods.tex <==
%!TEX root = main.tex



Using bool-neighborhoods in the quotient construction presented in Section~\ref{subsection-alchi-data}, the number of equivalence classes drops, yielding the following:


\begin{restatable}{lemma}{lemmaboolcountermodel}
	\label{lemma-bool-countermodel}
	If there exists a countermodel for an UCQ $q$ over a $\dllitebool$ cKB $\circkb$, then there exists a countermodel for $q$ over $\circkb$ with size at most $(\sizeof{\abox} + 2^\sizeof{\tbox})^{\sizeof{q}^2(\sizeof{\tbox} +1)}$.
\end{restatable}


\iffalse

As for the general $\ALCHI$ case, this leads us to characterize the $n$-core-neighbourhood of an element $c \in \interleavingof{\I}$ via a subset $\Sigma_{n, c}$ of $\Omega_{n}$, (we recall $\Omega_n$ is the set of words over $\Omega$ with length $\leq 2n$) and by the following function $\chi_{n, c}$.
\[
\begin{array}{l}
	\chi_{n, c} : \Sigma_{n, c} \rightarrow  \domain{*} \cup \{ \emptyset \} \\
	w      \mapsto \left \lbrace 
	\begin{array}{ll}
		\emptyset &  \text{if } \interlace(\neighroot{n}{c} w) \notin \domain{*} \\
		\interlace(\neighroot{n}{c} w) & \text{if } \interlace(\neighroot{n}{c} w) \in \domain{*}
	\end{array} \right.
\end{array}
\]
%\todo{previous par uses $\Sigma_c^{q, n}$, but preceding math, this par, and next def uses $\Sigma_{n, c}$}
Notice Lemma~\ref{lemma-poly-neighborhoods} ensures the set $\Sigma_{n, c}$ has size at most $\sizeof{q}^2 ( \sizeof{\tbox} + 1)$, that is polynomial, while we kept track of the full $\Omega_n$ in the $\ALCHI$ setting.
This will ensure that the following equivalence relation, used to merge elements, only admits an exponential number of equivalent classes.

\begin{definition}
	The equivalence relation $\sim^{\textrm{core}}_n$ on $\boolunrav$ is defined as follows: an element $e \in \domain{*}$ is $\sim_n$-equivalent only to itself; elements {$c_1, c_2$} from $\domain{\interleavingof{\I}} \setminus \domain{*}$ are $\sim^{\textrm{core}}_n$-equivalent iff
	{
		$w^{c_1}_{n, c_1} = w^{c_2}_{n, c_2}$,
		$\chi_{n, c_1} = \chi_{n, c_2}$, 
		$\Sigma_{n, c_1} = \Sigma_{n, c_2}$,
		and $|c_1| = |c_2| \!\!\mod \maxmod$.
	}
\end{definition}

We obtain a finite model of the required size by merging elements with respect to $\sim^{\textrm{core}}_{\maxradius}$. 

\begin{theorem}
	\label{theorem:core-quotient}
	The interpretation $\J := \interleavingof{\I}/{\sim^{\textrm{core}}_{\maxradius}}$ is a model of $\kb$ that has at most as many c-matches for $q$ as $\countermodel$. 
	Its size is polynomial w.r.t. data complexity, simply-exponential w.r.t. combined complexity.
\end{theorem}

\begin{proof}
	Modelhood is known from \cite{kostylevreutter:count}, but can also be easily verified based on the $\DLcore$ subparts from the proof of Theorem~\ref{theorem:quotient}.
	
	To obtain an injective mapping of counting matches of $q$ in $\J$ to counting matches of $q$ in $\boolunrav$, one follows
	a similar proof strategy to the one used in 
	%the same proof line as in 
	Section~\ref{chapter:ccq-section:finite-countermodels-subsection:alchi}, building homomorphisms from core-neighbourhoods in the quotient to core-neighbourhoods in the interleaving.
	We shall not go into %unfold 
	the full details, but instead mention a significant point.
	In the proof of Theorem~\ref{morphismneighbourhoods}, one can verify the image of inductively built homomorphisms $\qtoi{n}$ belongs to the $n$-core-neighbourhood (and not simply to the usual $n$-neigbourhood!).
	Indeed, when building the image of an element $\overline{e}$ belonging to $\coreneighof{n}{\overline{c}}{\J}{\overline{\domain{\basecandidate}}}$, hence being reached by some match $\match : p \rightarrow \J_{\mid (\coreneighof{n-1}{\overline{c}}{\J}{\overline{\domain{\basecandidate}}} \,\setminus\, \overline{\domain{\basecandidate}}) \,\cup\, \{ \overline{e} \}}$, the resulting element $\qtoiof{n}{e}$ is reached by the match $\qtoi{n} \circ \match : p \rightarrow \boolunrav_{\mid (\coreneighof{n-1}{c}{\boolunrav}{{\domain{\basecandidate}}} \,\setminus\, {\domain{\basecandidate}}) \,\cup\, \{ e \}}$, ensuring $\qtoiof{n}{e}$ belongs to $\coreneighof{n}{c}{\boolunrav}{\domain{\basecandidate}}$.
	
	Finally, regarding the size of $\J$, we remark that an equivalence class $\overline{d}$ is now characterized by:
	$|d| \mod \maxmod$, that is one equivalence class among $\maxmod$ possible classes;
	$w_{\maxradius, d}^d$, that is a word over an alphabet with at most $|\tbox|$ symbols and a length at most $\maxradius$;
	$\Sigma_{\maxradius, d}$, that is a subset, with size at most $\sizeof{q}^2 ( \sizeof{\tbox} + 1)$ (Lemma~\ref{lemma-poly-neighborhoods}), of the exponentially large set $\Omega_n$;
	and $\chi_{\maxradius, d}$, that is a function from a set with at most $\sizeof{q}^2 ( \sizeof{\tbox} + 1)$ elements to a set with at most $|\domain{*}| + 1$ elements. %\todo{is this bound correct, shouldn't it be just $|\domain{*}|  + 1$ elements?}
	Therefore, the number of possibly different equivalence classes, that is $|\domain{\J}|$, is at most:
	\[
	(2\sizeof{q} + 3) \times |\tbox|^{\sizeof{q} + 2} \times ({|\tbox|^{2\sizeof{q} + 3}})^{\sizeof{q}^2 ( \sizeof{\tbox} + 1)} \times (|\domain{*}| + 1)^{\sizeof{q}^2 ( \sizeof{\tbox} + 1)}.
	\]
	Recall Lemma~\ref{lemma:basic-counter-models} allows to assume $|\domain{*}| \leq |\individuals| + (\sizeof{\individuals(\abox)} + 3 \, \sizeof{\tbox}\, 2^{\sizeof{\tbox}})^\sizeof{q} |q|$, we have the claimed bounds for the size of $\J$, which concludes the proof of Theorem~\ref{theorem:core-quotient}.
\end{proof}
\fi

==> criteria-combined.tex <==
%!TEX root = main.tex


\begin{lemma}
	\label{lemma-criteria-combined}
	%Let $\I$ be a model of a $\dllitebool^{\Hmc^-}$ KB $\kb$ and $\CP$ a circumscription pattern.
	The following two conditions are equivalent:
	\begin{enumerate}
		\item There exists $\J \models \kb$ s.t.\ $\J <_\CP \I$;
		\item There exist $\Pmc \subseteq \domain{\I}$ with $\sizeof{\Pmc} \leq 2\sizeof{\tbox} + 1$ and $\J_\Pmc \models \kb$ with $\J_\Pmc <_\CP \I_\Pmc$ s.t.\ for all $e \in \domain{\I} \setminus \domain{\I_\Pmc}$, there exists $\J_{\Pmc, e} \models \kb$ with $\J_{\Pmc, e} <_\CP \I_{\Pmc \cup \{ e\} }$ and $\J_{\Pmc, e}|_{\domain{\J_\Pmc}} = \J_\Pmc$.
	\end{enumerate} 
\end{lemma}

The intuition behind our criteria is that the union of all $\J_{\Pmc, e}$, since they agree on $\J_\Pmc$, forms a suitable $\J$.

To piece together the $\J_{\Pmc, e}$, we first prove the following property:

\begin{lemma}
	\label{lemma-portions-union}
	%Let $\I$ be a model of a $\dllitebool^{\Hmc^-}$ KB $\kb$ and $\CP$ a circumscription pattern.
	Let $\Pmc_1, \Pmc_2 \subseteq \domain{\I}$ and $\J_1$, $\J_2$ two models of $\kb$ s.t.\ $\J_1 <_\CP \I_{\Pmc_1}$ and $\J_2 <_\CP \I_{\Pmc_2}$.
	If $\J_1 |_{\domain{\J_2}} = \J_2 |_{\domain{\J_1}}$, then $\J_1 \cup \J_2 <_\CP \I_{\Pmc_1 \cup \Pmc_2}$.
\end{lemma}

\begin{proof}
	Assume $\J_1 |_{\domain{\J_2}} = \J_2 |_{\domain{\J_1}}$.
	It is easily verified that $\J_1 \cup \J_2$ is also a model of $\kb$ since $\J_1$ and $\J_2$ agree on their shared domain.
	We now check that all four conditions from the definition of $<_\CP$ are satisfied:
	\begin{enumerate}
		\item 
		From $\J_1 <_\CP \I_{\Pmc_1}$ we have $\domain{\J_1} = \domain{\I_{\Pmc_1}}$ and similarly for $\J_2$ we have $\domain{\J_2} = \domain{\I_{\Pmc_2}}$.
		It follows from its definition that $\domain{\I_{\Pmc_1 \cup \Pmc_2}} = \domain{\I_{\Pmc_1}} \cup \domain{\I_{\Pmc_2}}$.
		Therefore we have as desired $\domain{\J_1 \cup \J_2} = \domain{\I_{\Pmc_1 \cup \Pmc_2}}$.
		\item 
		Let $A \in \Fsf$.
		From $\J_1 <_\CP \I_{\Pmc_1}$ we have $A^{\J_1} = A^{\I_{\Pmc_1}}$ and similarly for $\J_2$ we have $A^{\J_2} = A^{\I_{\Pmc_2}}$.
		It follows from its definition that $A^{\I_{\Pmc_1 \cup \Pmc_2}} = A^{\I_{\Pmc_1}} \cup A^{\I_{\Pmc_2}}$.
		Therefore we have as desired $A^{\J_1 \cup \J_2} = A^{\I_{\Pmc_1 \cup \Pmc_2}}$.
		\item 
		Let $A \in \Msf$ such that $A^{\J_1 \cup \J_2} \not\subseteq A^{\I_{\Pmc_1 \cup \Pmc_2}}$.
		We may assume w.l.o.g.\ that $A$ is minimal w.r.t.\ $\prec$ for this property.
		We thus have $e \in A^{\J_1 \cup \J_2} \setminus A^{\I_{\Pmc_1 \cup \Pmc_2}}$.
		We either have $e \in \domain{\J_1}$ or $e \in \domain{\J_2}$.
		We treat the case $e \in \domain{\J_1}$, the arguments for $e \in \domain{\J_2}$ are similar.
		From $\J_1 <_\CP \I_{\Pmc_1}$, there exists a concept $B_1 \prec A$ s.t.\ $B_1^{\J_1} \subsetneq B_1^{\I_{\Pmc_1}}$.
		We chose such a $B_1$ that is minimal for this property, that is s.t.\ for all $B \prec B_1$, we have $B^{\J_1} = B^{\I_{\Pmc_1}}$ (recall $A$ is minimal for its property so that such a $B$ must verify $B^{\J_1 \cup \J_2} \subseteq B^{\I_{\Pmc_1 \cup \Pmc_2}}$ hence $B^{\J_1} \subseteq B^{\I_{\Pmc_1}}$).
		If $B_1^{\J_2} \subseteq B_1^{\I_{\Pmc_2}}$, then we are done as we obtain $B_1^{\J_1 \cup \J_2} \subsetneq B_1^{\I_{\Pmc_1 \cup \Pmc_2}}$.
		Otherwise, we have $B_1^{\J_2} \not\subseteq B_1^{\I_{\Pmc_2}}$ and from $\J_2 <_\CP \I_{\Pmc_2}$, there exists a concept $B_2 \prec B_1$ s.t.\ $B_2^{\J_2} \subsetneq B_2^{\I_{\Pmc_2}}$.
		Since $B_1$ has been chosen minimal, we have in particular $B_2^{\J_1} = B_2^{\I_{\Pmc_1}}$, which yields $B_2^{\J_1 \cup \J_2} \subsetneq B_2^{\I_{\Pmc_1 \cup \Pmc_2}}$.
		\item
		From $\J_1 <_\CP \I_{\Pmc_1}$, there exists a concept $A_1 \in \Msf$ s.t.\ $A_1^{\J_1} \subsetneq A_1^{\I_{\Pmc_1}}$ and for all $B \prec A_1$, we have $B^{\J_1} = B^{\I_{\Pmc_1}}$.
		If $A_1^{\J_2} \subsetneq A_2^{\Pmc_2}$ and for all $B \prec A_1$, $B^{\J_2} = B^{\Pmc_2}$, then we obtain directly $A_1^{\J_1 \cup \J_2} \subsetneq A_1^{\I_{\Pmc_1 \cup \Pmc_2}}$ and for all $B \prec A_1$, $B^{\J_1 \cup \J_2} = B^{\I_{\Pmc_1 \cup \Pmc_2}}$ and we are done.
		Otherwise:
		\begin{itemize}
			\item If $A_1^{\J_2} \not\subseteq A_1^{\I_{\Pmc_2}}$, then from $\J_2 <_\CP \I_{\Pmc_2}$, there exists a concept $A_2 \prec A_1$ s.t.\ $A_2^{\J_2} \subsetneq A_2^{\I_{\Pmc_2}}$.
			Consider a minimal such $A_2$, that is s.t.\ for all $A \prec A_2$, we have $A^{\J_2} = A^{\I_{\Pmc_2}}$ or $A^{\J_2} \not\subseteq A^{\I_{\Pmc_2}}$. 
			Notice the second option cannot happen otherwise from $\J_2 <_\CP \I_{\Pmc_2}$ we could obtain $A_3 \prec A_2$ s.t.\ $A_2^{\J_2} \subsetneq A_2^{\I_{\Pmc_2}}$, contradicting the minimality of $A_2$.
			Therefore $A_2$ being minimal yields that for all $A \prec A_2$, we have $A^{\J_2} = A^{\I_{\Pmc_2}}$.
			Now, from the minimality of $A_1$, we extend this to $\J_1 \cup \J_2$ and obtain $A_2^{\J_1 \cup \J_2} \subsetneq A_2^{\I_{\Pmc_1 \cup \Pmc_2}}$ and for all $B \prec A_2$, $B^{\J_1 \cup \J_2} = B^{\I_{\Pmc_1 \cup \Pmc_2}}$.
			\item If there exists $A_2 \prec A_1$ s.t.\ $A_2^{\J_2} \neq A_2^{\I_{\Pmc_2}}$.
			Consider a minimal such $A_2$, that is s.t.\ for all $A \prec A_2$, we have $A^{\J_2} = A^{\I_{\Pmc_2}}$.
			Notice we must have $A_2^{\J_2} \subseteq A_2^{\I_{\Pmc_2}}$, otherwise from $\J_2 <_\CP \I_{\Pmc_2}$ we could obtain $A_3 \prec A_2$ s.t.\ $A_2^{\J_2} \subsetneq A_2^{\I_{\Pmc_2}}$, contradicting that for all $A \prec A_2$, we have $A^{\J_2} = A^{\I_{\Pmc_2}}$.
			Therefore, since $A_2^{\J_2} \neq A_2^{\I_{\Pmc_2}}$, it must be that $A_2^{\J_2} \subsetneq A_2^{\I_{\Pmc_2}}$.
			Now, from the minimality of $A_1$, we extend this to $\J_1 \cup \J_2$ and obtain $A_2^{\J_1 \cup \J_2} \subsetneq A_2^{\I_{\Pmc_1 \cup \Pmc_2}}$ and for all $B \prec A_2$, $B^{\J_1 \cup \J_2} = B^{\I_{\Pmc_1 \cup \Pmc_2}}$.
			%\item Otherwise we have $A_1^{\J_1 \cup \J_2} \subsetneq A_1^{\I_{\Pmc_1 \cup \Pmc_2}}$ and for all $B \prec A_1$, $B^{\J_1 \cup \J_2} = B^{\I_{\Pmc_1 \cup \Pmc_2}}$ and we are done.
		\end{itemize}
	\end{enumerate}
	Overall, this proves $\J_1 \cup \J_2 <_\CP \I_{\Pmc_1 \cup \Pmc_2}$ as desired.
\end{proof}

We are now ready to properly prove Lemma~\ref{lemma-criteria-combined}.

\begin{proof}[Proof of Lemma~\ref{lemma-criteria-combined}]
	``$1 \Rightarrow 2$''. 
	Assume there exists $\J \models \kb$ s.t.\ $\J <_\CP \I$.
	Based on $\J$, we build a subset $\Pmc \subseteq \domain{\J}$ containing:
	\begin{itemize}
		\item for each role $r$ s.t.\ $r^\J \neq \emptyset$, an element $w_r' \in (\exists r^-)^\J$;
		\item for each $A \in \Msf$ s.t.\ $A^\J \not\subseteq A^\I$, an element $e_A \in B^\J \setminus B^\I$ for some $B \prec A$ (Condition~3 in the definition of $\J <_\CP \I$ ensures existence of such $B$ and $e_A$);
		\item an element $e_\Msf \in A^\J \setminus A^\I$ for some $A \in \Msf$ s.t.\ $A^\J \subsetneq A^\I$ and for all $B \prec A$, $B^\J = B^\I$
		(Condition~4 in the definition of $\J <_\CP \I$ ensures existence of such $A$ and $e_\Msf$).
	\end{itemize}
	Notice $\Pmc$ has size at most $2\sizeof{\tbox} +1$.
	We now build $\J_\Pmc$ as:
	\begin{align*}
		\domain{\J_\Pmc} = \; & \domain{\I_\Pmc}
		\\
		\cstyle{A}^{\J_\Pmc} = \; & \cstyle{A}^{\J} \cap \domain{\J_\Pmc}
		\\
		\rstyle{r}^{\J_\Pmc} = \; & \rstyle{r}^{\J} \cap (\indsof{\abox} \times \indsof{\abox}) 
		\\
		& \cup \{ (e, w_s') \mid e \in (\exists s)^\J, \tbox \models s \incl r \}
		\\
		& \cup \{ (w_s', e) \mid e \in (\exists s)^\J, \tbox \models s \incl r^- \}
	\end{align*}
	It is easily verified that $\J_\Pmc$ is a model of $\kb$, and we now prove $\J_\Pmc <_\CP \I_\Pmc$.
	We check that all four conditions from the definition of $<_\CP$ are satisfied:
	\begin{enumerate}
		\item 
		By definition, we have $\domain{\J_\Pmc} = \domain{\I_\Pmc}$.
		\item 
		Let $A \in \Fsf$. Definitions of $\I_\Pmc$ and $\J_\Pmc$ ensure $A^\I \cap {\domain{\I_\Pmc}} = A^{\I_\Pmc}$ and $A^\J \cap {\domain{\I_\Pmc}} = A^{\J_\Pmc}$.
		From $\J <_\CP \I$, we get $A^{\I} = A^{\J}$, which thus yields $A^{\I_\Pmc} = A^{\J_\Pmc}$.
		\item 
		Let $A \in \Msf$ such that $A^{\J_\Pmc} \not\subseteq A^{\I_\Pmc}$.
		Therefore $A^{\J} \not\subseteq A^{\I}$, and recall we kept in $\Pmc$ an element $e_A \in B^\J \setminus B^\I$ for some $B \prec A$ to belong to $\Pmc$.
		Joint with $B^{\J_\Pmc} \subseteq B^{\I_\Pmc}$ being trivial, $e_A$ additionally witnesses that $B^{\J_\Pmc} \subsetneq B^{\I_\Pmc}$.
		\item
		Recall we kept in $\Pmc$ an element $e_\Msf \in A^\J \setminus A^\I$ for some $A \in \Msf$ s.t.\ $A^\J \subsetneq A^\I$ and for all $B \prec A$, $B^\J = B^\I$.
		It gives immediately that $A^{\J_\Pmc} \subsetneq A^{\I_\Pmc}$ and for all $B \prec A$, $B^{\J_\Pmc} = B^{\I_\Pmc}$.
	\end{enumerate}
	This proves $\J_\Pmc <_\CP \I_\Pmc$.
	It remains to prove that for all $e \in \domain{\I} \setminus \domain{\I_\Pmc}$, there exists $\J_{\Pmc, e} \models \kb$ with $\J_{\Pmc, e} <_\CP \I_{\Pmc \cup \{ e\} }$ and $\J_{\Pmc, e}|_{\domain{\J_\Pmc}} = \J_\Pmc$.
	This is achieved by constructing $\J_{\Pmc, e}$ as $\J_\Pmc$ above, but from $\Pmc \cup \{ e \}$ instead of $\Pmc$.
	Verifying $\J_{\Pmc, e}$ satisfies the required properties is then done in a similar manner, and it is straightforward that $\J_{\Pmc, e}|_{\domain{\J_\Pmc}} = \J_\Pmc$.
	
	``$2 \Rightarrow 1$''. 
	Assume there exist $\Pmc \subseteq \domain{\I}$ with $\sizeof{\Pmc} \leq 2\sizeof{\tbox} + 1$ and $\J_\Pmc \models \kb$ with $\J_\Pmc <_\CP \I_\Pmc$ s.t.\ for all $e \in \domain{\I} \setminus \domain{\I_\Pmc}$, there exists $\J_{\Pmc, e} \models \kb$ with $\J_{\Pmc, e} <_\CP \I_{\Pmc \cup \{ e\} }$ and $\J_{\Pmc, e}|_{\domain{\J_\Pmc}} = \J_\Pmc$.
	Consider such a $\Pmc \subseteq \domain{\I}$, $\J_\Pmc \models \kb$ and $\J_{\Pmc, e}$ for each $e \in \domain{\I} \setminus \domain{\I_\Pmc}$.
	We build:
	\[
	\J = \J_{\Pmc} \, \cup \, \bigcup_{e \in \domain{\I} \setminus \domain{\I_\Pmc}} \J_{\Pmc, e}
	\]
	It is clear $\domain{\J} = \domain{\I}$ and since all $\J_{\Pmc, e}$ agree on the shared domain $\domain{\J_\Pmc}$, we apply Lemma~\ref{lemma-portions-union} to obtain $\J <_\CP \I$.
\end{proof}











%\begin{lemma}
%	\label{lemma-criteria-combined}
%	Let $\I$ be a model of a $\dllitehorn^{\Hmc^-}$ KB $\kb$ and $\CP$ a circumscription pattern.
%	The following two conditions are equivalent:
%	\begin{enumerate}
%		\item $\I \models \circkb$;
%		\item $\I_\Pmc \models \circkb$ for all $\Pmc \subseteq \domain{\I}$ s.t.\ $\sizeof{\Pmc} \leq 2\sizeof{\tbox} + 1$.
%	\end{enumerate} 
%\end{lemma}
%
%\begin{proof}
%	``$1 \Rightarrow 2$''. 
%	Assume $\Imc \models \circkb$.
%	Consider $\Pmc \subseteq \domain{\I}$ s.t.\ $\sizeof{\Pmc} \leq 2\sizeof{\tbox} +1$.
%	We first verify that $\I_\Pmc$ models $\kb$:
%	\begin{itemize}
%		\item $\I_\Pmc$ models $\abox$ as it inherits interpretations of concepts and roles on $\indsof{\abox}$ from $\I$, which is a model of $\abox$.
%		\item Axioms in $\tbox$ with shape $\axtop$, $\axand$, $\axnotright$ or $\axnotleft$ are satisfied since $\I_\Pmc$ inherits interpretations of concept names from $\I$, which is a model of $\tbox$.
%		\item Axioms in $\tbox$ with shape $A \incl \exists r$ are witnessed with an $r$-edge pointing to $w_r$.
%		\item Axioms in $\tbox$ with shape $\exists r \incl A$ are satisfied since every element in $\I_\Pmc$ receiving some $r$-edge already received some in $\I$ (and interpretations of concept names are preserved).
%		\item Role inclusions $r \incl s$ are satisfied on $\indsof{\abox} \times \indsof{\abox}$ from $\I$ being a model of $\tbox$ in the first place, otherwise directly from the definition of $s^{\Imc_\Pmc}$.
%	\end{itemize}
%	It remains to prove $\I_\Pmc$ also complies with $\CP$.
%	By contradiction assume there exists $\J_\Pmc$ a model of $\kb$ with $\J_\Pmc <_\CP \I_\Pmc$.
%	Notice that, for each forced role $r$ in $\I$, there must exists an element $w_r' \in (\exists r^-)^{\J_\Pmc}$ as we kept element $f_r \in \domain{\I_\Pmc}$ and $r$ is a consequence of the fixed predicates on $f_r$ that must have been preserved in $\J_\Pmc$ (see Condition~2 from the definition of $<_\CP$).
%	We assume chosen such an element $w_r'$ per forced role and build an interpretation $\Jmc$:
%	\begin{align*}
%		\domain{\J} = \; & \domain{\I}
%		\\
%		\cstyle{A}^{\J} = \; & \cstyle{A}^{\J_\Pmc} \cup \{ e \in \domain{\I} \setminus \domain{\J_\Pmc} \mid A \in \ftypeinof{\I}{e} \}
%		\\
%		\rstyle{r}^{\J} = \; & \rstyle{r}^{\J_\Pmc} 
%		\cup \left\{ (e, w_s') \; \middle| \begin{array}{l} e \in \domain{\I} \setminus \domain{\J_\Pmc} \\ \exists s \in \ftypeinof{\I}{e}, \tbox \models s \incl r \end{array} \right\}
%		\\
%		& \cup \left\{ (w_s', e) \; \middle| \begin{array}{l} e \in \domain{\I} \setminus \domain{\J_\Pmc} \\ \exists s \in \ftypeinof{\I}{e}, \tbox \models s \incl r^- \end{array} \right\}
%	\end{align*}
%	It is easily verified that $\J$ is a model of $\kb$, and we now prove $\J <_\CP \I$, which will contradict $\I \models \circkb$.
%	We first notice a useful property: for all concept name $A$, we have $A^\J \cap (\domain{\I} \setminus \domain{\I_\Pmc}) \subseteq  A^\I \cap (\domain{\I} \setminus \domain{\I_\Pmc})$ ($\star$).
%	Indeed, if $e \in A^\J \cap (\domain{\I} \setminus \domain{\I_\Pmc})$, then $A \in \ftypeinof{\I}{e}$, and therefore $e \in A^\I$.
%	The converse does not holds in general.
%	We now check that all four conditions from the definition of $<_\CP$ are satisfied:
%	\begin{enumerate}
%		\item 
%		By definition, we have $\domain{\J} = \domain{\I}$.
%		\item 
%		Let $A \in \Fsf$. Definitions of $\I_\Pmc$ and $\J$ ensure $A^\I \cap {\domain{\I_\Pmc}} = A^{\I_\Pmc}$ and $A^\J \cap {\domain{\I_\Pmc}} = A^{\J_\Pmc}$.
%		From $\J_\Pmc <_\CP \I_\Pmc$, we get $A^{\I_\Pmc} = A^{\J_\Pmc}$, which yields $A^\I \cap {\domain{\I_\Pmc}} = A^\J \cap {\domain{\I_\Pmc}}$.
%		For an element $e \in \domain{\I} \setminus \domain{\I_\Pmc}$, we remark: $e \in A^\I$ iff $A \in \ftypeinof{\I}{e}$ iff $e \in A^\J$.
%		Altogether, we obtain $A^\I = A^\J$.
%		\item 
%		Let $A \in \Msf$ such that $A^\J \not\subseteq A^\I$.
%		Let thus $e \in A^\J \setminus A^\I$.
%		Notice $e$ must belong to $\domain{\I_\Pmc}$, as otherwise $\star$ yields $e \in A^\I$.
%		It follows that $e \in A^{\J_\Pmc} \not\subseteq A^{\I_\Pmc}$.
%		Since $\J_\Pmc <_\CP \I_\Pmc$, there exists $B \prec A$ s.t.\ $B^{\J_\Pmc} \subsetneq B^{\I_\Pmc}$.
%		By $\star$, this extends into $B^{\J} \subsetneq B^{\I}$ and we found $B$ as desired.
%		\item
%		From $\J_\Pmc <_\CP \I_\Pmc$, there exists $A \in \Msf$ s.t.\ $A^{\J_\Pmc} \subsetneq A^{\I_\Pmc}$ and for all $B \prec A$, $B^{\J_\Pmc} = B^{\I_\Pmc}$.
%		Joint with $\star$, it follows that $A^{\J} \subsetneq A^{\I}$ and for all $B \prec A$, $B^{\J} \subseteq B^{\I}$.
%		If ever there exists such a $B \prec A$, such that additionally $B^{\J} \subsetneq B^{\I}$, then we select a minimal such $B$ w.r.t.\ $\prec$, which provides the desired minimized concept.
%		Otherwise, $A$ fits.
%	\end{enumerate}
%	This proves $\J <_\CP \I$, contradicting $\I \models \circkb$ as desired.
%	
%	``$2 \Rightarrow 1$''. 
%	Assume $\I_\Pmc \models \circkb$ for all $\Pmc \subseteq \domain{\I}$ s.t.\ $\sizeof{\Pmc} \leq 2\sizeof{\tbox} +1$.
%	By hypothesis, we already have $\I \models \kb$.
%	By contradiction, assume now there exists $\J < \I$.
%	Based on $\J$, we build a subset $\Pmc \subseteq \domain{\J}$ containing:
%	\begin{itemize}
%		\item for each role $r$ s.t.\ $r^\J \neq \emptyset$, an element $w_r' \in (\exists r^-)^\J$;
%		\item for each $A \in \Msf$ s.t.\ $A^\J \not\subseteq A^\I$, an element $e_A \in B^\J \setminus B^\I$ for some $B \prec A$ (Condition~3 in the definition of $\J <_\CP \I$ ensures existence of such $B$ and $e_A$);
%		\item an element $e_\Msf \in A^\J \setminus A^\I$ for some $A \in \Msf$ s.t.\ $A^\J \subsetneq A^\I$ and for all $B \prec A$, $B^\J = B^\I$
%		(Condition~4 in the definition of $\J <_\CP \I$ ensures existence of such $A$ and $e_\Msf$).
%	\end{itemize}
%	Notice $\Pmc$ has size at most $2\sizeof{\tbox} +1$.
%	We now build $\J_\Pmc$ as:
%	\begin{align*}
%		\domain{\J_\Pmc} = \; & \domain{\I_\Pmc}
%		\\
%		\cstyle{A}^{\J_\Pmc} = \; & \cstyle{A}^{\J} \cap \domain{\J_\Pmc}
%		\\
%		\rstyle{r}^{\J_\Pmc} = \; & \rstyle{r}^{\J} \cap (\indsof{\abox} \times \indsof{\abox}) 
%		\\
%		& \cup \{ (e, w_s') \mid e \in (\exists s)^\J, \tbox \models s \incl r \}
%		\\
%		& \cup \{ (w_s', e) \mid e \in (\exists s)^\J, \tbox \models s \incl r^- \}
%	\end{align*}
%%	It remains to verify $\J_\Pmc <_\CP \Imc_\Pmc$.
%	It is easily verified that $\J_\Pmc$ is a model of $\kb$, and we now prove $\J_\Pmc <_\CP \I_\Pmc$, which will contradict $\I_\Pmc \models \circkb$.
%%	We first notice a useful property: for all concept name $A$, we have $A^\J \cap (\domain{\I} \setminus \domain{\I_\Pmc}) \subseteq  A^\I \cap (\domain{\I} \setminus \domain{\I_\Pmc})$ ($\star$).
%%	Indeed, if $e \in A^\J \cap (\domain{\I} \setminus \domain{\I_\Pmc})$, then $A \in \ftypeinof{\I}{e}$, and therefore $e \in A^\I$.
%%	The converse does not holds in general.
%	We now check that all four conditions from the definition of $<_\CP$ are satisfied:
%	\begin{enumerate}
%		\item 
%		By definition, we have $\domain{\J_\Pmc} = \domain{\I_\Pmc}$.
%		\item 
%		Let $A \in \Fsf$. Definitions of $\I_\Pmc$ and $\J_\Pmc$ ensure $A^\I \cap {\domain{\I_\Pmc}} = A^{\I_\Pmc}$ and $A^\J \cap {\domain{\I_\Pmc}} = A^{\J_\Pmc}$.
%		From $\J <_\CP \I$, we get $A^{\I} = A^{\J}$, which thus yields $A^{\I_\Pmc} = A^{\J_\Pmc}$.
%		\item 
%		Let $A \in \Msf$ such that $A^{\J_\Pmc} \not\subseteq A^{\I_\Pmc}$.
%		Therefore $A^{\J} \not\subseteq A^{\I}$, and recall we kept in $\Pmc$ an element $e_A \in B^\J \setminus B^\I$ for some $B \prec A$ to belong to $\Pmc$.
%		Joint with $B^{\J_\Pmc} \subseteq B^{\I_\Pmc}$ being trivial, $e_A$ additionally witnesses that $B^{\J_\Pmc} \subsetneq B^{\I_\Pmc}$.
%		\item
%		Recall we kept in $\Pmc$ an element $e_\Msf \in A^\J \setminus A^\I$ for some $A \in \Msf$ s.t.\ $A^\J \subsetneq A^\I$ and for all $B \prec A$, $B^\J = B^\I$.
%		It gives immediately that $A^{\J_\Pmc} \subsetneq A^{\I_\Pmc}$ and for all $B \prec A$, $B^{\J_\Pmc} = B^{\I_\Pmc}$.
%	\end{enumerate}
%	This proves $\J_\Pmc <_\CP \I_\Pmc$, contradicting $\I_\Pmc \models \circkb$ as desired.
%	
%\end{proof}

==> criteria-data.tex <==
%!TEX root = main.tex

\begin{restatable}{lemma}{lemmacriteriadata}
	\label{lemma-criteria-data}
	Let $\I$ be a model of a $\dllitebool^{\Hmc^-}$ KB $\kb$ and $\CP$ a circumscription pattern.
	The following two conditions are equivalent:
	\begin{enumerate}
		\item $\I \models \circkb$;
		\item $\I_\Pmc \models \Circ(\kb_\Pmc)$ for all $\Pmc \subseteq \domain{\I}$ s.t.\ $\sizeof{\Pmc} \leq 2\sizeof{\tbox} +1$.
	\end{enumerate} 
\end{restatable}

\begin{proof}
	``$1 \Rightarrow 2$''. 
	Assume $\Imc \models \circkb$.
	Consider $\Pmc \subseteq \domain{\I}$ s.t.\ $\sizeof{\Pmc} \leq 2\sizeof{\tbox} +1$.
	We first verify that $\I_\Pmc$ models $\kb_\Pmc$:
	\begin{itemize}
		\item $\I_\Pmc$ models $\abox_\Pmc$ as it inherits interpretations of concepts on $\indsof{\abox'}$ from $\I$, which is a model of $\abox$.
		\item Axioms in $\tbox$ with shape $\axtop$, $\axand$, $\axnotright$ or $\axnotleft$ are satisfied since $\I_\Pmc$ inherits interpretations of concept names from $\I$, which is a model of $\tbox$.
		\item Axioms in $\tbox$ with shape $A \incl \exists r$ are witnessed with an $r$-edge pointing to $w_r$.
		\item Axioms in $\tbox$ with shape $\exists r \incl A$ are satisfied since every element in $\I_\Pmc$ receiving some $r$-edge already received some in $\I$ (and interpretations of concept names are preserved).
		\item Role inclusions $r \incl s$ are satisfied directly from the definition of $s^{\Imc_\Pmc}$.
	\end{itemize}
	It remains to prove that $\I_\Pmc$ also complies with $\CP$.
	Assume to the contrary that there exists a model $\J_\Pmc$ of $\kb_\Pmc$ with $\J_\Pmc <_\CP \I_\Pmc$.
	Notice that, for each role $r$ s.t.\ $r^{\J_\Pmc} \neq \emptyset$, there must be an element $w_r' \in (\exists r^-)^{\J_\Pmc}$.
	We can chose such an element $w_r'$ for each such role $r$, and build the following interpretation $\J$:
	\begin{align*}
		\domain{\J} = \; & \domain{\I}
		\\
		\cstyle{A}^{\J} = \; & \cstyle{A}^{\J_\Pmc} \cup \{ e \in \domain{\I} \setminus \domain{\J_\Pmc} \mid \refof{e} \in A^{\J_\Pmc} \}
		\\
		\rstyle{r}^{\J} = \; & \{ (a, b) \mid \kb \models r(a, b) \} \\
		&
		\cup \{ (e, w_s') \mid \refof{e} \in (\exists s)^{\J_\Pmc}, \tbox \models s \incl r \}
		\\
		& \cup \{ (w_s', e) \mid \refof{e} \in (\exists s)^{\J_\Pmc}, \tbox \models s \incl r^- \}
	\end{align*}
	It is easily verified that $\J$ is a model of $\kb$
	{\color{red}(Quentin: Maybe I should elaborate? This is where we rely on $\abox_\Pmc$ and ABox-types.)}, 
	\textcolor{blue}{Robin: I think maybe for axioms of the form $A \sqsubseteq \exists r$ and $\exists r \sqsubseteq A$; the others are obvious.}
	and we now prove $\J <_\CP \I$, which will contradict $\I \models \circkb$.
	It suffices to prove that for each concept name $A$ and $\odot \in \{\subseteq, \supseteq\}$, we have $A^{\J} \odot A^\Imc$ iff $A^{\Jmc_\Pmc} \odot A^{\I_\Pmc}$.
	Let $A$ be a concept name.
	%
	We prove the claim for $\odot =\; \subseteq$ only; for $\odot =\; \supseteq$, the arguments are similar.
	
	``$\Rightarrow$''.
	%
	Let $A^{\J} \subseteq A^\I$ and $d \in A^{\J_\Pmc}$.
	In particular, $d \in A^{\J}$ by definition of $A^{\J}$.
	Thus, by hypothesis, $d \in A^{\I}$, and since $d \in \domain{\J_\Pmc} = \domain{\I_\Pmc}$ we obtain $d \in A^{\I_\Pmc}$ by definition of $A^{\I_\Pmc}$.
	
	``$\Leftarrow$''.
	%
	Let $A^{\J_\Pmc} \subseteq A^{\I_\Pmc}$ and $d \in A^{\J}$; we need to show $d \in A^{\I}$.
	If $d \in \domain{\Jmc_\Pmc}$, then it is straightforward.
	Otherwise, we know that $\refof{d} \in A^{\J_\Pmc}$ by definition of $A^{\J}$.
	Therefore $\refof{d} \in A^{\I_\Pmc}$ by hypothesis, that is $A \in \typeinof{\I}{\refof{d}}$.
	Since $d$ and $\refof{d}$ have same type, it yields $A \in \typeinof{\I}{d}$, that is $d \in A^{\I}$.
	
	

	
	``$2 \Rightarrow 1$''. 
%	{\color{red} (Quentin: Spoiler alert, this is the very same proof as in Lemma~\ref{lemma-criteria-combined}.)}
	Assume $\I_\Pmc \models \Circ(\kb_\Pmc)$ for all $\Pmc \subseteq \domain{\I}$ s.t.\ $\sizeof{\Pmc} \leq 2\sizeof{\tbox} +1$.
	By hypothesis, we already have $\I \models \kb$.
	By contradiction, assume now there exists $\J < \I$.
	Based on $\J$, we build a subset $\Pmc \subseteq \domain{\J}$ containing:
	\begin{itemize}
		\item for each role $r$ s.t.\ $r^\J \neq \emptyset$, an element $w_r' \in (\exists r^-)^\J$;
		\item for each $A \in \Msf$ s.t.\ $A^\J \not\subseteq A^\I$, an element $e_A \in B^\J \setminus B^\I$ for some $B \prec A$ (Condition~3 in the definition of $\J <_\CP \I$ ensures existence of such $B$ and $e_A$);
		\item an element $e_\Msf \in A^\J \setminus A^\I$ for some $A \in \Msf$ s.t.\ $A^\J \subsetneq A^\I$ and for all $B \prec A$, $B^\J = B^\I$
		(Condition~4 in the definition of $<_\CP$ ensures the existence of such $A$ and $e_\Msf$).
	\end{itemize}
	Notice $\Pmc$ has size at most $2\sizeof{\tbox} +1$.
	We now build $\J_\Pmc$ as:
	\begin{align*}
		\domain{\J_\Pmc} = \; & \domain{\I_\Pmc}
		\\
		\cstyle{A}^{\J_\Pmc} = \; & \cstyle{A}^{\J} \cap \domain{\J_\Pmc}
		\\
		\rstyle{r}^{\J_\Pmc} = \; & \{ (e, w_s') \mid e \in (\exists s)^\J  \cap \domain{\I_\Pmc}, \tbox \models s \incl r \}
		\\
		& \cup \{ (w_s', e) \mid e \in (\exists s)^\J  \cap \domain{\I_\Pmc}, \tbox \models s \incl r^- \}
	\end{align*}
%	It remains to verify $\J_\Pmc <_\CP \Imc_\Pmc$.
	It is easily verified that $\J_\Pmc$ is a model of $\kb_\Pmc$, and we now prove $\J_\Pmc <_\CP \I_\Pmc$, which will contradict $\I_\Pmc \models \Circ(\kb_\Pmc)$.
	%	We first notice a useful property: for all concept name $A$, we have $A^\J \cap (\domain{\I} \setminus \domain{\I_\Pmc}) \subseteq  A^\I \cap (\domain{\I} \setminus \domain{\I_\Pmc})$ ($\star$).
	%	Indeed, if $e \in A^\J \cap (\domain{\I} \setminus \domain{\I_\Pmc})$, then $A \in \ftypeinof{\I}{e}$, and therefore $e \in A^\I$.
	%	The converse does not holds in general.
	We now check that all four conditions from the definition of $<_\CP$ are satisfied:
	\begin{enumerate}
		\item 
		By definition, we have $\domain{\J_\Pmc} = \domain{\I_\Pmc}$.
		\item 
		Let $A \in \Fsf$. Definitions of $\I_\Pmc$ and $\J_\Pmc$ ensure $A^\I \cap {\domain{\I_\Pmc}} = A^{\I_\Pmc}$ and $A^\J \cap {\domain{\I_\Pmc}} = A^{\J_\Pmc}$.
		From $\J <_\CP \I$, we get $A^{\I} = A^{\J}$, which thus yields $A^{\I_\Pmc} = A^{\J_\Pmc}$.
		\item 
		Let $A \in \Msf$ such that $A^{\J_\Pmc} \not\subseteq A^{\I_\Pmc}$.
		Therefore $A^{\J} \not\subseteq A^{\I}$, and recall we kept in $\Pmc$ an element $e_A \in B^\J \setminus B^\I$ for some $B \prec A$ to belong to $\Pmc$.
		Joint with $B^{\J_\Pmc} \subseteq B^{\I_\Pmc}$ being trivial, $e_A$ additionally witnesses that $B^{\J_\Pmc} \subsetneq B^{\I_\Pmc}$.
		\item
		Recall we kept in $\Pmc$ an element $e_\Msf \in A^\J \setminus A^\I$ for some $A \in \Msf$ s.t.\ $A^\J \subsetneq A^\I$ and for all $B \prec A$, $B^\J = B^\I$.
		It gives immediately that $A^{\J_\Pmc} \subsetneq A^{\I_\Pmc}$ and for all $B \prec A$, $B^{\J_\Pmc} = B^{\I_\Pmc}$.
	\end{enumerate}
	This proves $\J_\Pmc <_\CP \I_\Pmc$, contradicting $\I_\Pmc \models \Circ(\kb_\Pmc)$ as desired.
	
\end{proof}

==> def-core.tex <==
%!TEX root = main.tex
%
%
\begin{definition}
	\label{def-core}
%
Let $\I$ be an interpretation.
Let $\mn{TP}_{\mn{core}}(\Imc)$ be the subset of $\mn{TP}(\Imc)$
that contains all types $t$ such that
%
$$
|\{ d \in \Delta^\Imc \setminus \mn{ind}(\Amc) \mid \mn{tp}_\Imc(d)=t \}| < |\mn{TP}(\Tmc)|
$$
%
and let $\mn{TP}_{\overline{\mn{core}}}(\Imc)=\mn{TP}(\Imc) \setminus \mn{TP}_{\mn{core}}(\Imc)$.
%
We define $$\Delta^\Imc_\mn{core} = \{  d \in \Delta^\Imc \mid \mn{tp}_\Imc(d) \in \mn{TP}_{\mn{core}}(\Imc) \}.$$
\end{definition}%

==> def-interlacing.tex <==
%!TEX root= main.tex
%
\begin{definition}
	\label{def-interlacing}
The interlace function $\interlace$ of $\I$ is:
\[
\begin{array}{cccl}
\interlace : &
\exexof{\I} 	& \rightarrow 	& \coredomainof{\I} \uplus (\exexof{\I} \setminus \coredomainof{\I})
\\[3pt] &
w 							& \mapsto		& 	\left\{ \begin{array}{ll}
													\exextomodof{w}
														& \textrm{if } \exextomodof{w} \in \coredomainof{\I}
													\\
													w 
														& \textrm{otherwise}
												\end{array} \right.
\end{array}
\]
The \emph{interlacing} $\interlacingof{\I}$ of $\I$ is the interpretation whose domain is $\domain{\interlacingof{\I}} := \interlaceof{\exexof{\I}}$ and which interprets concept and role names as follows:
\begin{align*}
	\cstyle{A}^{\interlacingof{\I}} \, = \, &
	\{ \interlaceof{u} \mid u \in \exexof{\I}, \exextomodof{u} \in \cstyle{A}^\I \}
	\\
	\rolestyle{P}^{\interlacingof{\I}} \, = \, &
	\{ (\indstyle{a}, \indstyle{b}) \mid \indstyle{a}, \indstyle{b} \in \indsof{\abox}, \kb \models \roleassertion{P}{a}{b} \}
	%\tag{\ensuremath{\triangledown_0}}\label{case:rind}
	\\ & \cup \, 
	\{ (\interlaceof{u}, \interlaceof{u \cdot \rolestyle{R}.\cstyle{B}}) \mid \tbox \models \axiom{\rstyle R}{\rstyle P} \} 
	%\tag{\ensuremath{\triangledown_+}}\label{case:rplus}
	\\ & \cup \,
	\{ (\interlaceof{u \cdot \rolestyle{R}.\cstyle{B}}, \interlaceof{u}) \mid \tbox \models \axiom{\rstyle{R^-}}{\rstyle P} \} 
	%\tag{\ensuremath{\triangledown_-}}\label{case:rminus}
\end{align*}
\end{definition}

==> def-type.tex <==
%!TEX root = main.tex


\begin{definition}
	\label{def-type}
	A \emph{type for $\Tmc$} is a subset
	$t \subseteq \cnames(\tbox)$ s.t.\ there is a model \Imc of
	$\Circ(\Kmc)$ and a $d \in \Delta^\Imc$ with
	$t = \typeinof{\I}{d} \coloneqq \{ \cstyle{C} \in \cnames(\tbox) \mid d \in
	\cstyle{C}^\Imc \}$.
	%
	The set of all types for $\Tmc$ is denoted $\types(\tbox)$.
	If $\I$ is an interpretation, $\types(\I)$ denotes the set of types $t \in \types(\tbox)$ s.t.\ $\typeinof{\I}{d} = t$ for some $d \in \domain{\Imc}$.
\end{definition}


\iffalse
\begin{definition}
	\label{def-type}
	The set of concepts that occur in $\Tmc$, closed under subconcept and single negation, is denoted $\mn{cl}(\Tmc)$.
	%
	A \emph{type for $\Tmc$} is a subset
	$t \subseteq \mn{cl}(\Tmc)$ s.t.\ there is a model \Imc of
	$\Circ(\Kmc)$ and a $d \in \Delta^\Imc$ with
	$t=\mn{tp}_\Imc(d) \coloneqq \{ C \in \mn{cl}(\Tmc) \mid d \in
	C^\Imc \}$.
	%
	The set of all types for $\Tmc$ is denoted $\mn{TP}(\Tmc)$.
	If $\I$ is an interpretation, we use $\mn{TP}(\Imc)$ to denote the set of types $t \in \mn{TP}(\Tmc)$ s.t.\ $\mn{tp}_\Imc(d)=t$ for some $d \in \Delta^\Imc$.
\end{definition}
\fi

==> instance-lower-el.tex <==

%
\begin{theorem}
	\label{thm-combined-lower-el-aq}
  AQ evaluation on circumscribed \EL KBs is $\coNExpTime^\NPclass$-hard w.r.t.\ combined
  complexity.
        %
  This holds even without
  fixed concept names and with an empty preference order.
\end{theorem}
%
To prove this result, we provide a polynomial time reduction from AQ
evaluation on circumscribed \ALC KBs, which is known to be
$\coNExpTime^\NPclass$-hard w.r.t.\ combined complexity even without
fixed concept names and with an empty preference relation \cite{Bonatti2009}.


Let $\mn{Circ}_\CP(\Kmc)$ be a circumscribed \ALC KB, with $\Kmc=(\Tmc,\Amc)$, $A_0$ an AQ, and $a_0 \in \Ind(\Amc)$.  We construct a
        circumscribed $\EL$ KB $\mn{Circ}_\CP(\Kmc')$, with
        $\Kmc'=(\Tmc',\Amc')$, such that
        $\mn{Circ}_\CP(\Kmc) \models A_0(a_0)$ iff $\mn{Circ}_\CP(\Kmc') \models A_0(a_0)$.

        With $\ELU_\bot$, we mean the extension of \EL with disjunction and $\bot$.
        It is well-known that every \ALC TBox $\Tmc$ can be rewritten in polynomial time into an $\ELU_\bot$ TBox $\Tmc^\ast$ that is a conservative extension of $\Tmc$ in the sense that every
        model of $\Tmc^\ast$ is a model of $\Tmc$ and every model of $\Tmc$ can be extended to a model of $\Tmc^\ast$ by interpreting the fresh concept and role names in $\Tmc^\ast$ \cite{DBLP:conf/ijcai/BaaderBL05}. It follows that $\mn{Circ}_\CP(\Kmc)
        \models A_0(a_0)$ iff $\mn{Circ}_\CP(\Tmc^\ast,\Amc) \models A_0(a_0)$, assuming that all the fresh concept names in $\Tmc^\ast$ vary in \CP.
        In the following, we recall the rewriting, which proceeds in three steps:
        %
        \begin{enumerate}

        \item \emph{Remove value restrictions} by replacing every subconcept
          $\forall r . C$ with $\neg \exists r . \neg C$.

        \item \emph{Remove negation of compound concepts} by replacing
          every subconcept $\neg C$, with $C$ compound, by $\neg X$
          where $X$ is a fresh concept name, and adding the CIs
          %
          $$
             C \sqsubseteq X \qquad X \sqsubseteq C.
          $$
          
        \item \emph{Remove negation entirely} by replacing every subconcept
          $\neg A$ with the fresh concept name $\overline A$, and adding
          the CIs
          %
          $$
             \top  \sqsubseteq A \sqcup \overline{A} \qquad
             A \sqcap \overline{A} \sqsubseteq \bot.
          $$

        \end{enumerate}
        %
        We may thus assume w.l.o.g.\ that the TBox \Tmc in the given circumscribed KB
        \Kmc is
        an $\ELU_\bot$ TBox. We may further assume that disjunction occurs in \Tmc
        only in CIs of the form
        %
        $$
           B \sqsubseteq B_1 \sqcup B_2
        $$
        %
        where $B,B_1,B_2$ are concept names, by replacing every disjunction
        $C_1 \sqcup C_2$ with a fresh concept name $X$ and adding the CIs
        %
        $$
        \begin{array}{r@{\;}c@{\;}lcr@{\;}c@{\;}lcr@{\;}c@{\;}l}
          X &\sqsubseteq& Y_1 \sqcup Y_2 && Y_1 &\sqsubseteq& X &&
                                                                   Y_2 &\sqsubseteq& X \\[1mm]
          C_i & \sqsubseteq & Y_i && Y_i &\sqsubseteq& C_i && \text{for } i \in \{1,2\}
        \end{array}
        $$
        %
        where also $Y_1,Y_2$ are fresh concept names. Finally, we may assume
        that \Tmc contains only a single CI $B \sqsubseteq B_1 \sqcup B_2$
        by replacing every such CI with
        %
        $$
        B \sqsubseteq \exists r_{B_1,B_2} . D \quad
        \exists r_{B_1,B_2} . D_1 \sqsubseteq B_1 \qquad 
        \exists r_{B_1,B_2} . D_2 \sqsubseteq B_2 
        $$
        %
        where $r_{B_1,B_2}$ is a fresh role name and $D,D_1,D_2$ are fresh concept names,
        and adding the CI
        %
        $$
            D \sqsubseteq D_1 \sqcup D_2.
        $$
        %
        We may clearly also assume that $\bot$ occurs in \Tmc only in the form
        $C \sqsubseteq \bot$ with $C$ an \EL-concept.
        Note that the TBoxes resulting from these transformations are conservative
        extensions of the original ones. In \CP, all of the freshly introduced
        concept names are varying.

        \smallskip
        We are now ready for the actual reduction, which combines ideas from
        the proofs of Theorems~\ref{thm:combined-lower-el} and~\ref{thm-data-lower-el}. To construct the TBox $\Tmc'$,
        We start with  relativized versions  of the \EL-CIs in \Tmc. 
        For an \EL
        concept $C$,
        inductively define the concept $C_\X$ as follows:
        %
        \begin{align*}
                A_\X    & \coloneqq \X \sqcap A & (\exists r.D)_\X & \coloneqq \X \sqcap \exists r.D_\X \\
                \top_\X & \coloneqq \X          & (D \sqcap D')_\X & \coloneqq D_\X \sqcap D'_\X
        \end{align*}
        %
        We then include in $\Tmc'$ all CIs 
        % 
        \begin{align}
                C_\X \sqsubseteq D_\X 
        \end{align}
        %
        such that $C \sqsubseteq D \in \Tmc$ is neither the unique disjunctive
        CI $B \sqsubseteq B_1 \sqcup B_2$
        nor of the form $C \sqsubseteq \bot$. To construct the ABox $\Amc'$,
        we start with the extension of \Amc by
        %
        \begin{align}
          X(a) \quad \text{ for all } a \in \Ind(\Amc).
          \label{Xmarking}
        \end{align}

        Of course, we need to compensate the removal of the mentioned CIs.
        To simulate the disjunctive CI $B \sqsubseteq B_1 \sqcup B_2$, we
        extend $\Tmc'$ with
        %
        \begin{align}
        B &\sqsubseteq \exists r_D . (D \sqcap \mn{Pos}) \qquad
            \exists r_D . D_1 \sqsubseteq B_1
            \label{blablaone}
          \\
                                                             B &\sqsubseteq \exists r_D . (D \sqcap \mn{Neg}) 
                                                          \qquad
                                                                 \exists r_D . D_2 \sqsubseteq B_2
                                                                 \label{blablatwo}
        \end{align}
        % \begin{array}{rclcrcl}
        % B &\sqsubseteq& \exists r_D . (D \sqcap \mn{Pos}) &&
        % \exists r_D . D_1 &\sqsubseteq& B_1 
        %   \\[1mm]
        %                                                      B &\sqsubseteq& \exists r_D . (D \sqcap \mn{Neg}) 
        %                                                   &&
        %                                                      \exists r_D . D_2 &\sqsubseteq& B_2
        % \end{array}
%        $$
        %
        where $D,D_1,D_2,\mn{Pos}$, and $\mn{Neg}$ are fresh concept names and $r_D$ is a fresh role name.
        We update \CP so that $D$ is minimized. We further extend \Amc with the
        assertions
        %
\begin{align}
	D(d_1^+) 	& & D(d_1^-) 	& &D(d_2^+) 	& & D(d_2^-) \\
	D_1(d_1^+) 	& & D_1(d_1^-) 	& &
                                                            D_2(d_2^+)
                                                                                & & D_2(d_2^-)  	 \\
	\mn{Pos}(d_1^+) 	& & \mn{Neg}(d_1^-) 	& & \mn{Pos}(d_2^+) 	& &\mn{Neg}(d_2^-).
\end{align}
%
where $d^+_1,d^-_1,d^+_2,d^-_2$ are fresh individuals. Note that these individuals are \emph{not} marked with $X$, exempting them from $\Tmc$ is why the CIs from \Tmc are relativized in $\Tmc'$. Note that the way we simulate disjunction is similar to the way in which we choose truth values in the proof of Theorem~\ref{thm-data-lower-el},
and also the reason for using a positive and a negative witness is the same.
We need to make sure that the positive and negative witness are distinct,
which is achieved by otherwise making the query true.
%
% Further introduce fresh role names $\mn{freeze}$ %, $\mn{freeze}_{D_2}$,
% and \mn{checks} and for every $a \in \Ind(\Amc)$, fresh individuals $a_{D_1}$ and $a_{D_2}$.  Then extend $\Amc'$ with
% %
% $$
% \begin{array}{rcl}
%   \exists \mn{freeze}. D_1 \sqsubseteq D
% \end{array}
% $$
To this end, we introduce a fresh role name $u$ and fresh concept
names $G, A_0'$. We update \CP so that $G$ is minimized and extend $\Tmc'$ with:%
%
\begin{align}
	\mn{Pos} \sqcap \mn{Neg} & \sqsubseteq \exists u.(G \sqcap A'_0)
	\label{barlabel} \\
	A_0 &\sqsubseteq A'_0
	\label{barbarlabel}
\end{align}
%
We add
$
G(a_0)
$
to $\Amc'$ and the new query is $A'_0$.

For the compensation of the removal of the CIs \mbox{$C \sqsubseteq \bot$}, we consider another fresh concept name $M$ and update \CP so that $M$ is minimized. We further extend $\Tmc'$ with
%
%$$
\begin{align}
	C \sqsubseteq M \sqcap \exists u . (G \sqcap A'_0) \quad \text{ for all } C \sqsubseteq \bot \in \Tmc.
	\label{lastone}
\end{align}
So if a concept $C$ with $C \sqsubseteq \bot \in \Tmc$ is
satisfied, then we force the minimized concept name $M$ to be non-empty
and make the (new) query true.

\iffalse
We introduce fresh a role name \mn{check} and extend $\Amc'$ with
%
\begin{align}
  \mn{check}(a_0,a)  \qquad \text{for all } a \in \Ind(\Amc)
  \label{foolabel}
\end{align}
%
and $\Tmc'$ with
%
\begin{align}
\exists \mn{check} . \exists r_D . (\mn{Pos} \sqcap \mn{Neg}) &\sqsubseteq A'_0
  \label{barlabel} \\
  A_0 &\sqsubseteq A'_0
        \label{barbarlabel}
\end{align}
%
where $A'_0$ is a fresh concept name that is the new query.


Now for the compensation of the removal of the CIs \mbox{$C \sqsubseteq \bot$}. Let $u$ be a fresh role name and $G,M$ fresh concept names. We update \CP so that $G,M$ are both minimized and extend $\Tmc'$ with
%
%$$
\begin{align}
  C \sqsubseteq M \sqcap \exists u . (G \sqcap A'_0) \quad \text{ for all } C \sqsubseteq \bot \in \Tmc.
  \label{lastone}
\end{align}
%$$
%
and add 
%
$
G(a_0)
$
to $\Amc'$. So if a concept $C$ with $C \sqsubseteq \bot \in \Tmc$ is
satisfied, then we force the minimized concept name $M$ to be non-empty
and make the (new) query true.
\fi
Let $\CP'$ be the extended circumscription pattern.
%
It remains to establish correctness of the reduction.
        %
        \\[2mm]
        {\bf Claim.} 
                $\Circ(\Kmc) \models A_0(a_0)$ iff $\Circ(\Kmc') \models A'_0(a_0)$.
                \\[2mm]
                To prepare for the proof of the claim, we first observe that every
                model \Imc of \Kmc gives rise to a model $\Imc'$ of $\Kmc'$
                in a natural way. More precisely, we set $\Delta^{\Imc'} = \Delta^\Imc \uplus \{ d^+_1,d^-_1,d^+_2,d^-_2\}$,
                define the extension of all concept and role names that occur in \Kmc
                exactly as in \Imc, and interpret the fresh concept and role names as
                follows:
                %
                $$
                \begin{array}{rcl}
                  X^{\Imc'} &=& \Delta^\Imc \\[1mm]
                  D^{\Imc'} &=& \{ d^+_1,d^-_1,d^+_2,d^-_2\} \\[1mm]
                  D_i^{\Imc'}&=& \{d^+_i, d^-_i \} \text{ for } i \in \{1,2\} \\[1mm]
                  \mn{Pos}^{\Imc'} &=& \{ d^+_1,d^+_2 \}\\[1mm]
                  \mn{Neg}^{\Imc'} &=& \{ d^-_1,d^-_2 \}\\[1mm]
                  r_D^{\Imc'} &=& \{ (d,d^+_1),(d,d^-_1) \mid d \in (B \sqcap B_1)^\Imc \} \, \cup \\[1mm]
                         && \{ (d,d^+_2),(d,d^-_2) \mid d \in (B \sqcap B_2)^\Imc \} \\[0.5mm]
                  \mn{check}^{\Imc'} &=& \{ (a_0,a) \mid a \in \mn{ind}(\Amc) \\[1mm]
                  {A'_0}^{\Imc'} &=& A_0^\Imc \\[1mm]
                  u^{\Imc'} &=& \emptyset \\[1mm]
                  M^{\Imc'} &=& \emptyset \\[1mm]
                  G^{\Imc'} &=& \{ a_0 \}\\[1mm]
                \end{array}
                $$
                It is easily checked that ${\Imc'}$ is indeed a model of $\Kmc'$.
%
        Now for the actual proof of the claim
        \smallskip
                
        ``$\Leftarrow$''.  Assume that $\Circ(\Kmc) \not\models A_0(a_0)$. Then there is a model \Imc of \Kmc that is minimal w.r.t.\ \CP and satisfies $\Imc\not\models A_0(a_0)$. Let ${\Imc'}$ be the corresponding model of $\Kmc'$ defined above. We
                clearly have
            ${\Imc'} \not\models A'_0(a_0)$. To show that $\Circ(\Kmc') \not\models A'_0(a_0)$, it thus remains to show that $\Imc'$ is minimal w.r.t.\ $\CP'$.

            Assume to the contrary that there is a model $\Jmc' <_{\CP'} \Imc'$ of~$\Kmc'$.
            As $\Imc'$ interprets $D,M,$ and $G$ minimally among all models of $\Kmc'$,
            we must have $D^{\Jmc'} = D^{\Imc'} = \{ d^+_1,d^-_1,d^+_2,d^-_2\}$, $M^{\Jmc'} = \emptyset$, and
            $G^{\Jmc'} = G^{\Imc'} = \{ a_0 \}$. We show that the restriction $\Jmc$
            of $\Jmc'$ to domain $X^{\Jmc'}$ is a model
            of $\Kmc$. Moreover, $\Jmc' <_{\CP'} \Imc'$, $D^{\Jmc'} = D^{\Imc'}$, $M^{\Jmc'} = M^{\Imc'}$, and
            $G^{\Jmc'} = G^{\Imc'}$ imply $\Jmc <_\CP \Imc$, which then yields a contradiction against the minimality of \Imc.

            Based on the facts that $\Jmc'$ is a model of $\Amc'$, $\Ind(\Amc) \subseteq X^{\Jmc'}$ due to (\ref{Xmarking}), and $\Amc \subseteq \Amc'$, it is clear that $\Jmc$ is a model of \Amc. Moreover, since $\Jmc'$ is a model of $\Tmc'$, by
            construction of $\Jmc$ it is easy to see that $\Jmc$ satisfies all CIs in \Tmc
            with the possible
            exceptions of the disjunctive CI $B \sqsubseteq B_1 \sqcup B_2$ and the
            CIs of the form $C \sqsubseteq \bot$. The former, however, is satisfied due to
            CIs~(\ref{blablaone}) and~(\ref{blablatwo}) and since
            $D^{\Jmc'} = \{ d^+_1,d^-_1,d^+_2,d^-_2\}$. And the latter is satisfied
            due to the CIs~(\ref{lastone}) and since $M^{\Jmc'}=\emptyset$.
            
            %
            % Call an element $d \in \Delta^{\Jmc'}$ \emph{reachable} if there is a sequence
            % $d_0,r_0,d_1,r_1,\dots,r_{n-1},d_n$ such that $d_0 \in \Ind(\Amc)$, $(d_i,d_{i+1}) \in r^{\Jmc'}$ for $0 \leq i < n$, and $d_n=d$. We may assume w.l.o.g.\ that domain
            % elements in $\Jmc'$ that are not reachable do not occur in the extension of
            % concept and role names. NOT TRUE!!!!

\smallskip
            
``$\Rightarrow$''.  Assume that $\Circ(\Kmc') \not\models A'_0(a_0)$. Then there is a model $\Imc'$ of $\Kmc'$ that is minimal w.r.t.\ $\CP'$ and satisfies $\Imc'\not\models A'_0(a_0)$. 
We first argue that $G^{\Imc'}=\{ a_0 \}$ as, otherwise, we can find a model $\Jmc' <_{\CP'} \Imc'$ of~$\Kmc'$, contradicting the minimality of $\Imc'$.
We have $G^{\Imc'} \subseteq \{ a_0 \}$ since $\Imc'$ is a model of $\Amc'$. Assume to the contrary of what we want to show that the converse fails.  Then we construct $\Jmc'$ by modifying $\Imc'$ as follows:
%
\begin{itemize}
	
	\item set $G^{\Jmc'} = \{ a_0 \}$;
	
	\item add $a_0$ to ${A'_0}^{\Jmc'}$;
	
	\item reroute $u$ as $u^{\Jmc'} = \{ (e, a_0) \mid e \in (\exists u)^{\Imc'} \}$.
	
\end{itemize}
%
It is easy to see that, indeed, $\Jmc'$ is still a model of $\Kmc'$ and $\Jmc' <_{\CP'} \Imc'$.

Since $\I'$ satisfies CIs~(\ref{blablaone}) and~(\ref{blablatwo}), for every $e \in B^{\I'}$ we can choose two elements $e^+ \in (D \sqcap \mn{Pos})^{\Imc'}$ and $e^- \in (D \sqcap \mn{Neg})^{\Imc'}$ such that $(e,e^+), (e, e^-) \in r_D^{\I'}$. If $e^+ = e^-$ for some $e$, then by~(\ref{barlabel}) and $G^{\Imc'} = \{ a_0\}$, we have $a_0 \in A_0^{\Imc'}$,
which is impossible since $\Imc'\not\models A'_0(a_0)$. Thus  $e^+ \neq e^-$ for
all $e$.

We next argue that the following conditions are satisfied:
%
\begin{enumerate}

\item for all $e \in B^{\Imc'}$:
$\{ e^+, e^- \} \cap \{ d^+_1, d^-_1,d^+_2, d^-_2\}
\neq \emptyset$;

%\item $G^{\Imc'}=\{ a_0 \}$;

\item $M^{\Imc'}=\emptyset$.

\end{enumerate}
%
If, in fact, any of the above conditions is violated, then we can again find a model $\Jmc' <_{\CP'} \Imc'$ of~$\Kmc'$, contradicting the minimality of $\Imc'$.
We start with Condition~1.

Assume to the contrary that for some $e \in B^{\Imc'}$, $e^+, e^- \notin \{ d^+_1, d^-_1,d^+_2, d^-_2\}$.  Then we construct
$\Jmc'$ by modifying \Jmc as follows:
%
\begin{itemize}

\item remove $e^-$ from $D^{\Jmc'}$;

\item add $e^+$ to $\mn{Neg}^{\Jmc'}$;
  
\item add $a_0$ to ${A'_0}^{\Jmc'}$;

\item {\color{red} add $(e^+, a_0)$ to $u^{\Jmc'}$.}

\end{itemize}
%
It is easy to see that, indeed, $\Jmc'$ is still a model of $\Kmc'$ and $\Jmc' <_{\CP'} \Imc'$.  

%Next for Condition~2. We have $G^{\Imc'} \subseteq \{ a_0 \}$ since $\Imc'$ is a model of $\Amc'$. Assume to the contrary of what we want to show that the converse fails.  Then we construct $\Jmc'$ by modifying \Jmc as follows:
%%
%\begin{itemize}
%
%\item set $G^{\Jmc'} = \{ a_0 \}$;
%
%\item add $a_0$ to ${A'_0}^{\Jmc'}$. 
%
%\end{itemize}
%%
%It is easy to see that, indeed, $\Jmc'$ is still a model of $\Kmc'$ and $\Jmc' <_{\CP'} \Imc'$.  

In the case of Condition~2, we can construct the model $\Jmc'$ simply as \Jmc modified by setting $M^{\Jmc'}=\emptyset$. The resulting $\Jmc'$ is a model of $\Kmc'$.  The only potentially problematic item are the CIs~(\ref{lastone}). But since $\Imc'\not\models A'_0(a_0)$ and $G^{\Imc'}=\{a_0\}$, we can infer from~(\ref{lastone}) that $C^{\Imc'} = \emptyset$ for all $C \sqsubseteq \bot \in \Tmc$, and thus the same holds for $\Jmc'$. Consequently, the CIs~(\ref{lastone}) are never triggered in $\Jmc'$ and it is safe to set $M^{\Jmc'}=\emptyset$.

Let $\Imc$ be the restriction of $\Imc'$ to $X^{\Imc'}$. It can be verified that $\Imc'$ is a model of \Amc and that it satisfies all CIs in \Tmc
with the possible
            exceptions of the disjunctive CI $B \sqsubseteq B_1 \sqcup B_2$ and the
            CIs of the form $C \sqsubseteq \bot$. The former, however, is satisfied by
            Condition~1 and due to
            CIs~(\ref{blablaone}) and~(\ref{blablatwo}). And the latter is satisfied
            by Condition~2 and 
            due to CI~(\ref{lastone}).

            Since $\Imc' \not\models A'_0(a_0)$ and by (\ref{barbarlabel}), we have $\Imc \not\models A_0(a_0)$. To show that $\Kmc \not\models A_0(a_0)$, it thus remains
            to show that $\Imc$ is minimal w.r.t.\ $<_\CP$.
            Assume to the contrary that there is a model $\Jmc <_\CP \Imc$ of $\Kmc$
            and let $\Jmc'$ be the corresponding model of $\Kmc'$ constructed at
            the beginning of the correctness proof. Since $\Jmc'$ interprets
            the minimized concept names $D$, $M$, and $G$ in a minimal way among
            the models of $\Kmc'$, it follows from $\Jmc <_\CP \Imc$ that
            $\Jmc' <_{\CP'} \Imc'$, in contradiction to $\Imc'$ being minimal.




==> lem-interlacing-is-countermodel.tex <==
%!TEX root = main.tex
%
%
\begin{lemma}
	\label{lem_interlacing_is_countermodel}
	If $\I$ is countermodel for $\Query$ over $\circkb$, then its interlacing $\interlacing$ also is.
\end{lemma}

\begin{proof}
	Let $\I$ be a countermodel for $\Query$ over $\circkb$.
	Verifying that $\interlacing$ is a model of $\kb$ with no match for $\Query$ follows the same arguments as in \cite{maniere:thesis}, and can be found in the appendix.
	It is worth mentioning that $\interlacing$ embeds in $\I$ by applying $f$ on $\exexof{\I} \cap \domain{\interlacing}$ (elements that were not already put back in place by $\interlace$), which proves that $\interlacing$ has no match for $\Query$.
	%
	It remains to prove that $\interlacing$ complies with $\CP$.
	We rely on Lemma~\ref{lem-lemma5}.
	Notice that $\coredomainof{\I} \subseteq \domain{\interlacing}$.
	By definition of concept interpretations, for all $u \in \exexof{\I}$ we have $\typeinof{\I}{\exextomodof{u}} = \typeinof{\interlacing}{\interlaceof{u}}$.
	%
	Let $e \in \coredomainof{\I}$ and $u \in \exexof{\I}$ such that $\interlaceof{u} = e$.
	By the above remark, we have $\typeinof{\I}{\exextomodof{u}} = \typeinof{\interlacing}{\interlaceof{u}}$.
	Since $\interlaceof{u} \in \coredomainof{\I}$, we have $\exextomodof{u} = e$.
	Therefore $\typeinof{\I}{e} = \typeinof{\interlacing}{e}$.
	Condition~1 of Lemma~\ref{lem-lemma5} is thus satisfied.
	%
	Let now $t \in \typeinof{\interlacing}{\domain{\interlacing} \setminus \coredomainof{\I}}$.
	By definition, there exists $u \in \exexof{\I}$ such that $\typeinof{\interlacing}{\interlaceof{u}} = t$.
	Since $\interlaceof{u} \notin \coredomainof{\I}$, we have $\exextomodof{u} \notin \coredomainof{\I}$.
	Therefore $\typeinof{\I}{\exextomodof{u}} \in \noncoretypesof{\I}$, that is $t = \typeinof{\interlacing}{\interlaceof{u}} = \typeinof{\I}{\exextomodof{u}} \in \noncoretypesof{\I}$.
	%
	Conversely, let $t \in \noncoretypesof{\I}$.
	Recall $\typeinof{\I}{r_t} = t$ and notice $\exextomodof{r_t} = \interlaceof{r_t} = r_t \notin \coredomainof{\I}$.
	Therefore $t \in \typeinof{\interlacing}{\domain{\interlacing} \setminus \coredomainof{\I}}$.
	Condition~2 of Lemma~\ref{lem-lemma5} is thus satisfied as well, which ensures $\interlacing$ is a model of $\circkb$.
	
\end{proof}
		


\begin{toappendix}
	{\vspace{5pt}\noindent\bf Proofs of claims from Lemma~\ref{lem_interlacing_is_countermodel}.}
	\begin{claim}
		\label{claim-interlacing-is-model-of-kb}
		If $\I$ is a model for $\kb$, then its interlacing $\interlacing$ also is.
	\end{claim}
	\begin{proof}
		We start by showing that $\interlacingof{\I}$ is a model, by 
		considering each possible shape of assertions and axioms (recall that $\tbox$ is {in} normal form):
		\todo[inline]{Move pseudo-injectivity as a lemma}
		
		\begin{itemize}
			
			\item[$\conceptassertion{A}{a}$.]
			Since $\I$ is a model, we have $\exextomodof{\istyle{a}} = \istyle{a} \in \rolestyle{A}^\I$.
			Therefore, the definition of $\cstyle{A}^{\interlacingof{\I}}$ gives $\interlaceof{\istyle{a}} = \istyle{a} \in \cstyle{A}^{\interlacingof{\I}}$.
			
			\item[$\roleassertion{P}{a}{b}$.]
			Setting $\rolestyle{P_0} := \rolestyle{P}$ in Case~\ref{case:rind} of the definition of $\rolestyle{P}^{\interlacingof{\I}}$ yields $(\interlaceof{\istyle{a}}, \interlaceof{\istyle{b}}) = (\istyle{a}, \istyle{b}) \in \rolestyle{P}^{\interlacingof{\I}}$.
			
			\item[$\axtop$.]
			Let $u \in \top^{\interlacingof{\I}} = \domain{\interlacingof{\I}}$.
			By definition of $\domain{\interlacingof{\I}}$, there exists $u_0 \in \exexof{\I}$ such that $\interlaceof{u_0} = u$.
			Since $\exextomodof{u_0} \in \top^{{\I}}$ and ${\I}$ is a model, it ensures $\exextomodof{u_0} \in \cstyle{A}^{\I}$.
			Therefore $u = \interlaceof{u_0} \in \cstyle{A}^{\interlacingof{\I}}$.
			
			\item[$\axand$.]
			Let $u \in (\cstyle{A}_1 \sqcap \cstyle{A}_2)^{\interlacingof{\I}}$.
			By definition of $\cstyle{A}_1^{\interlacingof{\I}}$ and $\cstyle{A}_2^{\interlacingof{\I}}$, there exists $u_1, u_2 \in \exexof{\I}$ with $\interlaceof{u_1} = \interlaceof{u_2} = u$ and such that $\exextomodof{u_1} \in \cstyle{A}_1^\I$ and $\exextomodof{u_2} \in \cstyle{A}_2^\I$.
			Since $\interlace$ is pseudo-injective, it yields $\exextomodof{u_1} = \exextomodof{u_2}$, hence $\exextomodof{u_1} \in (\cstyle{A}_1 \sqcap \cstyle{A}_2)^{{\I}}$.
			Since $\I$ is a model, it ensures $\exextomodof{u_1} \in \cstyle{A}^\I$.
			Recalling $\interlaceof{u_1} = u$, we obtain $u \in \cstyle{A}^{\interlacingof{\I}}$.
			
			\item[$\axexistsright$.]
			Let $u \in \cstyle{A}^{\interlacingof{\I}}$.
			By definition there exists $v \in \exexof{\I}$ with $\interlaceof{v} = u$ and such that $\exextomodof{v} \in \cstyle{A}^\I$. 
			Since $\I$ is a model, it ensures $\successorof[\I]{\exextomodof{v}}{R.B}$ is defined. 
			Therefore $v \cdot \rolestyle{R}.\cstyle{B} \in \exexof{\I}$ and element $w := \interlaceof{v \cdot \rolestyle{R.}\cstyle{B}}$ satisfies:
			\begin{itemize}
				\item $(u, w) \in \rstyle{R}^{\interlacingof{\I}}$ since $(u, w) = (\interlaceof{v}, \interlaceof{v \cdot \rstyle{R}.\cstyle{B}})$;
				\item $w \in \cstyle{B}^{\interlacingof{\I}}$ since $\exextomodof{v \cdot \rstyle{R}.\cstyle{B}} = \successorof[\I]{\exextomodof{v}}{R.B} \in \cstyle{B}^\I$ and $\interlaceof{v \cdot \rstyle{R}.\cstyle{B}} = w$.
			\end{itemize}
			Hence $u \in (\exists \rstyle{R}.\cstyle{B})^{\interlacingof{\I}}$.
			
			\item[$\axexistsleft$.]
			Let $u \in (\existsrole{R.B})^{\interlacingof{\I}}$, that is there exists $v \in \rolestyle{B}^{\interlacingof{\I}}$ with $(u, v) \in \rolestyle{R}^{\interlacingof{\I}}$.
			By definition of $\domain{\interlacingof{\I}}$, there exists $u_0 \in \exexof{\I}$ such that $\interlaceof{u_0} = u$, and by definition of $\rolestyle{B}^{\interlacingof{\I}}$ there also exists $v_0 \in \exexof{\I}$ such that $\interlaceof{v_0} = v$ and $\exextomodof{v_0} \in \rolestyle{B}^\I$. 
			Notice $(\interlaceof{u_0}, \interlaceof{v_0}) \in \rolestyle{R}^{\interlacingof{\I}}$ hence Lemma~\ref{lem:inter-to-mod-roles} gives $(\exextomodof{u_0}, \exextomodof{v_0}) \in \rolestyle{R}^\I$.
			Therefore $\exextomodof{u_1} \in (\existsrole{R.B})^{{\I}}$.
			Since $\I$ is a model, it ensures $\exextomodof{u_1} \in \rolestyle{A}^{{\I}}$, yielding $u = \interlaceof{u_1} \in \rolestyle{A}^{\interlacingof{\I}}$.
			
			\item[$\axnotright$.]
			By contradiction, assume $u \in \cstyle{A}^{\interlacingof{\I}} \cap \cstyle{B}^{\interlacingof{\I}}$.
			By definition there exists $v, w \in \exexof{\I}$ with $\interlaceof{v} = \interlaceof{w}= u$ and such that $\exextomodof{v} \in \rolestyle{A}^\I$ and $\exextomodof{w} \in \cstyle{B}^\I$.
			Since $\interlace$ is pseudo-injective, we obtain $\exextomodof{v} = \exextomodof{w}$.
			Hence $\exextomodof{v} \in \cstyle{A}^{{\I}} \cap \cstyle{B}^{{\I}}$, contradicting $\I$ being a model.
			
			\item[$\axnotleft$.]
			Let $u \in \rolestyle{\lnot B}^{\interlacingof{\I}}$.
			By definition of $\domain{\interlacingof{\I}}$, there exists $v \in \exexof{\I}$ such that $\interlaceof{v} = u$.
			Since $u \notin \rolestyle{B}^{\interlacingof{\I}}$, we have $\exextomodof{v} \notin \rolestyle{B}^\I$.
			Hence $\I$ being a model gives $\exextomodof{v} \in \rolestyle{A}^\I$, yielding by definition $u = \interlaceof{v} \in \rolestyle{A}^{\interlacingof{\I}}$.
			
			\item[$\axroleinclusion$.]
			Let $(u, v) \in \rolestyle{P}^{\interlacingof{\I}}$.
			By definition of $\domain{\interlacingof{\I}}$, there exists $u_0, v_0 \in \exexof{\I}$ such that $\interlaceof{u_0} = u$ and $\interlaceof{v_0} = v$.
			In case \ref{case:rind} from the definition of $\rolestyle{P}^{\interlacingof{\I}}$ we have $\kb \models \rolestyle{P}({u},{v})$, hence $\kb \models \rolestyle{R}({u},{v})$ and $(u, v) \in \rolestyle{R}^{\interlacingof{\I}}$ by definition of $\rolestyle{R}^{\interlacingof{\I}}$.
			Otherwise both cases \ref{case:rplus} and \ref{case:rminus} provides a subrole $\rolestyle{P_0} \in \posroles$ of $\rolestyle{P}$, hence also of $\rolestyle{R}$, which triggers the corresponding case for $\rolestyle{R}^{\interlacingof{\I}}$ and ensures $(u, v) \in \rolestyle{R}^{\interlacingof{\I}}$.
			
		\end{itemize}
	\end{proof}

	\begin{claim}
		\label{claim-interlacing-has-no-match}
		If $\I$ has no match for $\Query$, then $\interlace$ has none either.
	\end{claim}
	\begin{proof}
		\newcommand{\auxmatch}{\widetilde{\pi}}
		Let $\interlacingof{\I}$ be the $\interlace$-interlacing of $\I$.
		We prove that if $\match : \query \rightarrow \interlacingof{\I}$ is a match, then $(\intertomod \circ \match)_{\vert \tz} = \match_{\vert \tz}$.
		Since $\sigma \circ \match$ is a match of $\query$ in $\I$, it proves in particular that $\intertomod$ injects the c-matches of $\interlacingof{\I}$ in the c-matches of $\I$, hence the claim.
		Let us thus consider a match $\match : \query \rightarrow \interlacingof{\I}$. 
		By definition of $\domain{\interlacingof{\I}}$, we can pick some $\auxmatch : \query \rightarrow \exexof{\I}$ such that $\match = \interlace \circ \auxmatch$ (note that $\auxmatch$ is not a match since we do not define an interpretation on $\exexof{\I}$).
		By Theorem~\ref{thm:meta-interlacing-is-model}, $\intertomod \circ \match$ is a match of $\query$ in $\I$.
		Therefore we have $(\intertomod \circ \match)(\tz) \subseteq \deltastar$, that is $(\intertomod \circ \interlace \circ \auxmatch)(\tz) \subseteq \deltastar$.
		Remark~\ref{remark:f-is-rho-f'} ensures $\sigma \circ \interlace = \exextomod$, hence it is also $(f \circ \auxmatch)(\tz) \subseteq \deltastar$.
		Along with the definition of $\interlace$, it gives $\interlace \circ \auxmatch_{\vert \tz} = \exextomod \circ \auxmatch_{\vert \tz}$.
		Recall $\match = \interlace \circ \auxmatch$, by definition of $\auxmatch$, hence in particular $\match_{\vert \tz} = \interlace \circ \auxmatch_{\vert \tz}$.
		Therefore $\intertomod \circ \match_{\vert{\tz}} = \intertomod \circ \interlace \circ \auxmatch_{\vert \tz} = \exextomod \circ \auxmatch_{\vert \tz} = \interlace \circ \auxmatch_{\vert \tz} = \match_{\vert \tz}$.
		%		\input{\subsectionpath/fig:injection-of-matches}
	\end{proof}
\end{toappendix}

==> lem-lower-minimality-checking.tex <==
%!TEX root = main.tex


\begin{lemma}
\label{lem_lower_minimality_checking}
	For circumscribed \EL without priorities and fixed predicates, data complexity for deciding whether an interpretation is minimal is \coNP-hard. \unsure{Not sure whether this is actually data complexity, as I construct both the ABox and the interpretation but the TBox is fixed?}
\end{lemma}
%
\begin{proof}
	This proof extends Theorem 3 of \cite{Bonatti21}\todo{and uses some of its formulations}.
	We prove the Lemma by reducing the \mn{NP}-complete problem \mn{3}-\mn{coloring} to the complement of our problem, i.e., to deciding whether an interpretation is not minimal.
	
	Let $G=(V,E)$ be the input graph of \mn{3}-\mn{coloring}.
	%
	We encode $G$ in the following ABox \Amc.
	%
	\begin{align*}
		\mn{V}(v), \mn{r}(a,v)     & \qquad \text{for all } v \in V         \\
		\mn{e}(v_1,v_2)            & \qquad \text{for all } (v_1,v_2) \in E \\
		\mn{C}_i(c_i), \mn{C}(c_i) & \qquad \text{for all } i \in \{1,2,3\}
	\end{align*}
	%
	We consider the following (fixed) TBox.
	%
	\begin{align*}
		V                                                              & \sqsubseteq \exists \mn{hasColor} . \mn{C}                   \\
		\exists \mn{hasColor} . \mn{C}_i                               & \sqsubseteq \mn{C}'_i \qquad \text{for all } i \in \{1,2,3\} \\
		\exists \mn{r} . (\mn{C}'_i \sqcap \exists \mn{e} . \mn{C}'_i) & \sqsubseteq \mn{F} \qquad \text{for all } i \in \{1,2,3\}
	\end{align*}
	%
	We set $\Kmc = (\Tmc,\Amc)$ and $\CP = (\emptyset, M, \emptyset, \mn{sig}(\Kmc) \setminus M)$, where $M = \{\mn{C}, \mn{F}\}$.
	%
	We construct an interpretation \Imc by setting
	%
	\begin{align*}
		\Delta^\Imc        & = \{a,c_1,c_2,c_3\} \cup V                            \\
		\mn{V}^\Imc        & = V                                                   \\
		\mn{e}^\Imc        & = E                                                   \\
		\mn{C}_i^\Imc      & = \{c_i\} \qquad \text{for all } i \in \{1,2,3\}      \\
		\mn{C}^\Imc        & = \mn{C}_1^\Imc \cup \mn{C}_2^\Imc \cup \mn{C}_3^\Imc \\
		\mn{hasColor}^\Imc & = \mn{V^\Imc} \times C^\Imc                           \\
		{\mn{C}'}_i^\Imc   & = V  \qquad \text{for all } i \in \{1,2,3\}           \\
		\mn{F}^\Imc        & = \{a\}
	\end{align*}
	
	To show: If \Imc is not minimal, then $G$ can be \mn{3}-\mn{colored}.
\end{proof}

==> thm-combined-lower-bool-instance.tex <==
%!TEX root = main.tex


\begin{theorem}	\label{thm-combined-lower-bool-instance}
	AQ evaluation on circumscribed \dllitebool KBs is \coNExpTime-hard w.r.t.\ combined
	complexity.
\end{theorem}

\begin{proof}
	\newcommand{\ccenter}{\mathsf{Center}}
%	\newcommand{\cpair}{\mathsf{Pair}}
	\newcommand{\cbit}{\mathsf{Bit}}
	\newcommand{\cgoal}{\mathsf{Goal}}
	\newcommand{\callpairs}{\mathsf{AllPairs}}
	\newcommand{\cgoodcol}{\mathsf{GoodCol}}
	\newcommand{\cbadcol}{\mathsf{BadCol}}
	\newcommand{\cred}{\mathsf{R}}
	\newcommand{\cgreen}{\mathsf{G}}
	\newcommand{\cblue}{\mathsf{B}}
	\newcommand{\cgate}{G}
	\newcommand{\ctest}{\mathsf{T}}
	\newcommand{\istested}{\mathsf{Test}}
	
	
	The proof proceeds by reduction from the complement of the $\NExpTime$-complete \succinct\tcol\ problem. %, known to be $\NEXP$-complete due to \cite{papadimitriou-succinct}.
	An instance of \succinct\tcol\ consists of a Boolean circuit $\circuit$ with $2n$ input gates.
	The graph $\graph_\circuit$ encoded by $\circuit$ has $2^n$ vertices, identified by binary encodings on $n$ bits.
	Two vertices $u$ and $v$, with respective binary encodings $u_1 \dots u_n$ and $v_1 \dots v_n$, are adjacent in $\graph_\circuit$ iff $\circuit$ returns True when given as input $u_1 \dots u_n$ on its first $n$ gates and  $v_1 \dots v_n$ on the second half.
	The problem of deciding if $\graph_\circuit$ is 3-colorable has been proven to be $\NExpTime$-complete in \cite{Papadimitriou1986}.
	
	Let $\circuit$ be a Boolean circuit with $2n$ input gates.
	We build a \dllitebool cKB $\circkb$ with $\kb = (\tbox, \abox)$ s.t.\ the AQ $\cgoal(x)$ admits the individual $a$ as a certain answer iff $\circuit$ does not belong to \succinct\tcol.
	Let us already clarify that $\CP$ uses three minimized concept names, namely $\ccenter$, $\callpairs$ and $\cgoodcol$, with the following preference relation $\prec$:
	\begin{align}
		\ccenter \prec \callpairs \prec \cgoodcol
	\end{align}
	It also uses fixed concept names: each $\cbit_i$ for $1 \leq i \leq 2n$ and the six concept names $\cred_1$, $\cgreen_1$, $\cblue_1$, $\cred_2$, $\cgreen_2$ and $\cblue_2$, which will be useful to respectively represent binary encodings and color assignments.
	All other predicates are varying.
	
	Models of $\kb$ contain a central element $a$, that we enforce via the ABox $\abox = \{ \ccenter(a) \}$ and which will be unique
%	, and we add the following axiom in $\tbox$:
%	\begin{align}
%		\ccenter \equiv \; & \lnot \cpair
%	\end{align}
	by virtue of the preference relation.
	This central element will further be used to detect undesired behaviors of the models via the AQ.
%	To this end, we ask $\ccenter$ to be a minimized concept.
%	Let us already clarify that our AQ consists of the concept $\cgoal$ and that we will check whether $\cgoal$ holds on $a$.	
	In a model, each element represents a pair $(v_1, v_2)$ of vertices by its combination of fixed concepts $\cbit_i$ with $1 \leq i \leq 2n$ that corresponds to the binary encodings of $v_1$ and $v_2$.
	To detect models that do not represent all possible pairs, we require each element representing a pair $(v_1, v_2)$ to ``send'' at the center a binary sequence of $2n$ bits that must be different from the encoding of $(v_1, v_2)$.
	This is achieved by the following axioms in $\tbox$:
	\begin{align}
		\top \incl \; & \exists r_i \sqcup \exists \overline{r_i}
		\quad \text{ for each } 1 \leq i \leq 2n
		\\
		\exists r_i^- \incl \; & \ccenter
		\qquad \text{ for each } 1 \leq i \leq 2n
		\\
		\exists \overline{r_i}^- \incl \; & \ccenter
		\qquad \text{ for each } 1 \leq i \leq 2n
		\\
		\top \incl \; & \bigsqcup_{0 \leq i \leq 2n} (\exists r_i \sqcap \lnot \cbit_i) \sqcup (\exists \overline{r_i} \sqcap \cbit_i)
	\end{align}
	We now require the number of sent sequences to be unique, if possible, via the minimized concept name $\callpairs$, triggered by the following axioms in $\tbox$:
	\begin{align}
		\exists r_i^- \sqcap \exists \overline{r_i}^- \incl \; & \callpairs \quad \text{ for each } 1 \leq i \leq 2n
	\end{align}
	Therefore, if (at least) a pair is not represented in a model, then \emph{all} elements can send the binary encoding of a same missing pair to avoid instantiating $\callpairs$.
	If, on the other hand, each pairs is represented (at least once), then the number of sent sequences cannot be unique and $\callpairs$ must be satisfied on the central element $a$.
	To detect this with the AQ, we add the following axiom to $\tbox$:
	\begin{align}
		 \lnot\callpairs \incl \; & \cgoal
	\end{align}
	Now that we can detect whether all pairs are represented, we move to the encoding of colors.
	The respective colors of $v_1$ and $v_2$ are chosen locally via the following axioms in $\tbox$:
	\begin{align}
		\top \incl \; & \cred_1 \sqcup \cgreen_1 \sqcup \cblue_1
		\\
		\top \incl \; & \cred_2 \sqcup \cgreen_2 \sqcup \cblue_2
	\end{align}
	Recall concept names $\cred_1, \cgreen_1, \cblue_1$ and $\cred_2, \cgreen_2, \cblue_2$ are fixed.
	We additionally enforce that if an element represents a pair $(v_1, v_2)$ corresponding to an edge $\{ v_1, v_2 \}$ in $\graph_\circuit$, then it must assign different colors to $v_1$ and $v_2$.
	This is achieved by computing the output of $\circuit$ on input $v_1$ and $v_2$ via a fresh concept $\cgate$ for each gate $\cgate$ of $\circuit$ and adding the following axioms in $\tbox$:
	\begin{align}
		\cgate \equiv \; & \cbit_i \quad\qquad \text{ if } \cgate \text{ is the } i^{\text{th}} \text{ input gate of } \circuit
		\\
		\cgate \equiv \; & \cgate_1 \sqcap \cgate_2 \quad \text{ if } \cgate \text{ is a $\land$-gate with inputs } \cgate_1, \cgate_2
		\\
		\cgate \equiv \; & \cgate_1 \sqcup \cgate_2 \quad \text{ if } \cgate \text{ is a $\lor$-gate with inputs } \cgate_1, \cgate_2
		\\
		\cgate \equiv \; & \lnot \cgate' \quad\qquad \text{if } \cgate \text{ is a $\lnot$-gate with input } \cgate'
	\end{align}
	Assuming the output gate of $\circuit$ is $\cgate_{o}$, it now suffices to add the following axioms in $\tbox$:
	\begin{align}
		\cgate_{o} \sqcap \cred_1 \sqcap \cred_2 \incl \; & \bot
		\\
		\cgate_{o} \sqcap \cgreen_1 \sqcap \cgreen_2 \incl \; & \bot
		\\
		\cgate_{o} \sqcap \cblue_1 \sqcap \cblue_2 \incl \; & \bot
	\end{align}
	While the above allows to ensures each element $e$ representing an edge $\{ v_1, v_2 \}$ assign different colors to $v_1$ and $v_2$, there might still be inconsistent colorings in the sense that $v_1$ might have been assigned another color by some other element $e'$ representing an edge $\{ v_1, v_3 \}$.
	To detect such inconsistent colorings, the central element ``scans'' all colors assigned to a tested vertex, whose encoding correspond to a binary sequence of $n$ bits represented by dedicated concepts $\ctest_i$.
	To do so, the interpretation of each $\ctest_i$ on the center element is first copied by all elements via the following axioms in $\tbox$, defined for each $1 \leq i \leq n$:
	\begin{align}
		\top \incl \; & \exists t_i \sqcup \exists \overline{t_i}
		\\
		\exists t_i^- \incl \; & \ccenter \sqcap \ctest_i
		&
		\exists \overline{t_i}^- \incl \; & \ccenter \sqcap \lnot \ctest_i
		\\
		\exists t_i \incl \; & \ctest_i
		&
		\exists \overline{t_i} \incl \; & \lnot\ctest_i
	\end{align}
	Each element representing a pair $(v_1, v_2)$ then compares whether the encoding of either $v_1$ or $v_2$ matches the sequence $\ctest_i$, via the following axioms:
	\begin{align}
		\bigsqcap_{1 \leq i \leq n} \left( (\cbit_i \sqcap \ctest_i) \sqcup (\lnot \cbit_i \sqcap \lnot \ctest_i) \right) \equiv \; & \istested_1
		\\
		\bigsqcap_{1 \leq i \leq n} \left( (\cbit_{n + i} \sqcap \ctest_i) \sqcup (\lnot \cbit_{n + i} \sqcap \lnot \ctest_i) \right) \equiv \; & \istested_2
	\end{align}
	It then sends the corresponding assigned color back to the central element via the following axioms in $\tbox$, defined for each $C \in \{ \cred, \cgreen, \cblue \}$:
	\begin{align}
	 	\istested_1 \sqcap C_1 \equiv \; & \exists s_C
	 	\\
	 	\istested_2 \sqcap C_2 \equiv \; & \exists s_C
	 	\\
	 	\exists s_C^- \incl \, & \ccenter
 	\end{align}
 	The center now detects whether it receives two different colors for the tested vertex:
 	\begin{align}
 		\bigsqcup_{\substack{ C, C' \in \{ \cred, \cgreen, \cblue \} \\ C \neq C'}} (\exists s_C^- \sqcap \exists s_{C'}^-) \equiv \; & \lnot \cgoodcol
% 		(\exists s_\cred^- \sqcap \exists s_\cblue^-) \sqcup (\exists s_\cblue^- \sqcap \exists s_\cgreen^-) \sqcup (\exists s_\cgreen^- \sqcap \exists s_\cred^-) \incl  \equiv \, & \lnot \cgoodcol
 	\end{align}
	where $\cgoodcol$ is a minimized concept name, which forces the center element to detect an inconsistent coloring if it exists. 
	This is further translated in term of the AQ with:
	 	\begin{align}
		\lnot \cgoodcol \incl \; & \cgoal
	\end{align}
 	
 	We are now done with the construction of $\circkb$.
	It remains to prove that:
	\[
	\circkb \models \cgoal(a) \iff \circuit \notin \succinct\tcol.
	\]
	
	``$\Rightarrow$''.
	Assume $\circuit \in \succinct\tcol$.
	Build a model $\I$ of $\circkb$ based on a legit 3-coloring $\rho : \{ 0, \dots, 2^n - 1 \} \rightarrow \{ \cred, \cgreen, \cblue \}$ of $\graph_\circuit$.
	It is easily verified $\I$ is indeed a model of $\kb$ for which $a \notin \cgoal^{\I}$.
	It remains to verify $\I$ complies with $\CP$.
	By contradiction, assume there exists $\J <_\CP \I$.
	Notice that from the fixed predicates, $\J$ still encodes all pairs and the coloring $\rho$.
	Therefore $\J$ must interpret the minimized predicates as $\I$ does, contradicting $\J <_\CP \I$.
		
	``$\Leftarrow$''.
	Assume $\circuit \notin \succinct\tcol$.
	Consider a model $\I$ of $\circkb$.
	First notice that $\ccenter^\I = \{ a \}$.
	Indeed, $\I$ models $\abox$ hence $a \in \ccenter^\I$, and, if there were $b \in \ccenter^\I$ with $b \neq a$, then we could find $\J <_\CP \I$ by:
	\begin{itemize}
		\item dropping $b$ from $\ccenter^\I$;
		\item {\color{red} blabla $\callpairs$};
		\item copying everywhere in the model the interpretation of each $\ctest_i$ on $a$ ;
		\item modifying accordingly roles $t_i$ and $\overline{t_i}$, pointing to $a$, concepts $\istested_1$, $\istested_2$, roles $s_\cred$, $s_\cgreen$, $s_\cblue$ also pointing to $a$, and concepts $\cgoodcol$, $\cgoal$.
	\end{itemize}
	Let us first assume that there exists a pair that is not represented in $\I$, then we must have $\callpairs^\I = \emptyset$ and thus $a \in \cgoal^\I$.
	Let us now assume all pairs are represented.
	The assignment of colors cannot possibly be consistent since $\circuit \notin \succinct\tcol$.
	Therefore it ensures $\cgoodcol^\I = \emptyset$ and thus $a \in \cgoal^\I$.
	
\end{proof}

==> thm-combined-lower-dllitebool.tex <==
%!TEX root = main.tex

\begin{theorem}
	\label{thm-combined-lower-dllitebool}
	UCQ evaluation over \dllitebool cKBs is $\coNExpTime^\NPclass$-hard w.r.t.\ combined complexity, even
	if the preference relation is empty and there are no fixed predicates.
\end{theorem}

\unsure[inline]{proof does not work!}

\begin{proof}
	To prove this result, we provide a polynomial time reduction from AQ evaluation on circumscribed \ALC KBs, which is known to be $\coNExpTime^\NPclass$-hard w.r.t.\ combined complexity even without fixed concept names and with an empty preference order \cite{Bonatti2009}.

	Let $\Circ(\Kmc)$ be a circumscribed \ALC KB in normal form (see \cref{subsect:fundamental}) with $\Kmc = (\Tmc,\Amc)$, $A_0$ an AQ and $a_0 \in \mn{ind}(A)$.
	%
	We construct a circumscribed \dllitebool KB $\Circ(\Kmc')$ with $\Kmc' = (\Tmc',\Amc')$ and a UCQ $q$ such that $\Circ(\Kmc) \models A_0(a_0)$ iff $\Circ(\Kmc') \models q$.

	First, we add all axioms from \Amc to $\Amc'$.
	%
	Note that axioms of the form $A_1 \sqcap A_2 \sqsubseteq A$, $A \sqsubseteq \neg B$ and $\neg B \sqsubseteq A$ are already in \dllitebool, and can thus simply be taken over from \Tmc to $\Tmc'$; others have to be rewritten or simulated.
	%
	However, in slight abuse of notation, we also take over axioms of the form $\top \sqsubseteq A$, as $\top$ can easily be expressed via the available boolean operators $\neg$ and $\sqcup$.

	To simulate axioms of the form $A \sqsubseteq \exists r . B$, add, for each such axiom, the following axioms to $\Tmc'$:
	%
	\begin{align}
		A           & \incl \exists r_B & \exists r_B^- & \incl B \label{ax:A_r_B_B}          \\
		\exists r_B & \incl \exists r   & \exists r_B^- & \incl \exists r^-, \label{ax:r_B_r}
	\end{align}
	%
	where $r_B$ is a fresh role name for $r$ and $B$.

	To simulate axioms of the form $\exists r.B \incl A$, we start by adding the following axiom to \Tmc for each $\exists r.B \incl A \in \Tmc$:
	%
	\begin{align} \label{ax:a_not_a}
		\overline{A} \equiv \lnot A,
	\end{align}
	%
	where $\overline{A}$ is a fresh concept name for $A$.
	%
	Then, we construct a set $Q$ of CQs to later add to $q$, which will prevent countermodels to house instances of $\neg A \sqcap \exists r.B$.
	%
	Add the following CQ to $Q$:
	%
	\begin{align*}
		\exists y_1, y_2 \, \bar{A}(y_1) \land r(y_1, y_2) \land B(y_2)
	\end{align*}
	%
	As we also have to account for the fresh rules $r_C$, for each $C$ such that there is an axiom $D \incl \exists r.C \in \tbox$, add to $Q$ also the CQ as given next:
	%
	\begin{align*}
		\exists y_1, y_2 \, \bar{A}(y_1) \land r_C(y_1, y_2) \land B(y_2) &
	\end{align*}

	Finally, we construct $q$.
	%
	For this, we first construct a query $q_0$ aiming to encode the instance check $A_0(a_0)$:
	%
	Similar to the construction in \cref{thm:combined-lower-dlliter}, we eliminate the use of the constant $a_0$ by introducing a new concept name $B_{a_0}$ and adding to $\Amc'$ the assertion
	\begin{align*}
		B_{a_0}(a_0).
	\end{align*}
	%
	Then, we can set
	%
	\begin{align*}
		q_0 \coloneqq \exists x_{a_0} \, A_0(x_{a_0}) \wedge B_{a_0}(x_{a_0}),
	\end{align*}
	%
	and, together with the CQs in $Q$, define $q$ as follows:
	%
	\begin{align*}
		q \coloneqq q_0 \vee \bigvee_{q' \in Q} q'
	\end{align*}
	%
	This finishes the construction of $\Circ(\Kmc')$ and $q$.

	\begin{claim}
		$\Circ(\Kmc) \models A_0(a_0)$ iff $\Circ(\Kmc') \models q$.
	\end{claim}

	``$\Leftarrow$''.
	%
	Let $\Circ(\Kmc) \not \models A_0(a_0)$.
	%
	Then, there is a model \Imc of $\Circ(\Kmc)$ such that $\Imc \not \models A_0(a_0)$.
	%
	We construct an interpretation \Jmc as follows:
	%
	\begin{align*}
		\Delta^\Jmc       & \coloneqq \Delta^\Imc                  \\
		A^\Jmc            & \coloneqq A^\Imc                       \\
		\overline{A}^\Jmc & \coloneqq \Delta^\Imc \setminus A^\Jmc \\
		B_{a_0}^\Jmc      & \coloneqq \{a_0\}                      \\
		r^\Jmc            & \coloneqq r^\Imc                       \\
		r_A^\Jmc          & \coloneqq r^\Imc
	\end{align*}
	%
	for all concept names $A$ and role names $r$ that occur in \Kmc.
	%
	We show that \Jmc is a model of $\Circ(\Kmc')$ with $\Jmc \not \models q$.
	%
	It is obvious that \Jmc is a model of $\Amc'$ and that \Jmc satisfies all axioms in $\Tmc \cap \Tmc'$.
	%
	To see that \Jmc also satisfies the axioms in $\Tmc' \setminus \Tmc$, first consider the assertions (\ref{ax:A_r_B_B}) and (\ref{ax:r_B_r}) with $A \sqsubseteq \exists r.B$.
	%
	For $A \sqsubseteq \exists r_B$, let $a \in A^\Jmc$.
	%
	Then, 
	\todo[inline]{todo: Here I have a problem seeing that \Jmc is actually minimal}

	\smallskip

	``$\Rightarrow$''.
	%
	Let $\Circ(\Kmc') \not \models q$.
	%
	Then, there is a model \Imc of $\Circ(\Kmc')$ such that $\Imc \not \models q$.
	%
	%We show that $\Imc$ is also a model of $\Circ(\Kmc)$ with $\Imc \not \models A_0(a_0)$.

	%First note that \Imc must be a model of \Amc as it is a model of $\Amc'$ and $\Amc \subseteq \Amc'$.
	%
	%To see that \Imc is a model of \Tmc, consider any axiom $\alpha \in \Tmc$.
	%
	%If $\alpha$ has the form $A_1 \sqcap A_2 \sqsubseteq A$, $A \sqsubseteq \neg B$ and $\neg B \sqsubseteq A$, it follows immediately from $\alpha \in \Tmc'$ and \Imc being a model of $\Tmc'$ that \Imc satisfies $\alpha$.
	%
	%If $\alpha$ has the form $\top \sqsubseteq A$, the same follows trivially via the semantics of the operators $\neg$ and $\sqcup$ used to express $\alpha$ in \dllite.

	%If $\alpha$ has the form $A \squsbseteq \exists r.B$, consider some $a \in A^\Imc$.


	\todo[inline]{todo}

\end{proof}

==> thm-combined-lower-dllitepos.tex <==
%!TEX root = main.tex


\begin{restatable}{theorem}{thmcombinedlowerdllitepos}
	\label{thm-combined-lower-dllitepos}
	UCQ answering over \dllitepos cKBs involving a single minimized predicate and no fixed predicates is \coNExpTime-hard w.r.t.\ combined complexity
\end{restatable}

\begin{proof}
	To prove this result, we provide a polynomial time reduction from the complement of Succinct3COL, which is known to be \NExpTime-complete \cite{Papadimitriou1986}.

	Let $G = (V,E)$ be a graph with $V = \{v_1, v_2, \cdots, v_{2^n}\}$ and encode each vertex $v_i$ with a binary integer $\bar i$ of length $n$ (as we will handle a lot of indices, we use $\mn{t}$ and $\mn{f}$ for the binary numbers $1$ and $0$, respectively).
	%
	\textcolor{red}{Robin: Quentin said that I can assume $G$ to contain exactly $2^n$ vertices, although the sources allow for less vertices. As I have no references, I am not entirely convinced that this restriction is sound, but without it, the proof does not go through.}
	%
	A \emph{succinct representation} of $G$ is a circuit $C_G$ that computes the following function:
	%
	\[
		C_G(\bar i, \bar j) =
		\begin{cases}
			\mn{t} & \text{if } (v_i,v_j) \in E               \\
			\mn{f} & \text{if, otherwise, }(v_i,v_j) \notin E
		\end{cases}
	\]

	\noindent The problem Succinct3COL is, given the succinct representation $C_G$ of a graph $G$, to decide whether $G$ is 3-colorable.

	We construct a circumscribed \dllitepos KB $\Circ(\Kmc)$ with $\Kmc = (\Tmc,\Amc)$ and a UCQ $q$ that encode a given problem instance.
	%
	With the aim to restrict colors and truth values to those defined in the ABox (see axioms (\ref{ax:min_value_col})), we minimize exactly the concept name $\mn{Min}$ and let others vary freely.
	%
	Our reduction starts by representing the colors (\ref{ax:colors_def}) and truth values (\ref{ax:values_def}) in the ABox.
	%
	The role name $\mn{neq}$ makes the inequality relations within them explicit; see axioms (\ref{ax:neq_colors}) and (\ref{ax:neq_values}).
	%
	\begin{align}
		\mn{Col}(c)                      & \text{ for all } c \in \{\mn{r},\mn{g},\mn{b}\}         \label{ax:colors_def}                             \\
		\mn{neq}(c,c')                & \text{ for all } c,c' \in \{\mn{r},\mn{g},\mn{b}\}  \text{ with } c \neq c'  \label{ax:neq_colors}                            \\
		\mn{Val}_b(\mn{val}_b)           & \text{ for all } b \in \{\mn{f},\mn{t}\}      \label{ax:values_def}                        \\
		\mn{neq}(\mn{val}_b, \mn{val}_{b'}) & \text{ for all } b,b' \in \{\mn{f},\mn{t}\} \text{ with } b \neq b'    \label{ax:neq_values} \\
		\mn{Min}(x)                      & \text{ for all } x \in \{\mn{r},\mn{g},\mn{b},\mn{val}_\mn{t},\mn{val}_\mn{f}\} \label{ax:min_value_col}
	\end{align}

	We aim countermodels to contain $2^n$ instances that each encode a pair $(v_k,v_l) \in V^2$.
	%
	Towards this goal, we lay the foundation to branch a binary tree of depth $n$ from a root $a_\mn{tree}$, which will be later enforced via the constructed UCQ further down.
	%
	The concept names $(\mn{Index}_i)_{i = 1,\cdots,2n}$ encode the tree levels, which fork via the role names $\mn{next}_{i,\mn{t}}$ and $\mn{next}_{i,\mn{f}}$, encoding whether the $i$-th bit in $\bar k \cdot \bar l$ should be set to $\mn{t}$ or $\mn{f}$, respectively.
	%
	The aimed for elements will therefore be (a subset of) the extension $\mn{Index}_{2n}$.  
	%
	A role name $(\mn{hBit}_j)_{j = 1, \cdots, 2n}$ will later set the actual bit values.
	%
	Note that axioms (\ref{ax:index_hBit}) require any $i$-th tree level to set the bits $1$ to $i$, so that the UCQ can later ensure the truth values to coincide with the choice via $\mn{next}$.
	%
	Formally:
	%
	\begin{align}
		\mathclap{\mn{Index}_0(a_\mn{tree})} \label{ax:tree_root}                                                                                                                                         \\
		\mn{Index}_{i-1}            & \sqsubseteq \exists \mn{next}_{i,b}               \label{ax:tree_branch}                                                                                                \\
		\exists \mn{next}^-_{i,b} & \sqsubseteq  \mn{Index}_{i}                                                 \label{ax:next_index}                                                                     \\
		\mn{Index}_i            & \sqsubseteq \exists \mn{hBit}_{j}                                                                   &  & \text{ for all } j \in \{1, \cdots, i\}  \label{ax:index_hBit} \\
		\exists \mn{hBit}_j^-   & \sqsubseteq \mn{Min}                                                                                &  & \text{ for all } j \in \{1, \cdots, 2n\} \label{ax:hBit_min}
	\end{align}
	%
	for all $i \in \{1, \cdots, 2n\}$ and $b \in \{\mn{t}, \mn{f}\}$.

	We encode the color assignments of $(v_k,v_l)$ only at the $2n$-th level via the role name $\mn{hCol}$ for $v_k$ and $\mn{hCol}'$ for $v_l$:
	%
	\begin{align}
		\mn{Index}_{2n}     & \sqsubseteq \exists \mn{hCol} & \mn{Index}_{2n}        & \sqsubseteq \exists \mn{hCol}' \label{ax:hCol_index} \\
		\exists \mn{hCol}^- & \sqsubseteq \mn{Min}          & \exists {\mn{hCol}'}^- & \sqsubseteq \mn{Min} \label{ax:hCol_min}
	\end{align}
	%

	Finally, the computation of a gate $g$ in $C_G$ is enforced for each pair by an outgoing edge $\mn{gate}_g$ at the $2n$-th level.
	%
	Add:
	%
	\begin{align}
		\mn{Index}_{2n}     & \sqsubseteq \exists \mn{gate}_g \label{ax:index_gate}\\
		\exists \mn{gate}_g & \sqsubseteq \mn{Min} \label{ax:gate_min}
	\end{align}
	%
	for all gates $g$ in $C_G$.

	Let the constructed UCQ $q$ be the disjunction over all subsequent CQs.
	%
	We first make sure that no color is used as a truth value (CQs (\ref{cq:hasBit_not_to_color}) and (\ref{cq:gate_not_to_color})) or vice-versa (CQs (\ref{cq:hasCol_not_to_val}) and (\ref{cq:hasCol2_not_to_val})):
	%
	\begin{align}
		\exists x,y \, \mn{hBit}_j(x,y) \wedge \mn{Col}(y)  & \text{ for all } j \in \{1, \cdots, 2n\}     \label{cq:hasBit_not_to_color} \\
		\exists x,y \, \mn{gate}_g(x,y) \wedge \mn{Col}(y)  & \text{ for all gates } g \text{ in } G'   \label{cq:gate_not_to_color}      \\
		\exists x,y \, \mn{hCol}(x,y) \wedge \mn{Val}_b(y)  & \text{ for all } b \in \{\mn{t}, \mn{f}\} \label{cq:hasCol_not_to_val}      \\
		\exists x,y \, \mn{hCol}'(x,y) \wedge \mn{Val}_b(y) & \text{ for all } b \in \{\mn{t}, \mn{f}\} \label{cq:hasCol2_not_to_val}
	\end{align}

	We next simultaneously enforce that a) the structure constructed by axioms (\ref{ax:tree_root})--(\ref{ax:next_index}) really is a tree, and b) that the valuation required by axioms (\ref{ax:index_hBit}) and (\ref{ax:hBit_min}) is consistent with the branching of the tree.
	%
	We achieve this via CQs (\ref{cq:next_correct_additional_bit}), which makes countermodels assign the bits by $\mn{hBit}$ as dictated by $\mn{next}$, and via CQs (\ref{cq:next_same_bits}), which makes countermodels propagate the bit assignment of a node downwards the tree to all successors:
	%
	\begin{align}
		\begin{split}
			\exists x,y,z_1,z_2 \, & \mn{next}_{i-1,b}(x,y) \wedge \mn{hBit}_j(y,z_1) \\
			& \wedge \mn{neq}(z_1,z_2) \wedge \mn{Val}_b(z_2)
		\end{split} \label{cq:next_correct_additional_bit} \\
		\begin{split}
			\exists x,y,z_1,z_2 \, & \mn{next}_{i-1,b}(x,y) \wedge \mn{hBit}_j(x,z_1) \\
			& \wedge \mn{hBit}_j(x,z_2)  \wedge \mn{neq}(z_1,z_2)
		\end{split} \label{cq:next_same_bits}
	\end{align}
	%
	for all $i \in \{1, \cdots, 2n\}$, $j \in \{1, \cdots, i\}$ and $b \in \{\mn{t}, \mn{f}\}$.
	%
	Observe that the above indeed enforces a tree, as nodes must not assign different values to the same bit.

	We go on to construct CQs (\ref{cq:v_color_consistent}) and (\ref{cq:v_u_color_consistent}), which prohibit any two encoded pairs of vertices $(v,u)$ and $(v,u')$ or $(v,u)$ and $(u,u')$ to assign different colors to $v$ or $u$, respectively:
	%
	\begin{align}
		\begin{split}
			\exists & x,y,c,d,z_1, \cdots, z_n \, \mn{hCol}(x,c) \wedge \mn{hCol}(y,d) \\
			& \wedge \mn{neq}(c,d) \wedge \bigwedge_{1 \leq j \leq n} \big(\mn{hBit}_j(y, z_j) \wedge \mn{hBit}_j(x,z_j) \big)
		\end{split} \label{cq:v_color_consistent} \\
		\begin{split}
			\exists & x,y,c,d,z_1, \cdots, z_n \, \mn{hCol}(x,c) \wedge \mn{hCol}'(y,d) \\
			& \wedge \mn{neq}(c,d) \wedge \bigwedge_{1 \leq j \leq n} \big(\mn{hBit}_j(y, z_j) \wedge \mn{hBit}'_{j+n}(x,z_j) \big)
		\end{split} \label{cq:v_u_color_consistent}
	\end{align}

	To make sure that the computation of the boolean circuit is consistent, we construct CQs restricting $\mn{gate}_g$ to follow the logical operator of $g$.
	%
	For this, we assume w.l.o.g.\ that $C_G$ only contains unary NOT-gates, binary AND- and OR-gates, and $2n$ nullary INPUT-gates (each encoding a bit in $\bar k \cdot \bar l$).
	%
	Given an INPUT-gate $g$ from $C_G$, we denote the index of the encoded bit from $\bar k \cdot \bar l$ with $i_g$.
	%
	Construct, for each INPUT-gate $g$ from $C_G$, the CQ as given next:
	%
	\begin{align}
		\begin{split}
			\exists x,y,z \, \mn{gate}_g(x,y) \wedge \mn{hBit}_{i_g}(x,z) \wedge \mn{neq}(y,z) \label{cq:input_gates}
		\end{split}
	\end{align}
	%
	For all NOT-gates $g$ with their parent $g'$, construct
	%
	\begin{align}
		\begin{split}
			\exists x,y \, \mn{gate}_g(x,y) \wedge \mn{gate}_{g'}(x,y) \label{cq:not_gate}
		\end{split}
	\end{align}
	%
	For all AND-gates $g$ with parents $g_1,g_2$, construct
	%
	\begin{align}
		\begin{split}
			\exists x,y,z \, & \mn{gate}_g(x,y) \wedge \mn{Val}_\mn{t}(y) \wedge \mn{gate}_{g_1}(x,z) \\
			& \wedge \mn{Val}_\mn{f}(z)
		\end{split} \\
		\begin{split}
			\exists x,y,z \, & \mn{gate}_g(x,y) \wedge \mn{Val}_\mn{t}(y) \wedge \mn{gate}_{g_2}(x,z) \\
			& \wedge \mn{Val}_\mn{f}(z)
		\end{split} \\
		\begin{split}
			\exists x,y,z \, & \mn{gate}_g(x,y) \wedge \mn{Val}_\mn{f}(y) \wedge \mn{gate}_{g_1}(x,z)  \\
			& \wedge \mn{Val}_\mn{t}(z) \wedge \mn{gate}_{g_2}(x,z)
		\end{split}
	\end{align}
	%
	For all OR-gates $g$ with parents $g_1,g_2$, construct
	%
	\begin{align}
		\begin{split}
			\exists x,y,z \, & \mn{gate}_g(x,y) \wedge \mn{Val}_\mn{f}(y) \wedge \mn{gate}_{g_1}(x,z) \\
			& \wedge \mn{Val}_\mn{t}(z)
		\end{split} \\
		\begin{split}
			\exists x,y,z \, & \mn{gate}_g(x,y) \wedge \mn{Val}_\mn{f}(y) \wedge \mn{gate}_{g_2}(x,z) \\
			& \wedge \mn{Val}_\mn{t}(z)
		\end{split} \\
		\begin{split}
			\exists x,y,z \, & \mn{gate}_g(x,y) \wedge \mn{Val}_\mn{t}(y) \wedge \mn{gate}_{g_1}(x,z)  \\
			& \wedge \mn{Val}_\mn{f}(z) \wedge \mn{gate}_{g_2}(x,z)
		\end{split} \label{cq:or_true_despite_both_false}
	\end{align}

	Finally, we rule out the existence of monochromatic edges in countermodels via CQ (\ref{cq:monochromatic_edge}):
	%
	\begin{align}
		\exists x,y,z \, \mn{hCol}(x,y) \wedge \mn{hCol}'(x,y) \wedge \mn{gate}_{\dot g}(x,z)  \wedge \mn{Val}_\mn{t}(z) \label{cq:monochromatic_edge}
	\end{align}
	%
	where we here and in what follows denote by $\dot g$ the output gate of $C_G$.

	%	Reduction from coSuccinct3COL: ABox encodes 2 Booleans + 3 colors as instances of the minimized predicate $M$. ABox also encode the root of a tree. TBox encodes a tree generating all couples of vertices $(u, v)$. Binary encoding is achieved by having roles pointing to instances of $M$. Picking colors of $u$ and $v$ at each end node is done similarly. Computing the Boolean circuit for each $(u, v)$ is done by having one role per gate of the circuit pointing to an instance of $M$.

	%The query matches if one of the following holds: a color is used as a Boolean or vice-versa; binary encoding is inconsistent with the branchings of the tree; end nodes define a inconsistent 3-coloring (ie there are two end nodes assigning two different colors to a same $u$); the computation of the Boolean circuit is inconsistent; or finally if there is a monochromatic edge.

	\begin{lemma}
		$G$ is 3-colorable iff $\Circ(\Kmc) \not \models q$.
	\end{lemma}
	%
	``$\Rightarrow$''.
	%
	Let $G$ be 3-colorable.
	%
	Then there exists a 3-coloring $\pi : V \rightarrow \{\mn{r},\mn{g},\mn{b}\}$ such that $\pi(v) \neq \pi(u)$ for all $(v,u) \in V$.
	%
	To show that $\Circ(\Kmc) \not \models q$, we construct a countermodel \Imc of $\Circ(\Kmc)$ as follows.
	%
	Let $X \coloneqq \bigcup_{j = 1, \cdots, 2n} \{a_{j,1}, \cdots, a_{j,2^j}\}$; then set

	\begin{align*}
		\Delta^\Imc \coloneqq          & \Ind(\Amc) \cup X                                             \\
		A^\Imc \coloneqq          & \{ a \mid A(a) \in \Amc\}                                     \\
		\mn{neq}^\Imc \coloneqq        & \{ (a,b) \mid \mn{neq}(a,b) \in \Amc\}                        \\
		\mn{Index}^\Imc_i \coloneqq    & \{a_{i,1}, \cdots, a_{i,2^i}\}                                \\
		\mn{next}^\Imc_{i,\mn{t}} \coloneqq & \bigcup_{j = 1, \cdots, 2^{i-1}} \{(a_{i-1,j}, a_{i,2j})\}     \\
		\mn{next}^\Imc_{i,\mn{f}} \coloneqq & \bigcup_{j = 1, \cdots, 2^{i-1}} \{(a_{i-1,j}, a_{i,2j - 1})\} \\
		\begin{split}
			\mn{hBit}^\Imc_i \coloneqq &  \bigcup_{j = 1, \cdots, 2^{i-1}} \big( \{(a,\mn{val}_\mn{t}) \mid a \in  R(a_{i,2j})\} \\
			& \phantom{\bigcup_{1 \leq j \leq 2^{i-1}}\big(} \cup \{(a,\mn{val}_\mn{f}) \mid a \in  R(a_{i,2j-1})\} \big)
		\end{split}
	\end{align*}
	%
	for all concept names $A \in \{\mn{Col}, \mn{Val}_\mn{t},\mn{Val}_\mn{f},\mn{Min},\mn{Index}_0\}$ and $i\in \{1, \cdots, 2n\}$, where we use
	%
	\begin{itemize}
		\item $a_{0,1}$ to denote $a_\mn{tree}$, and
		      %
		\item $R(a_{k,l})$ to denote the set of instances that are reachable in $\Imc$ from $a_{k,l} \in X$ via the family of role names $\mn{next}_{i,\mn{t}}$ and $\mn{next}_{i,\mn{f}}$ (including $a_{k,l}$ itself).
	\end{itemize}
	%
	We furthermore set  $\mn{hCol}^\Imc, {\mn{hCol}'}^\Imc$ as follows.
	%
	Given some $a_{2n,i} \in X$ with $i \in \{1, \cdots 2^{2n}\}$, we denote by $\vartheta(a_{2n,i})$ the encoded pair $(v_k,u_l) \in V^2$, i.e., such that for all $j \in \{1, \cdots, 2n\}$, we have $(a_{2n,i}, \mn{val}_b) \in \mn{hBit}_j^\Imc$ iff the $j$-th bit in $\bar k \cdot \bar l$ is $b$ with $b \in \{\mn{t},\mn{f}\}$.
	%
	\begin{align*}
		\mn{hCol}^\Imc \coloneqq    & \left\{ \big(a_{2n,i}, \pi(v)\big) \mid \vartheta(a_{2n,i}) = (v,u) \right\} \\
		{\mn{hCol}'}^\Imc \coloneqq & \left\{ \big(a_{2n,i}, \pi(u)\big) \mid \vartheta(a_{2n,i}) = (v,u) \right\}
	\end{align*}
	%
	Finally, we set $\mn{gate}_g$ for all gates $g$ in $C_G$.
	%
	We denote the sub-circuit of $C_G$ that contains exactly $g$ and all its ancestors with $C_G^g$ .
	%
	Note that the output gate of $C_G^g$ is $g$, i.e., $C_G^g(\bar k, \bar l)$ computes the value of $g$ in $C_G$ given the input $(\bar k, \bar l)$.
	%
	Then, for all gates $g$, set:
	%
	\begin{align*}
		\begin{split}
			\mn{gate}_g^\Imc \coloneqq & \{(a_{2n,i}, \mn{val}_b) \mid \vartheta(a_{2n,i}) = (v_k,u_l)  \\
			&\phantom{\{(a_{2n,i}, \mn{val}_\mn{t}) \mid} \text{ and } C_G^g(\bar k, \bar l) = b \} \\
		\end{split}
	\end{align*}

	It is obvious that \Imc is a model of \Kmc.
	%
	As $a \in \mn{Min}^\Imc$ iff $\mn{Min}(a)$ for all $a \in \Delta^\Imc$, and $\mn{Min}$ is the only minimized concept, \Imc must furthermore be minimal.

	To see that $\Imc \not \models q$, it is readily checked that
	%
	\begin{itemize}
		\item \Imc by definition has no answer to CQs (\ref{cq:hasBit_not_to_color})--(\ref{cq:v_u_color_consistent}),
		\item additionally, \Imc has no answer to CQs (\ref{cq:input_gates})--(\ref{cq:or_true_despite_both_false}), as otherwise, the computation of $C_G$ would be inconsistent, and
		\item finally, \Imc has no answer to CQ (\ref{cq:monochromatic_edge}), as otherwise, $\pi$ would not be a 3-coloring of $G$.
	\end{itemize}

	\textcolor{red}{Robin: Not sure whether the above suffices or if I need to dig into all the details}

	\smallskip

	``$\Leftarrow$''.
	%
	Let $\Circ(\Kmc)\not \models q$.
	%
	Then there is a model \Imc of $\Circ(\Kmc)$ such that $\Imc \not \models q$.
	%
	We aim to extract a function $\pi : V \rightarrow \{\mn{r},\mn{g},\mn{b}\}$ and to show that $\pi$ is indeed a 3-coloring of $G$.
	%
	This is rather laborious, as we have to prepare the final argument in five steps. In Claim (\ref{claim:relation_ranges})--(\ref{claim:output_gate_edge}), respectively, we
	%
	\begin{enumerate}
		\item briefly argue that $\mn{hBit}$ and $\mn{gate}$ have the range $\{\mn{val}_\mn{t}, \mn{val}_\mn{f}\}$ and that $\mn{hCol}$ and $\mn{hCol}'$ have the range $\{\mn{r},\mn{g},\mn{b}\}$, which will be convenient later on,
		\item identify within \Imc the intended tree-structure,
		\item show that each leaf indeed encodes a pair $(v_k,v_l) \in V^2$, setting precisely the bits from $\bar k \cdot \bar l$,
		\item extract $\pi$ from \Imc and show that it is sound in the sense that any two leaves that encode the same vertex also assign it the same color, and
		\item proof that the leaves correctly compute all gates.
	\end{enumerate}
	%
	We start with the ranges of $\mn{hBit}, \mn{gate}$ and $\mn{hCol}$:
	%
	\begin{claim} \label{claim:relation_ranges}
		The following properties hold.
		\begin{itemize}
			\item both $(x,y) \in \mn{hBit}^\Imc_i$ and $(x,y) \in \mn{gate}^\Imc_g$ entail $y \in \{\mn{val}_\mn{t}, \mn{val}_\mn{f}\}$ for all $i \in \{1, \cdots, 2n\}$ and gates $g$ in $C_G$, and
			\item both $(x,y) \in \mn{hCol}^\Imc$ and $(x,y) \in {\mn{hCol}'}^\Imc$ entail $y \in \{\mn{r},\mn{g},\mn{b}\}$.
		\end{itemize}
	\end{claim}
	%
	\noindent The proof is simple: As \Imc is a model of \Amc, axioms (\ref{ax:min_value_col}) imply $\{\mn{r},\mn{g},\mn{b},\mn{val}_\mn{t},\mn{val}_\mn{f}\} \subseteq \mn{Min}^\Imc$.
	%
	Furthermore, it is obvious that there cannot be any $a \in \mn{Min}^\Imc$ with $\mn{Min}(a) \notin \Amc$, since \Imc would otherwise not be $<_\CP$ minimal (it would then be straightforward to construct a smaller model).
	%
	Ergo, $\mn{Min}^\Imc = \{\mn{r},\mn{g},\mn{b},\mn{val}_\mn{t},\mn{val}_\mn{f}\}$.

	%
	The rest of the claim follows from axioms (\ref{ax:colors_def}), (\ref{ax:values_def}), (\ref{ax:hBit_min}), (\ref{ax:hCol_min}), (\ref{ax:gate_min}), CQs (\ref{cq:hasBit_not_to_color})--(\ref{cq:hasCol2_not_to_val}), and $\Imc \not \models q$:
	%
	For example, in the case of $\mn{hCol}$, consider some $(x,y) \in \mn{hCol}^\Imc$.
	%
	By axiom (\ref{ax:hCol_min}), we have that $y \in\mn{Min}^\Imc$.
	%
	CQ (\ref{cq:hasCol_not_to_val}) and the fact that $\Imc \not \models q$ together yield $y \in\mn{Min}^\Imc \setminus (\mn{Val}_\mn{t} \cup \mn{Val}_\mn{f})$.
	%
	As $\{\mn{val}_\mn{t}, \mn{val}_\mn{f}\} \subseteq \mn{Val}_\mn{t} \cup \mn{Val}_\mn{f}$ by axioms (\ref{ax:values_def}), we thus have that $y \in \{\mn{r},\mn{g},\mn{b}\}$.
	%
	The other cases are analogous.

	This finishes the proof of Claim (\ref{claim:relation_ranges}).

	\smallskip

	We go on by identifying within \Imc the intended tree-structure:
	%
	\begin{claim}
		For all $i \in \{1, \cdots, 2n\}$ there is a set $Y_i \subseteq \mn{Index}^\Imc_i$ that satisfies the following properties:

		\begin{enumerate} \label{claim:tree_induction}
			\item for all $y \in Y_i$, there is exactly one \emph{parent $p \in Y_{i-1}$ of $y$} with $(p,y) \in \mn{next}_{i-1,b}^\Imc$ for some $b \in \{\mn{t}, \mn{f}\}$ (we set $Y_0 = \{a_\mn{tree}\}$),
			\item for all $y \in Y_i$ and $j \in \{1, \cdots, i \}$, there is exactly one $b \in \{\mn{t}, \mn{f}\}$ such that $(y, \mn{val}_n) \in \mn{hBit}_j$,
			\item for all $x, y \in Y_i$ with $x \neq y$, there is some $j \in \{1, \cdots, i\}$ such that $(x, \mn{val}_\mn{t}) \in \mn{hBit}_j$ iff $(y, \mn{val}_\mn{f}) \in \mn{hBit}_j$, and
			\item $|Y_i| = 2^i$.
		\end{enumerate}
	\end{claim}
	%
	\noindent The proof of Claim (\ref{claim:tree_induction}) goes via induction over $i$:
	%
	\begin{description}
		\item[Base case ($i=1)$.]
			%
			Axioms (\ref{ax:tree_root})--(\ref{ax:next_index}) require the existence of some $x,y \in \mn{Index}_1^\Imc$ such that $(a_\mn{tree},x)\in\mn{next}_{1,\mn{t}}^\Imc$ and $(a_\mn{tree},y)\in\mn{next}_{1,\mn{f}}^\Imc$.
			%
			Set $Y_1 = \{x,y\}$.
			%
			Property 1.\ of Claim (\ref{claim:tree_induction}) obviously holds as $a_\mn{tree}$ is, on one hand, the only element in $Y_0$, and, on the other hand, the parent of both $x$ and $y$.
			%
			Together with Claim (\ref{claim:relation_ranges}), axioms (\ref{ax:neq_values}), and (\ref{ax:index_hBit}), and CQs (\ref{cq:next_correct_additional_bit}) (and the fact that $\Imc \not \models q$), we have that $(x, \mn{val}_\mn{t}) \in \mn{hBit}_1^\Imc$ and $(y, \mn{val}_\mn{f}) \in \mn{hBit}_1^\Imc$, while $(x, \mn{val}_\mn{f}) \notin \mn{hBit}_1^\Imc$ and $(y, \mn{val}_\mn{t}) \notin \mn{hBit}_1^\Imc$, i.e., also properties 2.\ and 3.\ hold.
			%
			The above furthermore entails $x \neq y$, which is why also property 4.\ must hold.
			%
		\item[Induction step ($i > 1$).]
			% 
			By the induction hypothesis, there is a set $Y_{i-1}$ with the claimed properties.
			%
			For all $y \in Y_{i-1}$, axioms (\ref{ax:tree_root})--(\ref{ax:next_index}) entail the existence of elements $a_y,a_y' \in \mn{Index}_i^\Imc$ such that $(y,a_y)\in\mn{next}_{i,\mn{t}}^\Imc$ and $(y,a'_y)\in\mn{next}_{i,\mn{f}}^\Imc$.
			%
			Similar as in the base case, we deduct that $(a_y, \mn{val}_\mn{t}) \in \mn{hBit}_i^\Imc$ and $(a'_y, \mn{val}_\mn{f}) \in \mn{hBit}_i^\Imc$, while $(a_y, \mn{val}_\mn{f}) \notin \mn{hBit}_i^\Imc$ and $(a'_y, \mn{val}_\mn{t}) \notin \mn{hBit}_i^\Imc$ $(\dag)$ via Claim (\ref{claim:relation_ranges}), axioms (\ref{ax:neq_values}) and (\ref{ax:index_hBit}), and CQs (\ref{cq:next_correct_additional_bit}) (and the fact that $\Imc \not \models q$).
			%
			Set $Y_i = \bigcup_{y \in Y_{i-1}} \{a_y,a_y'\}$.

			To see that $Y_i$ satisfies property 1., assume to the contrary that there is some $a \in Y_i$ with two parents from $Y_{i-1}$, i.e., that there are two elements $y,y' \in Y_{i-1}$ such that $(y,a) \in \mn{next}_{i-1,b}^\Imc$ and $(y',a) \in \mn{next}_{i-1,b'}^\Imc$ for some $b,b' \in \{\mn{t},\mn{f}\}$.
			%
			By property 3.\ of the induction hypothesis, there must be some $j \in \{1,\cdots,i-1\}$ such that $(x, \mn{val}_\mn{t}) \in \mn{hBit}_j^\Imc$ iff $(x', \mn{val}_\mn{f}) \in \mn{hBit}_j^\Imc$.
			%
			Furthermore observe that Claim (\ref{claim:relation_ranges}) and axioms (\ref{ax:index_hBit}) require $a$ to assign the $j$-th bit, i.e., we have $(a, \mn{val}_\mn{t}) \in \mn{hBit}_j^\Imc$ or $(a, \mn{val}_\mn{f}) \in \mn{hBit}_j^\Imc$.
			%
			In either case, due to axioms (\ref{ax:neq_values}), we can find a homomorphism from CQ (\ref{cq:next_same_bits}) to \Imc, which contradicts the fact that \Imc is a countermodel to $q$.
			%
			Ergo, $Y_i$ must satisfy property 1.

			Property 2.\ follows, in case of $j = i$, from $(\dag)$, and, if otherwise $j \in \{1,\cdots,i-1\}$, from $Y_{i-1}$ satisfying property 2.\ and the fact that Claim (\ref{claim:relation_ranges}), axioms (\ref{ax:neq_values}) and (\ref{ax:index_hBit}), and CQs (\ref{cq:next_same_bits}) require all $a \in Y_i$ to assign the bits $1, \cdots, i-1$ exactly as their parents.

			For property 3, consider some $a,a' \in Y_i$ with $a \neq a'$.
			%
			If $a$ and $a'$ have the same parent $x$, property 3.\ follows from $(\dag)$ and property 1.
			%
			Otherwise, if $a$ has a parent $x$ and $a'$ has a parent $y$ such that $x \neq y$, observe that property 3.\ of the induction hypothesis implies the existence of some $j \in \{1,\cdots,i-1\}$ such that $(x, \mn{val}_\mn{t}) \in \mn{hBit}_j$ iff $(y, \mn{val}_\mn{f}) \in \mn{hBit}_j$.
			%
			Property 3.\ then follows from the fact that Claim (\ref{claim:relation_ranges}), axioms (\ref{ax:neq_values}) and (\ref{ax:index_hBit}), and CQs (\ref{cq:next_same_bits}) require $a$ and $a'$ to assign the bits $1, \cdots, i-1$ exactly as their parents.

			Regarding property 4., observe that by $(\dag)$, $Y_i$ contains two elements $a_y,a_y'$ with $a_y \neq a_y'$ for each $y \in Y_{i-1}$.
			%
			Given any two elements $x,y \in Y_{i-1}$, it is furthermore easy to see that $\{a_x,a_x'\}$ and $\{a_y,a_y'\}$ are disjoint, as by property 2.\ and 3.\ of the induction hypothesis, there must be some bit $j \in \{1,\cdots,i-1\}$ that $x$ and $y$ assign differently, which subsequently must then also be assigned differently by $\{a_x,a_x'\}$ and $\{a_y,a_y'\}$ due to Claim (\ref{claim:relation_ranges}), axioms (\ref{ax:neq_values}) and (\ref{ax:index_hBit}), and CQs (\ref{cq:next_same_bits}).
			%
			As, thus, $|Y_i| = 2 |Y_{i-1}|$, property 4.\ of the induction hypothesis implies $|Y_i| = 2^i$.
	\end{description}
	%
	This finishes the proof of Claim (\ref{claim:tree_induction}).

	\smallskip

	We go on to identify the instances in \Imc that encode pairs of vertices:
	%
	\begin{claim} \label{claim:identify_encoding_pairs}
		We can identify a set $Y \subseteq \mn{Index}_{2n}^\Imc$ and a bijective function $\vartheta : Y \rightarrow V^2$ such that $\vartheta(x) = (v_k,u_l)$ implies $(x, \mn{val}_b) \in \mn{hBit}_i^\Imc$ iff the $i$-th bit in $\bar k \cdot \bar l$ is $b$ for all $b \in \{\mn{t},\mn{f}\}$ and $i \in \{1, \cdots, 2n\}$.
	\end{claim}

	\noindent Claim (\ref{claim:identify_encoding_pairs}) builds upon Claim (\ref{claim:tree_induction}); set $Y = Y_{2n}$.
	%
	By property 2.\ of Claim (\ref{claim:tree_induction}), each $y \in Y$ assigns a unique $b \in \{\mn{t},\mn{f}\}$ to every $i$-th bit with  $i \in \{1, \cdots, 2n\}$, encoded via $(y, \mn{val}_b) \in \mn{hBit}_i^\Imc$.
	%
	Ergo, we can find a function $\vartheta : Y \rightarrow V^2$ such that $\vartheta(y) = (v_k,u_l)$ implies $(y, \mn{val}_b) \in \mn{hBit}_i^\Imc$ iff the $i$-th bit in $\bar k \cdot \bar l$ is $b$ for all $b \in \{\mn{t},\mn{f}\}$ and $i \in \{1, \cdots, 2n\}$.

	Note that $\vartheta$ must be surjective, as by $|Y| = 2^{2n}$ (property 4\ of Claim (\ref{claim:tree_induction})) and the fact that all $x,y \in Y$ pairwise assign at least one bit differently (property 3.\ of Claim (\ref{claim:tree_induction})).

	To see that $\vartheta$ is injective, consider some $x,y \in Y$ with $\vartheta(x) = (v_k,u_l) = \vartheta(y)$.
	%
	By definition of $\vartheta$, we have that $(x, \mn{val}_b) \in \mn{hBit}_i^\Imc$ iff $(y, \mn{val}_b) \in \mn{hBit}_i^\Imc$ for all with $b \in \{\mn{t},\mn{f}\}$ and $i \in \{1, \cdots, 2n\}$, and, together with property 2 \ of Claim (\ref{claim:tree_induction}), even that $(x, \mn{val}_\mn{t}) \in \mn{hBit}_i^\Imc$ iff $(y, \mn{val}_\mn{f}) \notin \mn{hBit}_i^\Imc$.
	%
	Property 3.\ of Claim (\ref{claim:tree_induction}) then entails $x = y$.

	This finishes the proof of Claim (\ref{claim:identify_encoding_pairs}).

	\smallskip

	We go on to extract $\pi$ from \Imc and show that \Imc is sound in the sense that any two elements $x,y \in Y$ that encode the same vertex also assign it the same color as defined by $\pi$.

	\begin{claim} \label{claim:sound_colors}
		The relation $\pi : V \rightarrow \{\mn{r},\mn{g},\mn{b}\}$ with
		%
		\begin{align*}
			\begin{split}
				\pi(v) \coloneqq \{c \in \{\mn{r},\mn{g},\mn{b}\} \mid & \exists y \in Y \text{ such that } \vartheta(y) = (v,u) \\
				& \text{ and } (y, c) \in \mn{hCol}^\Imc \}.
			\end{split}
		\end{align*}
		%
		is a function such that $(y,c_1) \in \mn{hCol}^\Imc$ and $(y,c_2) \in {\mn{hCol}'}^\Imc$ hold for all $y \in Y$ with $\vartheta(y) = (v,u)$, $\pi(v) = c_1$ and $\pi(u) = c_2$.
	\end{claim}
	%
	\noindent Indeed, $\pi$ is a function:
	%
	On one hand, Claim (\ref{claim:relation_ranges}) and axioms (\ref{ax:hCol_index}) ensure the existence of some $c,d \in \{\mn{r},\mn{g},\mn{b}\}$ such that $(y, c) \in \mn{hCol}^\Imc$ and $(y, d) \in \mn{hCol}'^\Imc$ for all $y \in Y$.
	%
	On the other hand, $\pi(y)$ is unique for all $y \in Y$:
	%
	Assume to the contrary that there are two elements $y,y' \in Y$ such that $\vartheta(y) = (v,u)$ with $(y, c) \in \mn{hCol}^\Imc$ and $\vartheta(y') = (v,u')$ with $(y', c') \in \mn{hCol}^\Imc$ and $c' \neq c$.
	%
	By definition of $\vartheta$, $y$ and $y'$ assign the bits with $1,\cdots,n$ the same, i.e., $(y,z) \in \mn{hBit}_i^\Imc$ iff $(y',z) \in \mn{hBit}_i^\Imc$.
	%
	Furthermore, $c' \neq c$ yields $(c',c) \in \mn{neq}^\Imc$ via axioms (\ref{ax:neq_colors}).
	%
	Then, however, there must be a homomorphism from CQ (\ref{cq:v_color_consistent}) to \Imc, which contradicts the fact that $\Imc \not \models q$.
	
	Now, consider some $y \in Y$ with $\vartheta(y) = (v,u)$, $\pi(v) = c_1$ and $\pi(u) = c_2$.
	%
	We first show that $(y,c_1) \in \mn{hCol}^\Imc$.
	%
	The definition of $\pi$ requires the existence of some $y' \in Y$ such that $\vartheta(y') = (v,u')$ and $(y',c_1) \in \mn{hCol}^\Imc$, while there must also be some $c \in \{\mn{r},\mn{g},\mn{b}\}$ such that $(y,c) \in \mn{hCol}^\Imc$ via Claim (\ref{claim:relation_ranges}) and axioms (\ref{ax:hCol_index}).
	%
	By $\vartheta(y) = (v,u)$ and $\vartheta(y') = (v,u')$, Claim (\ref{claim:identify_encoding_pairs}) implies that $(y, \mn{val}_b) \in \mn{hBit}_i^\Imc$ iff $(y', \mn{val}_b) \in \mn{hBit}_i^\Imc$ for all $i \in \{1, \cdots, n\}$ and $b \in \{\mn{t},\mn{f}\}$.
	%
	Then, we have that $(c_1,c) \notin \mn{neq}^\Imc$ via CQs (\ref{cq:v_color_consistent}) and the fact that $\Imc \not \models q$.
	%
	Ergo, by Claim (\ref{claim:relation_ranges}), and axioms (\ref{ax:neq_colors}) and (\ref{ax:hCol_index}), we have that $c = c_1$, i.e., $(y,c_1) \in \mn{hCol}^\Imc$.

	We go on to show that $(y,c_2) \in {\mn{hCol}'}^\Imc$.
	%
	Again, the definition of $\pi$ requires the existence of some $y' \in Y$ such that $\vartheta(y') = (u,u')$ and $(y',c_2) \in \mn{hCol}^\Imc$, while there must also be some $c \in \{\mn{r},\mn{g},\mn{b}\}$ such that $(y,c) \in {\mn{hCol}'}^\Imc$ via Claim (\ref{claim:relation_ranges}) and axioms (\ref{ax:hCol_index}).
	%
	By $\vartheta(y) = (v,u)$ and $\vartheta(y') = (v,u')$, Claim (\ref{claim:identify_encoding_pairs}) implies that $(y, \mn{val}_b) \in \mn{hBit}_{i+n}^\Imc$ iff $(y', \mn{val}_b) \in \mn{hBit}_i^\Imc$ for all $i \in \{1, \cdots, n\}$ and $b \in \{\mn{t},\mn{f}\}$.
	%
	Then, we have that $(c_2,c) \notin \mn{neq}^\Imc$ via CQs (\ref{cq:v_u_color_consistent}) and the fact that $\Imc \not \models q$.
	%
	Ergo, by Claim (\ref{claim:relation_ranges}), and axioms (\ref{ax:neq_colors}) and (\ref{ax:hCol_index}), we have that $c = c_1$, i.e., $(y,c_1) \in {\mn{hCol}'}^\Imc$.

	This finishes the proof of Claim (\ref{claim:sound_colors}).

	\smallskip

	As a last step before proving that $\pi$ indeed is a 3-coloring, we need to argue that the computation of the logical gates within \Imc is sound.

	\begin{claim} \label{claim:output_gate_edge}
		For all $y \in Y$, we have that $\vartheta(y) \in E$ implies $(y, \mn{var}_\mn{t}) \in \mn{gate}_{\dot g}^\Imc$, where $\dot g$ is the output gate of $C_G$.
	\end{claim}
	%
	\noindent As $\vartheta(y) \in E$ implies $C_G^{\dot g}(\bar k,\bar l) =  \mn{t}$, it suffices to show that $C_G^g(\bar k,\bar l) =  b$ implies $(y, \mn{var}_b) \in \mn{gate}_g^\Imc$ for all $y \in Y$ with $\vartheta(y) = (u_k,v_l)$, gates $g$ in $C_G$ and $b \in \{\mn{t}, \mn{f}\}$.
	%
	We do this per induction over the structure of $C_G^g$:
	%
	\begin{description}
		\item[$g$ is an INPUT gate.]
			%
			Let $C_G^g(\bar k,\bar l) =  b$.
			%
			Then, as $g$ is an INPUT gate, the $i_g$-th bit in $\bar k \cdot \bar l$ must be $b$.
			%
			Thus, $(y, \mn{var}_b) \in \mn{hBit}_{i_g}^\Imc$ by definition of $\vartheta$.
			%
			Claim (\ref{claim:relation_ranges}) and axioms (\ref{ax:index_gate}) entail $(y, \mn{var}_{b'}) \in \mn{gate}_g^\Imc$ for some $b' \in \{\mn{t}, \mn{f}\}$.
			%
			Finally, $(y, \mn{var}_b) \in \mn{hBit}_{i_g}^\Imc$, axioms (\ref{ax:neq_values}), CQs (\ref{cq:input_gates}), and the fact that $\Imc \not \models q$ entail $b' = b$, i.e., $(y, \mn{var}_b) \in \mn{gate}_g^\Imc$.
		\item[$g$ is a NOT gate with parent $g'$.]
			%
			Let $C_G^g(\bar k,\bar l) =  b$.
			%
			As $g$ is a NOT gate with parent $g'$, we have that $C_G^{g'}(\bar k,\bar l) =  b'$ for some $b' \in \{\mn{t}, \mn{f}\}$ such that $b' \neq b$.
			%
			By the induction hypothesis, we then have that $(y,\mn{var}_{b'}) \in \mn{gate}_{g'}^\Imc$.
			%
			Claim (\ref{claim:relation_ranges}) and axioms (\ref{ax:index_gate}) entail $(y, \mn{var}_{b''}) \in \mn{gate}_g^\Imc$ for some $b'' \in \{\mn{t}, \mn{f}\}$.
			%			
			Due to $b' \neq b$, CQs (\ref{cq:not_gate}) and the fact that $\Imc \not \models q$, it must be so that $b'' = b$, i.e., $(y, \mn{var}_b) \in \mn{gate}_g^\Imc$.
		\item[$g$ is a AND or OR gate.]
			%
			We omit the details, as these cases are very similar to the NOT case, with the exception that the respective semantics of the logical operators need to be applied.
	\end{description}

	We are now in the position to show that $\pi$ indeed is a 3-coloring.
	%
	Assume to the contrary that there is an edge $(v,u) \in E$ with $\pi(v) = \pi(u) \coloneqq c$.
	%
	Since $\theta$ is a bijection as of Claim (\ref{claim:identify_encoding_pairs}), there exists a unique $y \in Y$ such that $\vartheta(y) = (v,u)$.
	%
	We have $(y,\pi(v)) \in \mn{hCol}^\Imc$ and $(y,\pi(u)) \in {\mn{hCol}'}^\Imc$ by Claim (\ref{claim:sound_colors}), i.e., $(y,c) \in \mn{hCol}^\Imc$ and $(y,c) \in {\mn{hCol}'}^\Imc$.
	%
	Furthermore, by Claim (\ref{claim:output_gate_edge}), $(v,u) \in E$ entails $(y, \mn{var}_\mn{t}) \in \mn{gate}_{\dot g}^\Imc$.
	%
	Together with axioms (\ref{ax:values_def}), there must be a homomorphism from CQ (\ref{cq:monochromatic_edge}) to $\Delta^\Imc$.
	%
	However, this contradicts the fact that \Imc is a countermodel to $q$.
	%
	Ergo, $\pi$ must indeed be a 3-coloring, i.e., $G$ is 3-colorable.


\end{proof}

==> thm-combined-lower-dlliter.tex <==
%!TEX root = main.tex


\begin{theorem}	\label{thm:combined-lower-dlliter}
   UCQ evaluation on circumscribed \dlliter KBs is \TwoExpTime-hard w.r.t.\ combined
        complexity.
        %
        This holds even with a single minimized concept name and no
        fixed concept names.
\end{theorem}

\begin{proof}
  % , which is why we skip most
  % explanations.
	%
  We reduce from (Boolean) UCQ evaluation on \dlliter KBs with
  closed concept names, which is defined in the expected way
   and known to be \TwoExpTime-hard
   \cite{Ngo2016}.
   Let $\Kmc_\Sigma$ be a \dlliter KB with closed concept names,
   $\Kmc = (\Tmc,\Amc)$, and let $q$ be a Boolean UCQ.  We construct a
   circumscribed \dlliter KB $\mn{Circ}_\CP(\Kmc')$, with
   $\Kmc'=(\Tmc',\Amc')$, and a CQ $q'$ such that
   $\Kmc_\Sigma \models q$ iff $\mn{Circ}_\CP(\Kmc') \models q'$.

   As
   in the proof of \cref{thm:combined-lower-el}, we minimize only a
   single concept name $M$ and include \Amc in $\Amc'$. To construct
   $\Tmc'$, we start from \Tmc and extend with additional concept
   inclusions. For $q'$, we start from $q$ and extend with
   additional disjuncts. We will actually use individuals
   $a \in \mn{Ind}(\Amc)$ as constants in~$q'$. These can be
   eliminated by introducing a fresh concept name $A_a$, extending
   \Amc with $A_a(a)$, and replacing in each CQ in $q'$ the constant
   $a$ with a fresh variable $x_a$ and adding the atom $A_a(x_a)$.

   As in the proof of \cref{thm:combined-lower-el}, we include in
   $\Tmc'$ the CI
   %
   \begin{align}
		A \sqsubseteq \M & \quad \text{for all } A \in \Sigma
   \end{align}
	%
   and then have to rule out non-asserted instances of closed concept
   names. To rule out non-asserted instances inside of $\Ind(\Amc)$,
   we add to $q'$ the disjunct $A(a)$ for all $A \in \Sigma$ and
   $a \in \Ind(\Amc)$ with $A(a) \notin \Amc$.

   To rule out instances of closed concept names outside of
   $\Ind(\Amc)$, add
	%
	\begin{align}
		\M(\tc)
	\end{align}
	% s#
	where $\tc$ is a fresh individual. As in the proof of
        \cref{thm:combined-lower-el}, this guarantees that models with
        instances of closed concept names outside of $\Ind(\Amc)$ are
        not minimal. To ensure that no closed concept names are made
        true at \tc, we extend $q'$ with the disjunct $r(x,t)$ for every
        role name $r$ used in \Tmc.
%
                \\[2mm]
        {\bf Claim.} 
                $\Kmc_\Sigma \models q$ iff $\Circ(\Kmc') \models q'$.
\\[2mm]
        The proof is rather straightforward, we omit the details.
%                 \smallskip
%
% 	\noindent The proof is very similar to that of \cref{lem:K_Sigma_q_Circ_CP_K_q}, but some arguments differ.
% 	%
% 	Generally, replace every occurrence of $\Aqt$ with $\{\tc\}$.
% 	%
% 	In the ``$\Leftarrow$''-direction, to derive $\Jmc \not \models q'$, we need, due to $q' = q \cup \exists x.L$, the additional argument that $\mn{L}^\Jmc = \emptyset$ by construction, but can drop the arguments about $h(x) \in \X^\Jmc$ for each $x \in V$.
%
% 	For the ``$\Rightarrow$''-direction, replace the argument that the extension of $\mn{L}$ not being empty causes the identity function to be a homomorphism from $\Dmc_{q'}$ to {\Imc'} via \cref{eq:bar_X,eq:X_Bar_X,eq:copy_query_links,eq:propagate_L_copy} with any instance of $\mn{L}$ being an answer to $q'$.
% 	%
% 	That $\Jmc = \Imc |_{\X^\Imc}$ is a model of $\Tmc$ does not follow from the replaced \cref{eq:T_Axioms_X}, but by the facts that $\Tmc \subseteq \Tmc'$ and that, ensured by \cref{eq:r_X_X}, \tc is not used as a successor for any existential restriction.
% 	%
% 	That $\Jmc \not \models q$ follows directly from the construction of $q'$ and $\Imc \not \models q$.
% 	%
% 	Proving that \Jmc respects $\Sigma$ is much simpler:
% 	%
% 	In the case of $\hat x \notin \Ind(\Amc)$, we do not need to account for the copy of $\Dmc_q$ (i.e., to interpret it ``maximally'').
% 	%
% 	\cref{claim:V_type} can be ignored as well.
% 	%
% 	Finally, not needing to consider $C_\X$ turns the inductions for \cref{claim:t_type} into simple observations.
\end{proof}

==> thm-combined-lower-el-old.tex <==
%!TEX root = main.tex


\begin{proof}
        We give a polynomial time reduction from (Boolean) CQ evaluation on \EL KBs
        with closed concept names, which is \TwoExpTime-hard \cite{Ngo2016}.
        A \emph{KB with closed concept names} takes the form $\Kmc_\Sigma$
        with \Kmc a KB and $\Sigma \subseteq \NC$ a set of closed
        concept names.
        %
        We say that an interpretation \Imc \emph{respects}~$\Sigma$ if for all
        $A \in \Sigma$, $d \in A^\Imc$ implies $A(d) \in \Amc$. 
        %
        Moreover, \Imc is a \emph{model} of $\Kmc_\Sigma$ if \Imc is a
        model of \Kmc and \Imc respects $\Sigma$. Thus, the only
        instances of a closed concept name are those that are
        explicitly asserted in the ABox. Now the problem proved to be
        \TwoExpTime-hard in \cite{Ngo2016} is: given a KB with closed
        concept names $\Kmc_\Sigma$ and a Boolean CQ $q$, decide
        whether $\Kmc_\Sigma \models q$. We remark that the formalism
        in \cite{Ngo2016} also admits closed role names, but these are
        not used in the hardness proof.

        Let $\Kmc_\Sigma$ be an \EL KB with closed
        concept names, $\Kmc = (\Tmc,\Amc)$, and $q$ a Boolean CQ.
        We construct a
        circumscribed \EL KB $\mn{Circ}_\CP(\Kmc')$, with
        $\Kmc'=(\Tmc',\Amc')$, and a CQ $q'$ such that
        $\Kmc_\Sigma \models q$ iff $\mn{Circ}_\CP(\Kmc') \models q'$.

        A natural first attempt is to use use $\Kmc'=\Kmc$ and
        \mbox{$q'=q$}, and to minimize the concept names in $\Sigma$
        while letting all other concept names vary. Apart from using
        more than a single minimized concept name, this does not work
        since the extension of closed concept names may be too large.
        As a simple example, consider the empty ABox and the TBox
        $\top \sqsubseteq \exists r . A$ with $A \in \Sigma$. This KB
        is unsatisfiable when $A$ is closed, but satisfiable when $A$
        is minimized. We thus use a more refined approach.

        % we
        % must have $A^\Imc = \{ a \mid A(a) \in \Amc \}$ for all models
        % \Imc of $\Kmc_\Sigma$ and all $A \in \Sigma$ while this is not
        % necessarily the case for the models of the resulting circumscribed KB
        % $\mn{Circ}_\CP(\Kmc')$.  In fact, models of $\Kmc_\Sigma$ are
        % models of $\mn{Circ}_\CP(\Kmc')$, but it is easy to find
        % examples that refute the converse. We thus need to be more
        % careful in our construction.

        Let \CP be the circumscription pattern that minimizes the
        fresh concept name $M$ and lets all other symbols vary.  In
        what follows, we assemble $\Tmc'$ and $\Amc'$ and define
        $q'$. For $\Amc'$, we start from \Amc and extend with
        additional assertions. $\Tmc'$ contains the CIs from \Tmc
        in a modified form, as well as additional CIs, see below for
        details.

        \smallskip

        We start with connecting the concept names in $\Sigma$ to the
        minimized concept name $M$: % by including in~$\Tmc'$:
        %
        \begin{align}
                A \sqsubseteq \M & \quad \text{for all } A \in \Sigma
                \label{eq:A_subseteq_M}
        \end{align}
        %
        Much of the reduction is concerned with preventing
        non-asserted instances
        $d$ of closed concept names \mbox{$A \in \Sigma$}, that is, elements $d$
        that satisfy
        $A$ but are not an individual from $\mn{ind}(\Amc)$ such that
        \mbox{$A(d) \in
                        \Amc$}. There are three cases to be distinguished.

        We first consider the case that $d=a \in \mn{ind}(\Amc)$, but
        $A(d) \notin \Amc$. We mark such $a$ with
        a fresh concept name~$L$: %. Add to $\Amc'$:
        %
        \begin{align}
                \overline A(a) & \quad \text{for all } a \in
                                 \Ind(\Amc) \text{ with } A(a) \not
                                 \in \Amc \label{eq:bar_A} \\
%        \end{align}
 %       and add to~$\Tmc'$:
  %      \begin{align}
                A \sqcap \overline A \sqsubseteq L & \quad \text{for all }
                A \in \Sigma. \label{eq:L_A_Bar_A}
        \end{align}
        %
        where $\overline A$ is a fresh concept name for each $A \in \Sigma$.

        We next want to achieve that any model \Imc that satisfies  $a \in
                L^\Imc$ for some ABox individual $a$ also satisfies
        $\Imc \models q$ and is thus ruled out as a countermodel
        against the query being entailed. To
        this end, we add a copy of $q$ to $\Amc'$:
        %
        \begin{align}
                A(x)   & \quad \text{for all } A(x) \in \varphi \label{eq:copy_query_concepts}    \\
                r(x,y) & \quad \text{for all } r(x,y) \in \varphi \label{eq:copy_query_relations}
        \end{align}
        % 
        assuming w.l.o.g.\ that $\mn{var}(q) \cap \Ind(\Amc)= \emptyset$.
        % Since $q$
        % may contain concept names from $\Sigma$ and in view of
        % Equation \cref{eq:A_subseteq_M}

        % NEEDED?

        % \noindent\begin{minipage}{.49\linewidth}
        % 	\noindent\begin{align}
        % 	\end{align}
        % \end{minipage}
        % \begin{minipage}{.5\linewidth}
        % 	\noindent\begin{align}
        % \end{minipage}\smallskip


        We want the copy of $q$ in $\Amc'$ to only become `active'
        when the
        concept name $L$ is made true at some individual from $\mn{ind}(\Amc)$;
        otherwise, it should
        be `dormant'. The individual names in $\mn{ind}(\Amc)$, in contrast,
        should always be active.    To achieve this, we
        include in $\Amc'$ the following assertions where $X$ is
        a fresh concept name indicating activeness and $u$ is a
        fresh role name:
        %
        \begin{align}
                \X(a)  & \quad  \text{for all } a \in \Ind(\Amc),
                \label{eq:X_mark}                                          \\
                u(a,x) & \quad \text{for all } a \in \mn{Ind}(\Amc) \text{
                        and } x \in \mn{var}(q) \label{eq:copy_query_links}
        \end{align}
        %
        We then define the CQ $q'$ to be
        $$q' = q \wedge
                \bigwedge_{x \in \mn{var}(q)} \X(x),$$
        %
        and add to $\Tmc'$:
        %
        \begin{align}
                \exists u.L \sqsubseteq \X. \label{eq:propagate_L_copy}
        \end{align}
        %
        Elements generated by existential quantifiers on the right-hand
        side
        of CIs in \Tmc should of course also be active. Moreover,
        dormant elements should not trigger CIs from \Tmc as
        this might generate `unjustified' existential (thus active)
        elements.
        We deal with these issues as follows.
        For an \EL
        axiom $\alpha$,
        we define the axiom $\alpha_\X$ as follows:
        For an \EL
        concept $C$,
        we inductively define the concept $C_\X$ as follows:
        %
        \begin{align*}
                A_\X    & \coloneqq \X \sqcap A & (\exists r.D)_\X & \coloneqq \X \sqcap \exists r.D_\X \\
                \top_\X & \coloneqq \X          & (D \sqcap D')_\X & \coloneqq D_\X \sqcap D'_\X
        \end{align*}
        
        We now include in $\Tmc'$ the following relativized version of~\Tmc:
        
        \begin{align}
                C_\X \sqsubseteq D_\X \quad  \text{for all }C \sqsubseteq D \in \Tmc \label{eq:T_Axioms_X}
        \end{align}
        %
        Note that, when activating the copy of $q$ in $\Amc'$ by
        making $X$ true at all its individual names, then the
        CIs~(\ref{eq:T_Axioms_X}) apply also there and may make
        concept names $A$ with $A \in \Sigma$ true at elements
        $x \in \mn{var}(q)$. Because of~(\ref{eq:A_subseteq_M}), this
        may lead to models in which the copy of $q$ is activated to
        be incomparable to models in which it is not activated
        regarding
        $<_\CP$. This can be remedied by adding to $\Amc'$:
        %
        \begin{align}
                M(x) & \quad \text{ for all } x \in \mn{var}(q).
                \label{eq:M_var_q}
        \end{align}
        %
        The second case of non-asserted instances $d$ of closed concept
        names is that $d$ is not from $\mn{ind}(\Amc) \cup \mn{var}(q)$.
        The idea is that models with
        such instances $d$ should be non-minimal.
        %
        We achieve this by including in $\Amc'$ a fresh individual
        $\tc$ that must satisfy~$\M$, but not necessarily anything
        else. Since any existential instance $d$ of a closed concept
        name must also satisfy~$M$, we can find a model that is
        preferred w.r.t.\ $<_\CP$ by using $\tc$ as a surrogate
        for~$d$, that is, making true at $\tc$ exactly the concept
        names true at $d$, rerouting all incoming and outgoing role
        edges from $d$ to~$\tc$, and then removing $d$ from the
        extension of all concept and role names.  We thus include in
        $\Amc'$:
        %
        \begin{align}
                \M(\tc). \label{eq:M_t_c}
        \end{align}
        %
        The third and last case of non-asserted instances $d$ of closed
        concept names is that $d$ is $t$ or an individual in the copy
        of $q$ in~$\Amc'$. % , that is,
        % $d \in \mn{var}(q) \cup \{t\}$ by
        % assertions~(\ref{eq:M_var_q})~and~(\ref{eq:M_t_c}). 
        Since these individuals satisfy $M$, we may make true at them
        a closed concept name without producing a
        non-minimal model.  To fix this problem, it suffices to
        prevent the individuals in $\mn{var}(q) \cup \{t\}$ to be used
        as witnesses for existential restrictions in \Tmc, as this is
        the only possible reason for creating non-asserted instances of
        closed concept names of the described form.  It is, however,
        easy to identify such witnesses as they must be active and
        satisfy the concept name~$X$. We thus add
        %
        \begin{align}
                \overline \X (a) & \quad \text{for all } a \in
                \mn{var}(q) \cup \{ t\}
                \label{eq:bar_X}
                \\
                u(x,a)           & \quad \text{for all } a \in
                \mn{var}(q) \cup \{ t \} \text{
                        and } x \in \mn{var}(q) \label{eq:copy_query_links_add}
                                   \\
                &\X \sqcap \overline \X \sqsubseteq L. \label{eq:X_Bar_X}
        \end{align}
        %
        where $\overline X$ is a fresh concept name.
        This finishes the construction of $\Tmc'$ and $\Amc'$.
        %
        \\[2mm]
        {\bf Claim.} 
                $\Kmc_\Sigma \models q$ iff $\Circ(\Kmc') \models q'$.

                \smallskip
        \noindent ``$\Leftarrow$''.
        %
        Let $\Kmc_\Sigma \not \models q$.
        %
        Then, there is a model \Imc of $\Kmc_\Sigma$ such that $\Imc \not \models q$.
        %
        W.l.o.g. assume that $\Delta^\Imc \cap (\mn{var}(q) \cup
                \{t\})= \emptyset$.  % and $A^\Imc = \emptyset$ if $A \notin \mn{sig}(\Tmc)$.
        %
        We construct an interpretation \Jmc as follows:
        %
        \begin{align*}
                \Delta^\Jmc & \coloneqq \Delta^\Imc \cup \mn{var}(q)
                \cup \{ t \}                                           \\
                A^\Jmc      & \coloneqq A^\Imc \cup \{ x \mid A(x) \in
                \Amc'\}                                 \\
                %          \overline A^\Jmc & \coloneqq \emptyset  \qquad \text{ if } A
                %                             \in \Sigma\\
                r^\Jmc      & \coloneqq r^\Imc \cup \{ (x,y) \mid
                r(x,y) \in \Amc'\}                     \\
                \X^\Jmc     & \coloneqq \Delta^\Imc                    \\
                %         \overline X^\Jmc & \coloneqq \emptyset \\
                \M^\Jmc     & \coloneqq \bigcup_{A \in \Sigma } A^\Jmc
                \cup \mn{var}(q) \cup \{ t \}
                %		\M^\Jmc     & \coloneqq \Ind(\Aqt) \cup \bigcup_{B \in \Sigma } B^\Jmc 
        \end{align*}
        %
        for all concept names $A \notin \{X,M\}$ and role names $r$.
        %
        From $\Imc \models \Kmc$ and the construction of $\X^\Jmc$, it easily follows that $\Jmc \models \Kmc'$.
        To show $\Jmc \models \Circ(\Kmc')$, we are left to prove that \Jmc is minimal.

        Assume to the contrary that there is a model $\Jmc'$ of
        $\Kmc'$ with $\Jmc' <_\CP \Jmc$.
        %
        As $\M$ is the only minimized concept name, there must be some $a \in \M^\Jmc$ with $a \notin \M^{\Jmc'}$.
        %
        We must have $a \notin \mn{var}(q) \cup \{t\}$ since $M(x) \in \Amc'$ for $x \in \mn{var}(q) \cup \{t\}$ and $\Jmc'$ is
        a model of $\Kmc'$. But then, the definition of $M^\Jmc$
        implies
        $a \in
                A^\Jmc$ with $A \in \Sigma$. By definition of $A^\Jmc$, in turn,
        $a \in A^\Imc$ or  $A(a) \in \Amc'$. In the former case,
        it follows from the fact that \Imc respects
        $\Sigma$ that $A(a) \in \Amc \subseteq \Amc'$, and thus
        $A(a) \in \Amc'$ in both cases. Now,
        CI~(\ref{eq:A_subseteq_M}) and $a \notin \M^{\Jmc'}$ imply
        that
        $\Jmc'$ is not a model of $\Kmc'$, a contradiction.

        We are left to show that $\Jmc \not \models q'$.
        %
        Assume to the contrary that there is a homomorphism $h$ from $\Dmc_{q'}$ to \Jmc.
        %
        We derive a contradiction to $\Imc \not \models q$ by showing
        that $h$ is also a homomorphism from $\Dmc_q$ to \Imc.
        %
        First, note that $h$ is a function from $\mn{var}(q)$ to
        $\Delta^\Imc$ since $\mn{var}(q')=\mn{var}(q)$ and for each
        $x \in \mn{var}(q')$, we have $X(x) \in q'$ and thus $h(x)\in
                \X^\Jmc = \Delta^\Imc$.
        %
        Finally, observe that \Imc is identical to the restriction of
        \Jmc
        to $\Delta^\Imc$ and the concept and role names that occur
        in $\Kmc'$ and $q'$.

        \medskip
        ``$\Rightarrow$''.
        %
        Assume that $\Circ(\Kmc') \not \models q'$. Then there is a
        model \Imc of $\Circ(\Kmc')$ with $\Imc \not \models q'$.
        % %
        % The existence of a countermodel to $q'$ lets us find a ``pruned'' model \Imc of $\Circ(\Kmc')$ where the usage of $\Ind(\Aqt)$ is restricted to ABox assertions, as otherwise, \cref{eq:bar_X,eq:X_Bar_X,eq:copy_query_links,eq:propagate_L_copy} would ``activate'' $q'$.
        % %
        % Furthermore, we need $u$ to restrict to assertions in $\Amc'$ for later constructions (\cref{enum:prop_2}).
        % %
        % Formally:
        We show that w.l.o.g, we may assume that \Imc satisfies
        several additional conditions that shall prove to be
        convenient
        in what follows.
        % 
        \begin{claim} \label{claim:pruned_model}
                There is a model \Imc of $\Circ(\Kmc')$ with $\Imc \not \models q'$ that satisfies the following properties.
                %
                \begin{properties}
                        \item $a \in A^\Imc$ implies $A(a) \in \Amc'$
                        for all $a \in \mn{var}(q) \cup \{ t \}$, \label{enum:prop_1}
                        %
                        \item $(d,e) \in r^\Imc$ implies $r(d,e) \in
                                \Amc'$ for all $d,e \in \Delta^\Imc$ with
                        $\{d,e\} \cap (\{\mn{var}(q) \} \cup \{t \}) \neq \emptyset$, and \label{enum:prop_3}
                        %
                        \item $(d,e) \in u^\Imc$ implies $u(d,e) \in \Amc'$ for all $d,e \in \Delta^\Imc$. \label{enum:prop_2}
                \end{properties}
        \end{claim}

        \noindent We may construct the desired \Imc from any model
        $\Imc'$ of $\Circ(\Kmc')$ with $\Imc' \not \models q'$, as follows:
        %
        \begin{align*}
                \Delta^\Imc & \coloneqq \Delta^{\Imc'}                   \\
                A^\Imc      & \coloneqq A^{\Imc'} \setminus \{a \in
                \mn{var}(q) \cup \{t\} \mid A(a) \notin \Amc'\}          \\
                u^\Imc      & \coloneqq \{ (x,y) \mid u(x,y) \in \Amc'\} \\
                \begin{split}
                        r^\Imc      & \coloneqq r^{\Imc'} \setminus \{ (x,y) \mid r(x,y) \notin \Amc' \text{ and } \\
                        & \phantom{\coloneqq r^{\Imc'} \setminus \{ (x,y) \mid \;\,}  \{x,y\} \cap (\mn{var}(q) \cup \{t\})\neq \emptyset \}
                \end{split}
        \end{align*}
        %
        for all concept names $A$ and role names $r \neq u$.
        %
        Obviously, $\Imc \not \models q'$, $\Imc \models \Amc'$ and
        Points~\ref{enum:prop_1} to~\ref{enum:prop_3} hold by construction.
        %
        To show that $\Imc \models \Tmc'$, note the following:
        %
        \begin{itemize}
                \item \Imc obviously satisfies the CIs~(\ref{eq:A_subseteq_M}) by construction and the fact that $\Imc'$ is a model of $\Kmc'$.
                \item
                      \Imc satisfies
                      CIs~(\ref{eq:L_A_Bar_A}),~(\ref{eq:propagate_L_copy})~and~(\ref{eq:X_Bar_X}) as
                      $L^{\Imc'}$ must be empty---otherwise
                      Assertions~(\ref{eq:copy_query_links})~and~CIs~(\ref{eq:propagate_L_copy})
                      activate the copy of $q$ in $\Amc'$
                      and thus there is a trivial homomorphism from $q'$ to $\Imc'$, contradicting $\Imc' \not \models q'$.
                      %

                \item
                      For the CIs (\ref{eq:T_Axioms_X}), observe that $\X^{\Imc'} \cap
                              (\mn{var}(q) \cup \{t\})= \emptyset$ following the same argument and
                      using
                      Assertions~(\ref{eq:bar_X}) and CI~(\ref{eq:X_Bar_X}).
                      %
                      Hence $$\X^{\Imc'} \cap A^{\Imc'} = \X^\Imc \cap A^\Imc$$ and
                      $$(\X^{\Imc'} \times \X^{\Imc'}) \cap r^{\Imc'} = (\X^\Imc \times
                              \X^\Imc) \cap r^\Imc$$ for all concept names $A$
                      and role names $r \neq u$.
                      %
                      Consequently, $C_\X^{\Imc'} = C_\X^\Imc$.
                      %
                      Together with the fact that $\Imc' \models C_\X \sqsubseteq
                              D_\X$, \Imc must also satisfy $C_\X \sqsubseteq D_\X$.

                \item
                      We are left to show that \Imc is minimal; however, this is easy to see as $\Imc'$ is minimal and $\Imc \leq_\CP \Imc'$.
                      %
        \end{itemize}
        %
        This finishes the proof of Claim~\ref{claim:pruned_model}.

        \smallskip

        We aim to show that the interpretation $\Jmc$, obtained as the
        restriction of \Imc to domain ${\X^\Imc}$, is a model of
        $\Kmc_\Sigma$ with \mbox{$\Jmc \not \models q$}.
                We assume that the properties from
                Claim~\ref{claim:pruned_model}
                are satisfied, and Property~(a) yields $\Delta^\Jmc
                \cap (\mn{var}(q) \cup \{ t \}) = \emptyset$.
        %
                Assertion~(\ref{eq:X_mark}) yields
                $\Ind(\Amc) \subseteq \Delta^\Jmc$ and since
                $\Amc \subseteq \Amc'$ and \Imc is a model of $\Amc'$,
                \Jmc must be a model of~\Amc.
        %
        Since $\Jmc$ is the restriction of \Imc to $\X^\Imc$ and \Imc satisfies CIs~(\ref{eq:T_Axioms_X}), \Jmc must satisfy \Tmc as well.

        To see that $\Jmc \not \models q$, assume to the contrary that there is a homomorphism $h$ from $q$ to \Jmc.
        %
        As \Jmc is the restriction of \Imc to $\X^\Imc$ and $q'$ is
        the extension of $q$ that adds atoms $\X(x)$ for all variables
        $x$, $h$ must also be a homomorphism from $q'$ to~\Imc. This contradicts $\Imc \not \models q'$.

        We are left to argue that \Jmc respects $\Sigma$.
        %
        Assume to the contrary that there is some $A \in \Sigma$ and $d_0 \in A^\Jmc$ with \mbox{$A(d_0) \notin \Amc$}.
        %
        We have $d_0 \in \X^\Imc$ by construction of \Jmc.
        %
        First assume that $d_0 \in \Ind(\Amc)$. Then (\ref{eq:bar_A}),
        (\ref{eq:L_A_Bar_A}), (\ref{eq:copy_query_links}), and (\ref{eq:propagate_L_copy}) activate the
        copy of $q$ in $\Amc'$, giving a homomorphism from $q$ to \Imc, contradicting $\Imc \not \models q'$.
        %
        
        The more laborious case is $d_0 \notin \Ind(\Amc)$. As we show
        in the following, we may then
        %note that $d_0 \notin \Ind(\Aqt)$ by \cref{enum:prop_1} $(*)$.
        %
        construct a model $\Imc' <_\CP \Imc$ of~$\Kmc'$,
        contradicting the minimality of \Imc.

        Intuitively, in the construction of $\Imc'$ we replace $d_0$
        with $t$ by making true at $t$ all concept names that are true
        at $d_0$, making false all concept names at $d_0$, and
        ``redirecting'' all incoming and outgoing edges of $d_0$ to
        $\tc$.  This forces us to make $X$ true at $t$, and
        by~(\ref{eq:propagate_L_copy}) and (\ref{eq:bar_X}) to
        (\ref{eq:X_Bar_X}) we must activate the copy of $q$ in
        $\Amc'$. But then the CIs~(\ref{eq:T_Axioms_X}) apply to that
        copy. To satisfy them, we make all concept and role names
        true in the copy of $q$.  In detail:
        %
        \begin{align*}
                \Delta^{\Imc'} & \coloneqq \Delta^\Imc                \\
                A^{\Imc'}      & \coloneqq (A^\Imc \setminus \{d_0\})
                \cup \{ \tc \mid d_0 \in A^\Imc \}
                \cup \mn{var}(q)                                      \\
                L^{\Imc'}      & \coloneqq \Delta^\Imc                \\
                \begin{split}
                        r^{\Imc'} & \coloneqq (r^\Imc \setminus \{ (d,e) \mid d_0 \in \{d,e\} \}) \\ 
                        & \phantom{\coloneqq} \cup \{ (e, \tc) \mid (e,d_0) \in r^\Imc  \text{ and } e \neq d_0 \}                              \\
                        & \phantom{\coloneqq} \cup \{ (\tc, e) \mid (d_0,e) \in r^\Imc \text{ and } e \neq d_0 \} \\
                        & \phantom{\coloneqq} \cup \{ (\tc, \tc) \mid (d_0,d_0) \in r^\Imc \} \\
                        & \phantom{\coloneqq} \cup (\mn{var}(q) \times \mn{var}(q))
                \end{split}
        \end{align*}
        %
        for all concept names $A \neq L$ and role names $r$. % than $\mn{sig}(\Kmc') \setminus \{L\}$ and concepts $C,D \in \clT$.
        %

        Because \Imc satisfies 
        Assertions~(\ref{eq:M_var_q})~and~(\ref{eq:M_t_c}) and
        $d_0 \in \Delta^\Jmc$ cannot be from
        $\mn{var}(q) \cup \{ t \}$, we have
        $M^{\Imc'} = M^\Imc \setminus \{d_0\}$ by construction of
        $\Imc'$. Thus $\Imc' <_\CP \Imc$, as desired. It remains to
        prove that $\Imc'$ is a model of $\Kmc'$.
        %
        We have  $\Imc'\models \Amc'$ because $\Imc \models \Amc'$ and
        the restrictions of \Imc and of $\Imc'$ to $\Ind(\Amc')$ are identical.
        %
        Before we argue that $\Imc'$ is a model of $\Tmc'$, we show that the redirection does not ``damage'' concept extensions.
        %
        We denote with $\mn{sub}(\Tmc)$ the set of all concepts that occur in $\Tmc$, closed under subconcepts.
        %
        \begin{claim} \label{claim:t_type}
                The following hold for all $C \in \mn{sub}(\Tmc)$:
                %
                \begin{enumerate}
                        \item $\tc \in C_\X^{\Imc'}$ iff $d_0 \in C_\X^{\Imc}$, and \label{prop:tc_c_x}
                              %
                        \item $x \in C_\X^{\Imc'}$ iff $x \in C_\X^\Imc$ for all $x \in \Delta^\Imc \setminus (\mn{var}(q) \cup \{t\} \cup \{d_0\})$. \label{prop:x_c_x}
                \end{enumerate}
        \end{claim}
        %
        \noindent We prove Points~1 and~2 simultaneously by induction
        on the structure of $C$, making a case distinction according
        to the topmost operator in $C$:
        %
        \begin{itemize}
                \item
                      $C = \top$. Point~1 holds since $\tc \in \X^{\Imc'}$ and
                      $d_0 \in X^\Imc$ and Point~2 holds since by construction of
                      $\Imc'$,         $x \in \X^{\Imc'}$ iff $x \in \X^\Imc$ for all $x \in \Delta^\Imc \setminus (\mn{var}(q) \cup \{t\} \cup \{d_0\})$.

                \item $C = A$. Immediate by construction of $\Imc'$ and Point~\ref{enum:prop_1} of Claim~(\ref{claim:pruned_model}).

                \item $C = C_1 \sqcap C_2$. Straightforward using the
                      semantics and the induction hypothesis.

                \item $C = \exists r . D$.
                      Note that Point~\ref{enum:prop_3} of Claim~(\ref{claim:pruned_model}) and the construction of
                      $r^{\Imc'}$ entail the following for all $x,y \in \Delta^\Imc$:
                      \begin{align}
                        (\tc,y) \in r^{\Imc'} &\quad\text{iff} \quad (d_0, y) \in r^\Imc \tag{\dag} \\
                        (x,\tc) \in r^{\Imc'} &\quad\text{iff} \quad (x,d_0) \in r^\Imc \tag{\ddag}
                      \end{align}
                      %
                      For the "$\Rightarrow$"-direction of Point~1, let $t \in (\exists r.D_X)^{\Imc'}$, i.e., let there be some $y \in D_X^{\Imc'}$ with $(t,y) \in r^{\Imc'}$.
                      Via $(\dag)$, we conclude that $(d_0, y) \in r^\Imc$, and Point~2 of the induction hypothesis yields $y \in D_\X^\Imc$---together, $d_0 \in C_\X^{\Imc'}$.
                      %
                      The "$\Leftarrow$"-direction of Point~1 is analogous.

                      For the ``$\Rightarrow$''-direction of Point~2,
                      let $x \in (\exists r.D_X)^{\Imc'}$ such that $x \notin \mn{var}(q) \cup \{t\} \cup \{d_0\}$.
                      %
                      Then, there must be some $y \in D_X^{\Imc'}$ with $(x, y) \in r^{\Imc'}$.
                      %
                      The construction of $r^{\Imc'}$ implies that either $y \neq d_0$ with $(x,y) \in r^\Imc$ or $y = t$ hold.
                      %
                      In case of $y \neq d_0$ with $(x,y) \in r^\Imc$, we furthermore have $y \notin \mn{var}(q) \cup \{t\}$ by Point~\ref{enum:prop_3}.
                      %
                      Therefore, Point~2 of the induction hypothesis implies $y \in D_X^\Imc$; ergo $x \in C_X^\Imc$.
                      %
                      In case of $y = t$, $(\ddag)$ implies $(x,d_0)\in r^\Imc$, and Point~1 of the induction hypothesis yields $d_0 \in D_X^\Imc$---together, we again have $x \in C_X^\Imc$.

                      For the ``$\Leftarrow$''-direction of Point~2, let $x \in C_\X^\Imc$.
                      %
                      Then there is some $y \in D_\X^\Imc$ with $(x,y) \in r^\Imc$.
                      %
                      By Point~\ref{enum:prop_3} of Claim~(\ref{claim:pruned_model}), we have $y \notin \mn{var}(q) \cup \{t\}$.
                      %
                      Ergo, if $y \neq d_0$, $y \in D_\X^\Imc$ follows from Point~2 of the induction hypothesis, and $(x,y) \in r^{\Imc'}$ stems from the construction of $r^{\Imc'}$---together, $x \in C_\X^{\Imc'}$.
                      %
                      If otherwise $y=d_0$, we have $(x,\tc) \in r^{\Imc'}$ by $(\ddag)$  and $\tc \in D_\X^{\Imc'}$ by Point~1 of the induction hypothesis, i.e., $x \in  C_\X^{\Imc'}$.
                      %
        \end{itemize}
        This finishes the proof of Claim~\ref{claim:t_type}.

        \smallskip

        We will also rely on the following, which follows directly from the construction of $\Imc'$.

        \begin{observation} \label{claim:V_type}
                $\mn{var}(q) \subseteq C_\X^{\Imc'}$ for all $C \in \mn{sub}(\Tmc)$.
        \end{observation}

        \noindent We are now in the position to prove $\Imc'\models\Tmc'$.
        %
        To see that $\Imc'$ satisfies the CIs~(\ref{eq:A_subseteq_M}), let
        $x \in A^{\Imc'}$ with $A \in \Sigma$.
        %
        If $x \in \mn{var}(q) \cup \{t\}$, then $x \in \M^{\Imc}$ due
        to Assertions~(\ref{eq:M_var_q})~and~(\ref{eq:M_t_c}),
        and
        thus $x \in \M^{\Imc'}$
        by construction of $\Imc'$.
        %
        %        For the same reason, $\tc \in \M^{\Imc'}$.
        Otherwise, we have $x \in A^\Imc$ by construction of
        $A^{\Imc'}$, yielding $x \in \M^\Imc$ via
        Assertions~(\ref{eq:A_subseteq_M}).
        %
        We must have $x \neq d_0$ and thus $x \in \M^{\Imc'}$ by
        construction
        of $\Imc'$.
        %
        $\Imc'$ obviously satisfies CIs~(\ref{eq:L_A_Bar_A})~and~(\ref{eq:X_Bar_X}) by
        $L^{\Imc'} = \Delta^\Imc$.

        For CI~(\ref{eq:T_Axioms_X}), let $x \in C_\X^{\Imc'}$ for some
        $C \sqsubseteq D \in \Tmc$.
        %
        We know that $x \neq d_0$ as $d_0 \notin X^{\Imc'}$.
        %
        If $x \in \mn{var}(q)$, then Claim~\ref{claim:V_type} implies $x \in D_\X^{\Imc'}$.
        %
        If, otherwise, $x \in \Delta^\Imc \setminus (\mn{var}(q) \cup \{d_0\})$,
        then Claim~\ref{claim:t_type} and the fact that \Imc satisfies
        $C_\X \sqsubseteq D_\X$ clearly yields
        $x \in D_\X^\Imc$.
        %
        

        For CIs~(\ref{eq:propagate_L_copy}), let $x \in \exists (u . L)^{\Imc'}$.
        %
        Point~\ref{enum:prop_2} of Claim~(\ref{claim:pruned_model}) and the construction of $\Amc'$
        entail that $x \in \mn{var}(q)$.
        %
        By construction of $\Imc'$, we get $x \in \X^{\Imc'}$ as desired.

        %	This finishes the proof of \cref{lem:K_Sigma_q_Circ_CP_K_q,thm:combined-lower-el}.
\end{proof}

==> thm-combined-lower-pos-instance.tex <==
%!TEX root = main.tex

\begin{theorem}
	\label{thm-combined-lower-posh-instance}
	AQ evaluation over $\dllitepos$ cKBs is $\coNP$-hard w.r.t.\ combined complexity.
\end{theorem}

\begin{proof}
	\newcommand{\cgoal}{\mathsf{Goal}}
	\newcommand{\redge}{\mathsf{edge}}
	\newcommand{\cvertex}{\mathsf{Vertex}}
	\newcommand{\rhascol}{\mathsf{hasCol}}
	\newcommand{\ccolor}{\mathsf{Color}}
	\newcommand{\ccenter}{\mathsf{Center}}
	\newcommand{\rtovertex}{\mathsf{toVertex}}
	\newcommand{\rtocenter}{\mathsf{toCenter}}
	\newcommand{\is}{\mathsf{Is}}
	\newcommand{\rtothing}{\mathsf{toThing}}
	
	We reduce the complement of the graph 3-colorability problem (3Col) to deciding whether individual $a$ satisfies concept $\cgoal$ over models of the $\dllitepos$ cKB $\circkb$ we construct.
	Let $\graph = (\vertices, \edges)$ be an instance of 3Col.
	Models of our cKB will contain a central element, being the individual $a$ of interest, whose uniqueness is ensured by a minimized concept name $\ccenter$ and the following assertion in $\abox$:
	\begin{align}
		\ccenter(a)
	\end{align}
	For each $V \in \vertices$, we consider three fixed concept names $V_r$, $V_g$, $V_b$ aiming to represent the possible colors assigned to $V$.
	We require each of those concepts to be subsumed by a concept $V$, which is minimized but with a weaker preference compared to $\ccenter$.
	We add the following axioms to $\tbox$:
	\begin{align}
		V_c \incl V \quad \text{ for each } V \in \vertices \text{ and } c \in \{ r, g, b\}
	\end{align}
	and require the following to hold in the preference relation:
	\begin{align}
		\ccenter \prec V \quad \text{ for each } V \in \vertices
	\end{align}
	We now require our central element $a$ to be connected with instances of each $V$ that must also satisfy $\cgoal$, via the following axioms in $\tbox$, defined for each $V \in \vertices$:
	\begin{align}
		\ccenter & \incl \exists \rtovertex_V
		\\
		\exists \rtovertex_V^- & \incl V
		\\
		\exists \rtovertex_V^- & \incl \cgoal
	\end{align}
	Our central element already provides instances of each concept $V$ as we add the following assertions to $\abox$:
	\begin{align}
		V(a) \quad \text{ for each } V \in \vertices
	\end{align}
	Therefore, if $\cgoal$ is not to be satisfied by $a$, it must be because another instance of each $V$ is available elsewhere and cannot be collapsed on $a$.
	This is possible using instances of concepts $V_c$ since those are fixed.
	To ensure at most one color $c$ is chosen per $V \in \vertices$, we require each $V_c$ to send back its $c$ to the central element.
	This is achieved via the following axioms in $\tbox$, defined for each $V \in \vertices$ and $c \in \{ r, g, b\}$:
	\begin{align}
		V_c & \incl \exists \rtocenter_{V, c}
		\\
		\exists \rtocenter_{V, c}^- & \incl \ccenter
		\\
		\exists \rtocenter_{V, c}^- & \incl \is_{V, c}
	\end{align}
	Where each $\is_{V, c}$ is minimized with weaker preference, ie:
	\begin{align}
		U \prec \is_{V, c} \quad \text{ for each } U, V \in \vertices \text{ and } c \in \{ r, g, b\}
	\end{align}
	Each instance of $V_c$ must also be connected to some instances of $\is_{V, c'}$, with $c' \neq c$ that satisfies $\cgoal$.
	This is achieved via the following axioms in $\tbox$, defined for each $V \in \vertices$ and $c, c' \in \{ r, g, b\}$ with $c \neq c'$:
	\begin{align}
		V_c & \incl \exists \rtothing_{V, c'}
		\\
		\exists \rtothing_{V, c'}^- & \incl \is_{V, c'}
		\\
		\exists \rtothing_{V, c'}^- & \incl \cgoal
	\end{align}
	Therefore, if there exists an instance of $V_c$, then $\is_{V, c}$ must hold on $a$.
	Now, if there also exists an instance of $V_{c'}$ for some $c' \neq c$, then the subsequent role $\rtothing_{V, c}$ needs to point toward $a$ to minimize $\is_{V, c}$ and thus makes the query true.
	It is now very easy to represent edges of the graph in a similar manner: for each $\{ U, V \} \in \edges$ and each $c \in \{ r, g, b\}$, add the following axiom:
	\begin{align}
		U_c & \incl \exists \rtothing_{V, c}
	\end{align}
	So that, if ever $V$ happens to have the same color $c$ than $U$, then $\is_{V, c}$ holding on $a$ will force $\rtothing_{V, c}$ to point on $a$.
	
	Let $\circkb$ be the resulting \dllitepos cKB.
	We now prove the following claim:
	\[
	\graph \notin \text{3Col} \iff \circkb \models \cgoal(a)
	\]
	
	
	``$\Rightarrow$''. Assume $\graph \notin \text{3Col}$ and consider a model $\I$ of $\Jmc$.
	{\color{red} To complete.}
	
	``$\Leftarrow$''. Assume $\graph \in \text{3Col}$ and consider a 3-coloring $\tau : \vertices \rightarrow \{ r, g, b\}$.
	We build a model $\I_\tau$ of $\circkb$ by 
	{\color{red} To complete.}
\end{proof}

==> thm-combined-upper-alchi.tex <==
%!TEX root = main.tex

\begin{theorem}
	\label{thm-combined-upper-alchi}
	UCQ evaluation over \ALCHI cKBs is in \TwoExp w.r.t.\ combined complexity.
\end{theorem}

==> thm-combined-upper-dllitebool.tex <==
%!TEX root = main.tex


\begin{theorem}
	\label{thm-combined-upper-dllitebool}
	UCQ evaluation over $\dllitebool$ cKBs is in $\coNExpTime$ w.r.t.\ combined complexity.
\end{theorem}

\begin{proof}
	We exhibit a $\NExpTime$ procedure to decide the complement of our problem, that is existence of a countermodel for UCQ $q$ over $\dllitebool$ cKB $\circkb$.
	Our procedure starts by guessing a interpretation $\I$ whose domain has size at most $\abox + 2^{\sizeof{\tbox} \sizeof{q}}$.
	This can be done in exponentially many non-deterministic steps.
	It further checks whether $\I$ is a model of $\kb$ that does not entail $q$, and rejects otherwise.
	This can essentially be done naively in $\sizeof{\domain{\I}}^{\sizeof{\tbox}\sizeof{q}}$ deterministic steps, that is still simply exponential w.r.t.\ our input.
	The procedure finally checks whether $\I$ complies with $\CP$ by
	iterating over each $\Pmc$ with $\sizeof{\Pmc} \leq 2 \sizeof{\tbox} + 1$ and over each model $\J_\Pmc$ of $\kb$ s.t.\ $\J_\Pmc < \I_\Pmc$.
	If, for a choice of $\Pmc$ and $\J_\Pmc$, we can find a $\J_{\Pmc, e}$ for each $e \in \domain{\I} \setminus \domain{\I_\Pmc}$ s.t.\ $\J_{\Pmc, e} \models \kb$ with $\J_{\Pmc, e} <_\CP \I_{\Pmc \cup \{ e\} }$ and $\J_{\Pmc, e}|_{\domain{\J_\Pmc}} = \J_\Pmc$, then our procedure rejects.
	Otherwise, that is all choices of $\Pmc$ and $\J_\Pmc$ led to the existence of a $e \in \domain{\I} \setminus \domain{\I_\Pmc}$ without a fitting $\J_{\Pmc, e}$, then it accepts.
	Notice that: iterating over such $\Pmc$ can be done in $\sizeof{\domain{\I}}^{2 \sizeof{\tbox} + 1}$ iterations since we require $\sizeof{\Pmc} \leq 2 \sizeof{\tbox} + 1$.
	Computing $\I_\Pmc$ follows directly from the choice of $\Pmc$.
	Since each $\I_\Pmc$ has polynomial size, iterating over each $\J_\Pmc$ can be done naively with exponentially many steps.
	Further iterating over each $e \in \domain{\I} \setminus \domain{\I_\Pmc}$ can be done in $\sizeof{\domain{\I}}$ steps, which is at most exponential by construction.
	Since each $\I_{\Pmc \cup \{ e\} }$ has polynomial size, deciding the existence of $\J_{\Pmc, e}$ can be done naively in exponentially many steps.
	Overall, the procedure uses an exponential number of non-deterministic steps at the beginning and further performs several checks using exponentially many more deterministic steps.
	
	It remains to prove there exists an accepting run iff there is a countermodel for $q$ over $\circkb$.
	If there exists an accepting run, then the corresponding guessed interpretation $\I$ is a model of $\kb$ that does not entail $q$, and it must also comply with $\CP$ otherwise the ``$1 \Rightarrow 2$'' direction from Lemma~\ref{lemma-criteria-combined} ensures the procedure would have rejected it.
	Conversely, if there exists a countermodel, then Lemma~\ref{lemma-bool-countermodel} ensures existence of a countermodel $\I$ whose domain has exponential size.
	This $\I$ can be guessed by the procedure which checks it is indeed a model of $\kb$ not entailing $q$, hence do not reject it at first.
	The ``$2 \Rightarrow 1$'' direction from Lemma~\ref{lemma-criteria-combined} further ensures $\I$ also passes the remaining check performed by the procedure as otherwise it would contradict $\I$ being a model of $\circkb$.
\end{proof}


%\begin{theorem}
%	\label{thm-combined-upper-dllitebool}
%	UCQ evaluation over $\dllitebool$ cKBs is in $\coNExpTime^{\NPclass}$ w.r.t.\ combined complexity.
%\end{theorem}
%
%\begin{proof}
%	Guess candidate countermodel with simply-exp size and use the $\NPclass$ oracle to verify modelhood w.r.t.\ circumscription pattern.
%\end{proof}

==> thm-combined-upper-dllitecore.tex <==
%!TEX root = main.tex



\begin{theorem}
	\label{thm-combined-upper-dllitehorn}
	UCQ answering over \dllitehorn cKBs is in \coNExpTime w.r.t.\ combined complexity.
\end{theorem}

\begin{proof}
	Guess a single-exp large candidate countermodel $\I$.
	Check whether it is indeed a model of $\kb$ without a match for $\Query$.
	Check whether $\I$ complies with $\CP$ based on Lemma~\ref{lemma-criteria-combined}: enumerating every $\I_\Pmc$ with $\sizeof{\Pmc} \leq 2\sizeof{\tbox} +1$ can be done in \ExpTime, and further checking whether $\I_\Pmc$ is a model of $\circkb$ can also be brute-forced in $\ExpTime$ (since $\sizeof{\I_\Pmc} \leq \sizeof{\abox} + 4 \sizeof{\tbox} +1$).
\end{proof}

==> thm-combined-upper-hornh-instance.tex <==
%!TEX root = main.tex
%
\begin{theorem}
	\label{thm-combined-upper-hornh-instance}
	AQ evaluation on circumscribed $\dllitehorn^{\Hmc^-}$ KBs is in $\Uppi^\textrm{P}_2$.
\end{theorem}

\begin{proof}
	Guess a candidate interpretation $\I$ with size $\sizeof{\abox} + 2\sizeof{\tbox}$.
	Check whether it is a model of $\kb$ and if the AQ of interest is \emph{not} satisfied in $\I$. 
	Using a $\NPclass$ oracle, check whether $\I$ is a model of $\circkb$.
	If all above tests succeed, then accept, otherwise reject.
	From Lemma~\ref{lemma-linear-countermodel}, it is immediate that there exists a accepting run if there exists a countermodel for the AQ over $\circkb$.
	Conversely, if a run accepts, then the guessed model $\I$ is a countermodel.
\end{proof}

==> thm-combined-upper-posh-instance.tex <==
%!TEX root = main.tex

\begin{theorem}
	\label{thm-combined-upper-posh-instance}
	AQ evaluation over $\dlliteposh$ cKBs is in $\coNP$ w.r.t.\ combined complexity.
\end{theorem}

\begin{proof}
	Guess a candidate interpretation $\I$ with size $\sizeof{\abox} + 2\sizeof{\tbox}$.
	Check whether it is a model of $\kb$ and if the AQ of interest is \emph{not} satisfied in $\I$. 
	Using the $\PTime$ procedure from Lemma~\ref{lem-posh-modelhood}, check whether $\I$ is a model of $\circkb$.
	If all above tests succeed, then accept, otherwise reject.
	From Lemma~\ref{lemma-linear-countermodel}, it is immediate that there exists a accepting run if there exists a countermodel for the AQ over $\circkb$.
	Conversely, if a run accepts, then the guessed model $\I$ is a countermodel.
\end{proof}

==> thm-data-lower-dllitecoreh.tex <==
%!TEX root = main.tex



\begin{theorem} \label{thm-data-lower-coreh} UCQ evaluation on
  circumscribed $\dllitecoreh$ KBs is $\Uppi^\textrm{P}_2$-hard.  This
  holds even for instance queries, without fixed concept names, and
  with a single negative role inclusion.
\end{theorem}
%
\begin{proof}
	
	\renewcommand{\cstyle}[1]{{\mathsf{#1}}}
	\renewcommand{\rstyle}[1]{{\mathsf{#1}}}
	\newcommand{\ixvar}{{x}} % individual x-variable
	\newcommand{\iyvar}{{y}} % individual y-variable
	\newcommand{\itrue}{t} % individual true
	\newcommand{\itrueof}[1]{\itrue_{#1}} % individual true of some variable
	\newcommand{\ifalse}{f}% individual false
	\newcommand{\ifalseof}[1]{\ifalse_{#1}} % individual false of some variable
	\newcommand{\iclause}{c} % individual clause
	
	\newcommand{\cxvar}{\cstyle{XVar}} % concept x variable
	\newcommand{\cyvar}{\cstyle{YVar}} % concept y variable
	\newcommand{\cclause}{\cstyle{Clause}} % concept clause
	\newcommand{\cformula}{\cstyle{Formula}} % concept formula
	
	\newcommand{\rxeval}{\rstyle{eval}_{\cstyle{X}}}
	\newcommand{\ryeval}{\rstyle{eval}_{\cstyle{Y}}}
	\newcommand{\rceval}{\rstyle{eval}_{\cstyle{C}}}
	\newcommand{\reval}{\rstyle{eval}}
	\newcommand{\rnegeval}{\overline{\reval}}
	
	\newcommand{\cxval}{\cstyle{XVal}}
	\newcommand{\cyval}{\cstyle{YVal}}
	\newcommand{\ccval}{\cstyle{CVal}}
	
	\newcommand{\cvval}{\cstyle{VVal}}
	\newcommand{\cfval}{\cstyle{FVal}}
	
	\newcommand{\iformula}{f}
	\newcommand{\rfeval}{\rstyle{eval}_{\cstyle{F}}}
	
	\newcommand{\cgoal}{\cstyle{Goal}}
	
	
	
%	\newcommand{\J}{\Jmc}

	We give a polynomial time reduction from
        $\forall\exists\mn{3SAT}$, c.f.\ the proof
        of Theorem~\ref{thm-data-lower-el}. Let a
        $\forall\exists$-3CNF sentence
        $\forall \bar x \exists \bar y \, \vp$ be given where
        $\bar x=x_1 \cdots x_m$, $\bar y = y_1 \cdots y_n$, and
        $\varphi=\bigwedge^\ell_{i=1} \bigvee_{j=1}^3 L_{ij}$ with
        $L_{ij} = v$ or $L_{ij} = \lnot{v}$ for some
        $v \in \{ x_1, \dots x_m, y_1, \dots, y_n \}$.  We construct a
        circumscribed \dllitecoreh KB $\circkb$ and an
        instance query $\query$ such that $\circkb \models \query$ iff
        $\forall \bar x \exists \bar y \, \varphi$ is true.

        The circumscription pattern \CP involves four minimized
        concept names with the preference
        $$\cvval \prec \cxval \prec \ccval \prec \cfval,$$ and no
        fixed concept names. %  The
        % instance query is $$\query = \cgoal(\iformula).$$  
        We now
        describe the construction of the KB $\kb=(\Tmc,\Amc)$, not
        strictly
        separating \Tmc from \Amc. We first introduce an ABox
        individual for each variable, marking the existential
        variables
        with the concept name $\cxvar$ and the universal ones with
        $\cyvar$:
	%
	\begin{align}
		\cxvar(\ixvar)
		& \quad \text{for all } x \in \bar x
		\label{eq:xvars} \\
		%
		\cyvar(\iyvar)
		& \quad \text{for all } y \in \bar y.
		\label{eq:yvars}
	\end{align}
        %
        To choose truth values for variables, we use the minimized
        concept name $\cvval$. We introduce two instances of $\cvval$
        for each variable, one representing true and the other false:
        %
        	\begin{align}
		\cvval(\itrueof{v})
		& \quad \text{for all } v \in \bar x \cup \bar y
%		\label{eq:vvalstrue} 
		\\
		%
		\cvval(\ifalseof{v})
		& \quad \text{for all } v \in \bar x \cup \bar y.
%		\label{eq:vvalsfalse}
	\end{align}
        %
        Each variable must choose an instance of $\cvval$ via the role
        names $\rxeval$ an $\ryeval$, depending on whether it is
        existential
        or universal:
	\begin{align}
		\cxvar & \sqsubseteq \, \exists \rxeval
		\label{eq:xvariables_have_value} \\
		\cyvar & \sqsubseteq \, \exists \ryeval
		\label{eq:yvariables_have_value}\\
		\exists {\rxeval}^- & \sqsubseteq \, \cvval
		\label{eq:xvalues_are_vvalues} \\
		\exists {\ryeval}^- & \sqsubseteq \, \cvval.
		\label{eq:yvalues_are_vvalues}
	\end{align}
        %
        There is no guarantee yet, however, that a variable $v$ chooses
        one of the instances $\itrueof{v}$ and $\ifalseof{v}$ of
        $\cvval$ reserved for it.  To ensure this, we first install
        the following role inclusions:
		\begin{align}
		\rxeval  & \sqsubseteq \, \reval
		\label{eq:xeval_is_eval} \\
		\ryeval  & \sqsubseteq \, \reval
		\label{eq:yeval_is_eval} \\
		\reval & \sqsubseteq \, \lnot \rnegeval.
		\label{eq:eval_is_not_negeval}
	\end{align}
	The negative role inclusion allows us to control in a flexible
        way the targets for the existential restrictions in
        CIs~(\ref{eq:xvariables_have_value})
        and~(\ref{eq:yvariables_have_value}), as follows:
	\begin{align}
		\rnegeval(v, \itrueof{v'})
		& \quad \text{for all } v, v' \in \bar x \cup \bar y
           \text{ with }  v \neq v'
		\label{eq:varblock} \\
		%
		\rnegeval(v, \ifalseof{v'})
		& \quad \text{for all } v, v' \in \bar x \cup \bar y \text{ with }  v \neq v'.
		\label{eq:varblocktwo}
	\end{align}
	To force the truth values of the variables in $\bar x$ to be
        identical in all models that are smaller w.r.t.\
        `$<_\CP$', we mark those truth values with the minimized
        concept name
        $\cxval$:
	\begin{align}
          \exists {\rxeval}^- & \sqsubseteq \, \cxval.
                                \label{eq:implxval}
	\end{align}
	We next introduce an individual for each clause:
	\begin{align}
		\cclause(\iclause_i)
		& \quad \text{for } 1 \leq i \leq \ell.
		\label{eq:clauses}
	\end{align}
	We also assign a truth value to every clause, via the role
        name $\rceval$, another subrole of $\reval$. Every element with an
        incoming $\rceval$-edge must make the concept name $\ccval$
        true which is minimized, but with lower priority than
        $\cvval$ and $\cxval$. This reflects the fact that the truth values of
        variables
        determine the truth values of clauses. We put:
	\begin{align}
		\cclause & \sqsubseteq \, \exists \rceval
		\label{eq:clauses_have_value} \\
		\rceval  & \sqsubseteq \, \reval
		\label{eq:ceval_is_eval} \\
		\exists {\rceval}^- & \sqsubseteq \, \ccval
		\label{eq:rceval_is_ccval}
	\end{align}
	The truth values of clauses are represented by the same
        individuals
        as the truth values of variables:
	\begin{align}
	\ccval(\itrueof{v})
	& \quad \text{for all } v \in \bar x \cup \bar y
	\label{eq:cvalstrue} \\
	%
	\ccval(\ifalseof{v})
	& \quad \text{for all } v \in \bar x \cup \bar y
%	\label{eq:vvalsfalse} 
	\end{align}
	We again use the role $\rnegeval$ to control which instance of
        $\cclause$ can be used as truth values for which clause. This
        is based on the literals that occur in the clause.  If a
        variable $v$ occurs positively in the $i^{th}$ clause, then
        $\iclause_i$ has access to $\ifalseof{v}$, while if $v$ occurs
        negatively, then $\iclause_i$ has access to $\itrueof{v}$. And
        those are the only instances of $\cvval$ to which $\iclause_i$
        has access: for $1 \leq i \leq \ell$ and all $v \in \bar x
        \cup \bar y$,
        put
	\begin{align}
		\rnegeval(\iclause_i, \itrueof{v})
		& \quad \text{if } \lnot v \notin \{ L_{i, 1}, L_{i, 2}, L_{i, 3} \}
		\label{eq:clause_block_but_positive} \\
		%
		\rnegeval(\iclause_i, \ifalseof{v})
		& \quad \text{if }  v \notin \{ L_{i, 1}, L_{i, 2}, L_{i, 3} \}.
		\label{eq:clause_block_but_negative}
	\end{align}
        %
        Note that clause individual %$\itrueof{v}$, $\ifalseof{v}$
        % represents not only a truth value of variable $v$, but also a
        % literal for variable $v$. From this perspective, every
        $\iclause_i$ has access via $\rceval$ to $\itrueof{v}$ if
        making $v$ \emph{false} leads to satisfaction of the $i^{th}$
        clause, and likewise for $\ifalseof{v}$ and making $v$
        \emph{true}. Moreover, $v$ being made true is represented by
        an $\rxeval$- or $\ryeval$-edge from $v$ to $\itrueof{v}$ and
        likewise for $v$ being made false and $\ifalseof{v}$. Also
        recall that $\itrueof{v}$ and $\ifalseof{v}$ cannot have such
        incoming edges from elsewhere. Consequently, the $i^{th}$
        clause evaluates to true if we can find a target for the
        $\rceval$-edge that does \emph{not} have an incoming
        $\rxeval$- or $\ryeval$-edge:
	\begin{align}
		\exists {\rxeval}^- & \sqsubseteq \, \lnot \exists {\rceval}^-
		\label{eq:disjone} \\	
		\exists {\ryeval}^- & \sqsubseteq \, \lnot \exists {\rceval}^-.
		\label{eq:disjtwo}
	\end{align}
	In the case that a clause evaluates to false, it cannot reuse
        one of the admitted instances of $\ccval$. We introduce an
        extra instance $f$ of $\ccval$ that can be used instead:
		\begin{align}
		\ccval(\iformula).
		\label{eq:iformula_is_cval}
	\end{align}
	To make sure that $f$ is indeed used as an $\rceval$-target
        only if at least one clause is falsified, we use the fourth
        minimized concept name $\cfval$. Note that it is minimized
        with least priority. We make sure that $f$ must have an
        outgoing $\rfeval$-edge leading to an instance of $\cfval$,
        that $f$ itself is an instance of $\cfval$, and that having an
        incoming $\rfeval$-edge precludes having an incoming
        $\rceval$-edge. If all clauses evaluate to true, then there is
        no need to use $f$ as a target for $\rceval$ and $f$ can use
        itself as the $\rfeval$-target. But if a clause evaluates to
        false, then we must use $f$ as a last resort $\rceval$-target
        and cannot use it as an $\rfeval$-target. Since $\cfval$ is
        minimized with least priority, the latter will simply lead to a fresh instance of $\rfeval$
       to be created. In summary, all clauses evaluate to true
        if and only of $f$ has an incoming $\rfeval$-edge.  We put:
	\begin{align}
		\cformula(\iformula)
%		\label{eq:iformula_is_formula}
%		\\
		& \qquad \cfval(\iformula)
		\label{eq:iformula_is_fval} \\
%	\end{align}
%	And axioms:
%	\begin{align}
		\cformula & \sqsubseteq \, \exists \rfeval
%		\label{eq:clauses_have_value} 
		\\
		\exists {\rfeval}^- & \sqsubseteq \, \cfval
		\\
		\exists {\rceval}^- & \sqsubseteq \, \lnot \exists {\rfeval}^-.
		\label{eq:rcevalfcevaldisj}
	\end{align}
        %
        By what was said above, to finish the reduction it suffices to add
        %
        \begin{align}
          \exists {\rfeval}^- & \sqsubseteq \, \cgoal.
	\end{align}
        %
        to choose as the query $q=\cgoal(x)$, and to ask whether $f$
        is an answer.

        To prove correctness, we thus have to show the following.
        %
        \\[2mm]
        {\bf Claim.} $\circkb \models q(f)$ iff
        $\forall \bar x \exists \bar y \, \varphi$ is true.
        \\[2mm]
        To prepare for the proof of the claim, we first observe that
        every valuation $V$ for $\bar x \cup \bar y$ gives rise
        to a corresponding model $\Imc_V$ of \Kmc. We use domain 
        %
        $$
          \Delta^{\Imc_V} = \Ind(\Amc) 
        $$
        %
        and set
        $$
        A^{\Imc_V} = \{ a \mid A(a) \in \Amc \}
        $$
        for all concept names $$A \in \{ \cxvar, \cyvar, \cvval,
        \ccval, \cclause, \cformula \}.$$
        %
        We interpret $\rxeval$ and $\ryeval$ according to $V$,
        that is
        %
        $$
        \begin{array}{rcl}
          \rxeval^{\Imc_V} &=& \{ (x,\itrueof{v}) \mid x \in \bar x \text{
                           and }V(x)=1\} \,\cup\\[1mm]
                            && \{ (x,\ifalseof{v}) \mid x \in \bar x \text{
                           and }V(x)=0\} 
        \end{array}
        $$
        and analogously for $\ryeval$. Next we put
        %
        $$
        \cxval^{\Imc_V} = \{ e \mid (e,d) \in \rxeval^{\Imc_V} \}.
        $$
        If $V$ makes the $i^{th}$ clause true, then there is a literal
        in it that is true. Choose such a literal $L$ and set
        $w_i = \itrueof{v}$ if $L=\neg v$ an $w_i = \ifalseof{v}$ if
        $L=v$. If $V$ makes the $i^{th}$ clause false, then set
        $w_i=f$. We proceed with the definition of $\Imc_V$:
        %
        $$
        \begin{array}{rcl}
          \rceval^{\Imc_V} &=& \{ (c_i,w_i) \mid 1 \leq i \leq \ell \}
          \\[1mm]
          \reval^{\Imc_V} &=& \rxeval^{\Imc_V} \cup \ryeval^{\Imc_V} \cup
                          \rceval^{\Imc_V} \\[1mm]
          \rnegeval^{\Imc_V} &=& \{(a,b) \mid \rnegeval(a,b) \in \Amc \}
          \\[1mm]
          \cfval^{\Imc_V} &=& \{ f,c_1 \}  \\[1mm]
          \rfeval^{\Imc_V} &=& \{ (f,c_10) \} \\[1mm]
          \cgoal^{\Imc_V} &=& \{ c_1 \}.
        \end{array}
        $$
        %
        The choice of $c_1$ is somewhat arbitrary in the last three
        statements, any other individual without an incoming
        $\rceval$-edge would also do.
        % $V$ also assigns a truth value
        % to each clause, let $V(c_i)$ denote the value of the $i^{th}$
        % clause.
        It is straightforward to verify that $\Imc_V$ is a model of
        \Kmc with $\Imc_V \not\models q(f)$.

        We can define a variation $\Imc'_V$ of $\Imc_V$ that is still
        a model of~\Kmc provided that all clauses are satisfied by $V$
        (which guarantees that $f$ has no incoming $\rceval$-edge), and
        that satisfies $\Imc'_V \models q(f)$. To achieve this, we
        replace the last three lines from the definition of $\Imc_V$
        with
        %
        $$
        \begin{array}{rcl}
          \cfval^{\Imc_V} &=& \{ f \}  \\[1mm]
          \rfeval^{\Imc_V} &=& \{ (f,f) \} \\[1mm]
          \cgoal^{\Imc_V} &=& \{ f \}.
        \end{array}
        $$

        \medskip
        Now for the actual proof of the claim

        \smallskip
        
	``$\Rightarrow$''.  Assume that
        $\forall \bar x \exists \bar y \, \varphi$ is false, and thus
        $\exists \bar x \forall \bar y \, \lnot \varphi$ is true and
        there is a valuation $V_{\bar x}: \bar x \rightarrow \{0,1\}$
        such that $\forall \bar y \, \lnot \varphi'$ holds where
        $\varphi'$ is obtained from $\varphi$ by replacing every
        variable $x \in \bar x$ with the truth constant
        $V_{\bar x}(x)$. Consider any extension $V$ of $V_{\bar x}$ to
        the variables in $\bar y$ and the interpretation
        $\Imc_V$. Since $\Imc_V$ is a model of \Kmc with
        $\Imc_V \not\models q(f)$, to show that
        \mbox{$\circkb \not\models q(f)$} it remains to prove
        that there is no model $\Jmc <_\CP \I$ of \Kmc.

        Assume to the contrary that there is such a $\Jmc$. We first
        observe that $A^\Jmc=A^{\Imc_V}$ for all
        $A \in \{ \cvval, \cxval, \ccval \}$. This holds for $\cvval$
        since $\cvval^\Jmc \subsetneq \cvval^{\Imc_V}$ means that \Jmc
        does not satisfy \Amc, and likewise for $\ccval$. It also
        holds for $\cxval$ since every model of \Kmc must make
        $\cxval$ true at at least one of $\itrueof{x}$ and
        $\ifalseof{x}$ for all $x \in \bar x$. This is because of
        CIs~(\ref{eq:xvariables_have_value}),
        (\ref{eq:xvalues_are_vvalues}), (\ref{eq:xeval_is_eval}), and
        (\ref{eq:implxval}), the role
        disjointness~(\ref{eq:eval_is_not_negeval}), the
        assertions~(\ref{eq:varblock}) and~(\ref{eq:varblocktwo}), and
        the fact that minimization of $\cvval$ is preferred over
        minimization of $\cxval$.  But no subset of $\cxval^{\Imc_V}$
        satisfies this condition, so we must have  $\cxval^{\Imc_V}
        \subseteq \cxval^{\Jmc}$,
        consequently $\cxval^{\Jmc}=\cxval^{\Imc_V}$.

The above and $\Jmc <_\CP \I$ means that $\cfval^\Jmc \subsetneq
\cfval^{\Imc_V}$. Since \Jmc is a model of \Kmc, this implies $\cfval^\Jmc
= \{ f \}$.

Since $\cxval^\Jmc = \cxval^{\Imc_V}$ and \Jmc is a model of \Kmc,
$V(x)=1$ implies $(x,\itrueof{x}) \in \reval^\Jmc$ and $V(x)=0$
implies $(x,\ifalseof{x}) \in \reval^\Jmc$. Moreover, since
$\cvval^\Jmc = \cvval^{\Imc_V}$ and \Jmc is a model of \Kmc, for every
$y \in \bar y$ we have $(y,\itrueof{y}) \in \reval^\Jmc$ or
$(y,\ifalseof{y}) \in \reval^\Jmc$.  We thus find an extension $V'$ of
$V_{\bar x}$ to $\bar x \cup \bar y$ that is \emph{compatible with}
\Jmc in the sense that for all $v \in \bar x \cup \bar y$,
                               %
\begin{itemize}
\item 
$V'(v)=1$ implies $(v,\itrueof{v}) \in \reval^\Jmc$ and 
\item $V'(v)=0$ implies $(v,\ifalseof{v}) \in \reval^\Jmc$.
\end{itemize}
%
Choose some such $V'$. Since $\forall \bar y \, \lnot \varphi'$ holds,
at least one of the clauses must be made false by $V'$. As explained
alongside the construction of \Kmc, that clause can only have an
$\rceval$-edge to $f$. By~(\ref{eq:rcevalfcevaldisj}), the outgoing
$\rfeval$-edge from $f$ cannot end at $f$. But $\cfval^\Jmc = \{ f \}$
and thus~(\ref{eq:clauses_have_value}) implies that $f$ is the only
point where that edge may end.  We have arrived at a contradiction.


\smallskip ``$\Leftarrow$''.  Assume that
$\forall \bar x \exists \bar y \, \varphi(\bar x, \bar y)$ is true and
let \Imc be a model of $\circkb$. We have to show that
$\Imc \models q(f)$.
To this end, we first observe that
% 
\begin{equation*}
\cvval^\Imc = \{ a \mid \cvval(a) \in \Amc \}.
\tag{$*$}
\end{equation*}
                          %
If this is not the case, in fact, then we find a model
$\Jmc <_\CP \Imc$ of \Kmc, contradicting the minimality of \Jmc.
This model \Jmc is essentially $\Imc_V$ except that we might have
to extend the domain with additional elements that do not occur in
the extension of any concept or role name, to make sure that the
domains of \Imc and of $\Imc_V$ are identical.

It follows from ($*$) and the fact that \Imc is a model of \Kmc that
for every $x \in \bar x$, we have $(x,\itrueof{x}) \in \reval^\Jmc$ or
$(x,\ifalseof{x}) \in \reval^\Jmc$.  Consequently, we find a valuation
$V_{\bar x}$ for $\bar x$ that is compatible with \Imc as defined in
the ``$\Rightarrow$'' direction of the proof. Since
$\forall \bar x \exists \bar y \, \varphi(\bar x, \bar y)$ is true, we
can extend $V_{\bar x}$ to a valuation $V$ for $\bar x \cup \bar y$
that satisfies $\varphi$. Consider the model $\Imc'_V$, extended to
domain $\Delta^\Imc$. By construction of $\Imc'_V$ and ($*$), we have
$\cvval^\Imc = \cvval^{\Imc'_V}$. Using the facts that \Imc is a
minimal model of \Kmc and the construction of $\Imc'_V$, it can now be
observed that $\cxval^\Imc=\cxval^{\Imc'_V}$.  Moreover, by
construction $\Imc'_V$ interprets $\ccval$ and $\cfval$ in a the
minimal possible way among all models of \Kmc. Since \Imc is a minimal
model, this implies $\ccval^\Imc=\ccval^{\Imc'_V}$ and
$\cfval^\Imc=\cfval^{\Imc'_V}$. In particular,
$\cfval^{\Imc}= \{ f \}$. But this implies $(f,f) \in \rfeval^\Imc$ as
all objects with an incoming $\rfeval$-edge must satisfy $\cfval$.  It
follows that $f \in \cgoal^\Imc$ and thus $\Imc \models q(f)$, as
desired.
\end{proof}

==> thm-data-lower-dllitepos.tex <==
%!TEX root = main.tex

\begin{theorem}
	\label{thm-data-lower-dllitepos}
	CQ evaluation over \dllitepos cKBs involving a single minimized predicate and no fixed predicate is \coNP-hard w.r.t.\ data complexity
\end{theorem}

\begin{proof}
	\newcommand{\redge}{\mathsf{edge}}
	\newcommand{\cvertex}{\mathsf{Vertex}}
	\newcommand{\rhascol}{\mathsf{hasCol}}
	\newcommand{\ccolor}{\mathsf{Color}}
	We reduce the complement of the graph 3-colorability problem (3Col) to evaluating the Boolean CQ:
	\[
	q = \exists y_1 \, \exists y_2 \, \exists y ~ \redge(y_1, y_2) \land \rhascol(y_1, y) \land \rhascol(y_2, y)
	\]
	over the \dllitepos TBox:
	\[
	\tbox = \{ \cvertex \incl \exists \rhascol, \exists \rhascol^- \incl \ccolor \},
	\]
	where $\ccolor$ is minimized while all other predicates varying.
	Let $\CP$ be the resulting circumscription pattern.
	Given an instance $\graph = (\vertices, \edges)$ of 3Col, we build an ABox $\abox$ containing the following assertions:
	\begin{align}
		\cvertex(v) & \text{ for all } v \in \vertices
		\\
		\redge(v_1, v_2) & \text{ for all } \{v_1, v_2\} \in \edges
		\\
		\ccolor(c) & \text{ for all } c \in \{ r, g, b \}
	\end{align}
	We now prove the following claim:
	\[
	\graph \notin \text{3Col} \iff \circkb \models q
	\]
	First notice that every model $\I$ of $\circkb$ verifies $\ccolor^\I = \{ r, g, b \}$.
	Indeed, by contradiction, if $\I$ contains $e \in \ccolor^\I \setminus \{ r, g, b \}$, then we can build $\Jmc$ a model of $\kb$ with $\Jmc <_\CP \I$ by modifying $\I$ as follows:
	\begin{itemize}
		\item remove $e$ from $\ccolor^\I$, that is $\ccolor^\Jmc = \ccolor^\Imc \setminus \{ e \}$;
		\item reroute $\rhascol$ as: $\rhascol^\Jmc = \{ (v, r) \mid v \in (\exists \rhascol)^\I \}$.
	\end{itemize}
	It is then straightforward that $\Jmc$ satisfies the desired properties, contradicting $\I$ being a model of $\circkb$.
		
	``$\Rightarrow$''. Assume $\graph \notin \text{3Col}$ and consider a model $\I$ of $\Jmc$.
	By the above remark, we have $\ccolor^\I = \{ r, g, b \}$ and from $\I$ being a model of $\kb$, we can find a mapping $\tau : \vertices \rightarrow \{ r, g, b\}$ of $\graph$ such that for all $v \in \vertices$, if $\tau(v) = c$ then $(v, c) \in \rhascol^\I$.
	Since, by assumption, $\graph \notin \text{3Col}$, there exists an edge $\{ v_1, v_2 \} \in \edges$ such that $\tau(v_1) = \tau(v_2) = c$ for some $c \in \{ r, g, b \}$, which ensures $y_1 \mapsto v_1, y_2 \mapsto v_2, y \mapsto c$ is an homomorphism of $q$ in $\I$.
	
	``$\Leftarrow$''. Assume $\graph \in \text{3Col}$ and consider a 3-coloring $\tau : \vertices \rightarrow \{ r, g, b\}$.
	We build a model $\I_\tau$ of $\circkb$ by interpreting all concepts and roles as in $\abox$ except for $\rhascol$, which is interpreted as:
	\[
	\rhascol^{\I_\tau} = \{ (v, c) \mid v \in \vertices, \tau(v) = c \}.
	\]
	It is straightforward that $\I$ models $\circkb$ and does not embed $q$ (since $\tau$ is a 3-coloring).
\end{proof}

==> thm-data-upper-alchi.tex <==
%!TEX root = main.tex

\begin{theorem}
\label{thm-data-upper-alchi}
	UCQ evaluation over \ALCHI cKBs is in $\Uppi^\text{P}_2$ w.r.t.\ data complexity.
\end{theorem}

\begin{proof}
	We describe a $\NPclass^{\coNP}$ procedure to decide the complement of our problem.
	We start by guessing an interpretation \Imc with polynomial size w.r.t.\ data complexity.
	We then check whether \Imc is a model of$\circkb$ using a $\coNP$ oracle, and return ``no'' if it isn't.
	If $\I$ is a model of $\circkb$, we further check, for each $q \in \Query$ whether there exists a match for $q$ in \Imc, which is performed in $|\Imc|^{|q|}$ deterministic time.
	We return ``yes'' if there is no such match, and ``no'' otherwise.
	Due to Lemma~\ref{lem-quotient}, if a countermodel $\I$ for $\Query$ over $\circkb$ exists, then there is an accepting run for our procedure which guesses the corresponding model $\J$.
	The converse is trivial, as an accepting run witnesses existence of a countermodel for $\Query$ over $\circkb$.
\end{proof}

==> thm-data-upper-boolh-instance.tex <==
%!TEX root = main.tex



\begin{theorem} \label{thm-data-upper-boolh-instance} AQ evaluation on
	circumscribed $\dlliteboolh$ KBs is in $\PTime$.
\end{theorem}

\begin{proof}
	We compute $\kb'$, which can be done in polynomial-time and further checks whether $\Circ(\kb') \models C(c)$, which is can be decided in $\TwoExpTime$ w.r.t.\ the size of $\kb'$, that in constant time w.r.t.\ data complexity.
	The correctness of this procedure immediately follows from Lemma~\ref{lemma-data-indep}.
\end{proof}

==> thm-data-upper-dlliter.tex <==
%!TEX root = main.tex

\begin{theorem}
	\label{thm-data-upper-hornh}
	UCQ answering over $\dlliteboolh$ cKBs is in \coNP w.r.t.\ data complexity.
\end{theorem}

\begin{proof}
	We exhibit an $\NPclass$ procedure to decide the complement of our problem, that is existence of a countermodel for UCQ $q$ over $\dllitebool^{\Hmc^-}$ cKB $\circkb$.
	Our procedure starts by guessing an interpretation $\I$ whose domain has size at most $|\Amc|+(2^{|\Tmc|+2}+1)^{3|q|}$.
	This can be done in linearly many non-deterministic steps (w.r.t.\ data complexity)
	It further checks whether $\I$ is a model of $\kb$ that does not entail $q$, and rejects otherwise.
	This can essentially be done naively in $\sizeof{\domain{\I}}^{\sizeof{\tbox}\sizeof{q}}$ deterministic steps, that is still linear \textcolor{blue}{Really? Isn't it just polynomial?} w.r.t.\ data complexity.
	The procedure finally checks whether $\I$ complies with $\CP$ by
	iterating over each $\Pmc$ with $\sizeof{\Pmc} \leq 2 \sizeof{\tbox} + 1$ and checking whether there exists a model $\J_\Pmc$ of $\kb$ s.t.\ $\J_\Pmc < \I_\Pmc$.
	If, for a choice of $\Pmc$ and we can find such a $\J_{\Pmc}$ then our procedure rejects.
	Notice that iterating over such $\Pmc$ can be done in $\sizeof{\domain{\I}}^{2 \sizeof{\tbox} + 1}$ iterations since we require $\sizeof{\Pmc} \leq 2 \sizeof{\tbox} + 1$.
	Computing $\I_\Pmc$ follows directly from the choice of $\Pmc$.
	Since each $\I_\Pmc$ has constant size w.r.t.\ data complexity, iterating over each possible $\J_\Pmc$ can be done naively with constantly many steps.
	Overall, the procedure uses a linear number of non-deterministic steps at the beginning and further performs several checks using constantly \textcolor{blue}{what about the deterministic steps that are linear/polynomial w.r.t.\ data complexity, e.g., the check whether \Imc is a model of \Kmc that does not entail $q$?} many more deterministic steps.
	
	It remains to prove that there exists an accepting run iff there is a countermodel for $q$ over $\circkb$.
	If there exists an accepting run, then the corresponding guessed interpretation $\I$ is a model of $\kb$ that does not entail $q$, and the ``$2 \Rightarrow 1$'' direction from Lemma~\ref{lemma-criteria-data} ensures it also comply with $\CP$.
	Conversely, if there exists a countermodel, then Lemma~\ref{lem-quotient} ensures existence of a countermodel $\I$ whose domain has size at most $|\Amc|+(2^{|\Tmc|+2}+1)^{3|q|}$.
	This $\I$ can be guessed by the procedure, and as \Imc is indeed a model of $\kb$ not entailing $q$, will not be rejected.
	The ``$1 \Rightarrow 2$'' direction from Lemma~\ref{lemma-criteria-combined} further ensures $\I$ also passes the remaining checks performed by the procedure.
\end{proof}
